Transmission curves of narrow-band filters in large-FoV and fast astronomical instruments

Narrow-band filters are often used to constrain the chemical composition of astronomical objects through photometry. A challenge to derive accurate photometry is that narrow-band filters are based on interference of multiple reflections and refractions between thin layers of transparent dielectric material. When the light rays reach the surface of a filter not perpendicular to it, they cross the layers obliquely travelling a path longer than the thickness of the layers and different for each inclination. This results in a blue-shift of the central wavelength and a distortion of the transmission curve. Hence, particular care should be taken when narrow band filters are used in presence of small f-numbers and large non-telecentric angles, as frequent in the large field of view (FoV) instruments. Sometimes, the broadening and central wavelength shift of the transmission curve are considered and compensated in the design of filters for instruments with a small f-number. Here we consider the combined effect of small f-number, non-telecentricity and large FoV. Where single spectral lines are considered, a shift in central wavelength or a change in the shape of the transmission curve may introduce an instrumental dispersion in luminosity and in the linked color indices. We found that transmission curves of narrow band filters can be significantly different in shape than the nominal ones. The bottom limits for filters' effective FWHM for each f-number; the monotonic behavior of the blue-shift with distance from the center of FoV; the monotonic quality decrease of the transmission curves and the photometric dispersion introduced by the filters are computationally estimated. This work could represent a useful tool to evaluate the fitness of a particular filter at a particular facility.

==> TeX_files/AngleOnFilter.tex <==
\begin{tikzpicture}[>=stealth, inner sep=0pt, outer sep=2pt,scale=0.6]
	\draw  (0,0) circle (6);
	%\draw[thick] (0,0) circle (8);
	\fill[white] (0,0) circle(1);
	\draw (0,0) circle (1);
	\draw[thick,->] (-8,0)--(8,0);
	\foreach \x in {1.5,2,...,6} {
		%\pgfmathsetmacro\randalfa{rand*180};
		\def\randalfa{0}
		\foreach \alfa in {0,5,...,355} {

		\draw[thick,black!50,->] ({\x*sin(\alfa+\randalfa)},{\x*cos(\alfa+\randalfa)}) -- ({(0.95*\x)*sin(\alfa+\randalfa)},{(0.95*\x)*cos(\alfa+\randalfa)});
		}
	}
\end{tikzpicture}

\begin{tikzpicture}[scale=0.6]
		\foreach \x in {-8,-7,-6,-5,-4,-3,-2,2,3,4,5,6,7,8}{
		\draw (\x,0) -- (0,-11);
		}
		\draw (-8,-2.74) -- (8,-2.74);
		\draw (-8,-2.84) -- (8,-2.84);
		\draw[dashed] (6,-1) -- (6,-5);
		\draw (6,-1) coordinate(a) -- (6,-2.74) coordinate(b) --(8,0) coordinate (c) pic["$\rho_{0}=36\degree$", draw=orange,<->,angle eccentricity=1.3,angle radius=1cm]{angle=c--b--a};
		\draw (0,-2.5) node[above, align= center,text width=3cm, font=\small]{Close to normal rays fell in the obstruction};
\end{tikzpicture}



==> TeX_files/CaseStudy.tex <==
\chapter[Performance dell'indice $Cn_{JWL}$ ]{Performance dei filtri JWL39 e Ca per la stima dell'indice $Cn_{JWL}$ su LBC}\label{chap:casi}


\section{Caratteristiche dell'indice $Cn_{JWL}$ e modellizzazione dei filtri}

Come abbiamo già visto nel capitolo \ref{chap:MPsGCs}, lo studio delle popolazioni multiple negli ammassi globulari può trarre giovamento dallo studio delle abbondanze di elementi leggeri. Stelle di prima e seconda generazione (1G, 2G) presentano diverse abbondanze di alcuni elementi leggeri (inclusi C ed N) e anticorrelazioni tra gli stessi, probabilmente dovute alle catene di cattura protonica ed in particolare al ciclo CNO. La regione spettrale intorno a $3883\AA$ include la banda di assorbimento molecolare del CN per cui, a parità di temperatura efficace, Teff, e gravità, gli spettri di stelle di 2G mostrano bande CN più forti di quelli delle stelle di 1G. Scegliendo un filtro in grado di selezionare la banda a 3883\AA, le stelle di 2G avranno magnitudini più deboli di quelle di 1G. \\

Nella sezione \ref{sec:CneLee} abbiamo presentato l'indice spettrale S(3839), utilizzato per stimare l'abbondanza di CN tramite l'analisi degli spettri stellari, come indice adatto alla separazione delle stelle di 1G e 2G. Abbiamo anche accennato al fatto che Lee \parencite{Lee_2015, Lee_2017,Lee_2019} ha definito l'indice $Cn_{JWL}$ come differenza $m_{JWL39}-m_{NewCa}$ dei filtri JWL39 e NewCa da lui disegnati per la campagna osservativa tramite il telescopio da 0.9m del CTIO. In \textcite{Lee_2017} è stata mostrata una forte correlazione fra l'indice spettrometrico S(3839), e la sua rettificazione $\delta S(3839)$, con l'indice $Cn_{JWL}$, come visibile in figura \ref{figure:s3839}: con coefficiente di correlazione di Pearson rispettivamente pari a 0.757 e 0.941. L'indice ha inoltre dimostrato la sua ottima capacità di distinguere popolazioni multiple nel diagramma colore magnitudine (CMD), come visibile nel confronto in figura \ref{figure:confjwl} con altri indici fotometrici, utilizzati per lo studio delle popolazioni multiple negli ammassi globulari.\\

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{Figure/S3839vscnjwl.png}
	\caption{In \textcite{Lee_2017}, i pannelli (c) e (d) mostrano l'ottima correlazione dell'indice $Cn_{JWL}$ con l'indice spettrale S(3839) e $\delta S(3839)$ per le stelle di M5 studiate in \textcite{Smith_2013}}\label{figure:s3839}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{Figure/Confrontojwl.png}
	\caption{In \textcite{Lee_2017} sono riprodotti i diagrammi colore-magnitudine ottenuti con differenti indici fotometrici. L'indice $Cn_{JWL}$ mostra tutta la sua capacità di distinguere popolazioni multiple nel RGB}\label{figure:confjwl}
\end{figure}
 
Con l'obbiettivo di valutare la realizzabilità e l'utilità di un simile set di filtri su un telescopio a grande campo e di classe 8m, utilizzeremo qui i risultati, e il codice Python con cui li abbiamo ottenuti, presentati al capitolo \ref{Chap:Numerical}. \\
\textcite{Lee_2017} e \textcite{Lee_2019} hanno mostrato gli interessantissimi risultati ottenuti con uno strumento dotato di ridotta capacità di raccogliere radiazione (0.9m di apertura) ma ottimo campo di vista. La possibilità di utilizzare un simile set di filtri su uno strumento molto più grande e con simile campo di vista è sicuramente allettante per i motivi presentati in \ref{sec:grandetelescopio}.\\

Large Binocular Camera Blue Channel (LBC-B), lo strumento installato al primo fuoco di uno dei due specchi del Large Binocular Telescope (LBT) in Arizona, è un ottimo candidato per questi obbiettivi dato il suo campo di vista corretto del diametro di $\sim30 arcmin$ e uno specchio collettore di $8.4m$ \parencite{Giallongo_2008}. A tali caratteristiche si accompagnano però un rapporto focale molto esigente, F/1.45, e angoli non telecentrici piuttosto significativi. Per questo si rende necessario uno studio dettagliato della risposta in tale sistema ottico dei filtri interferenziali desiderati: in particolare la presenza di angoli non-telecentrici può introdurre una significativa aberrazione differenziale lungo il campo di vista come spiegato nei capitoli precedenti.\\
 
Per il presente studio abbiamo modellizzato approssimativamente i filtri $JWL39$ e $Ca_{New}$ come definiti in \textcite{Lee_2017}. In tabella \ref{table:EmpiFilter} sono sintetizzate le caratteristiche dei filtri costruiti per il 0.9m-CTIO \parencite{Lee_2017}, quelli approssimati per il presente lavoro di tesi e nelle ultime due colonne questi modificati dalla presenza di un rapporto focale molto sostenuto pari a quello di LBC \parencite{Giallongo_2008}.

\begin{table}[h]
	\centering
	\begin{tabular}{l|rr|rr|rr}
		& &\textcite{Lee_2017} & & Modello & & Modello in F/1.4 \\
		& $Ca_{New}$ & $JWL39$ & $Ca_{New}$ & $JWL39$ & $Ca_{New}$ & $JWL39$ \\ \hline\hline
		$\lambda_pivot$  & 3950 & 3900 & 3952 & 3901 & 3923 & 3873 \\ 
		$fwhm$ & 90 & 180 & 90 & 181 & 92 & 187 \\ \hline
	\end{tabular}
	\caption{Caratteristiche principali dei filtri usati in \textcite{Lee_2017} e quelli simulati nel presente lavoro, le lunghezze d'onda sono espresse in $\AA$} \label{table:EmpiFilter}
\end{table}

\section{Identificazione di popolazioni stellari multiple tramite l'indice $Cn_{JWL}$ su spettri sintetici di stelle di prima e seconda generazione}

Per simulare la resa dei filtri in esame abbiamo utilizzato due spettri sintetici, rispettivamente di prima e seconda popolazione. Questi spettri sono ottenuti come in \textcite{Milone_2018} utilizzando i codici ATLAS12 e SYNTHE con parametri atmosferici corrispondenti a stelle RGB collocate 2 magnitudini sopra il MS turn off in banda HST F814W. Per lo spettro di di 1G (CN-weak) C e N presentano abbondanze solari e [O/Fe]=0.4, in quelle di 2G (CN-strong)invece abbiamo [C/Fe]=-0.50, [N/Fe]=1.21, [O/Fe]=-0.9.

\begin{figure}\label{Figure:}
	\centering
	\includegraphics[width=0.8\textwidth]{Figure/ConfrontoSpettri.pdf}
\end{figure}


\subsection{Il caso ideale dei filtri teorici}
Per costruire un termine di paragone, basato sui medesimi spettri sintetici, abbiamo, per prima cosa, calcolato la convoluzione tra i filtri teorici con le caratteristiche definite in \ref{table:EmpiFilter} (ovvero il nostro modello dei filtri di Lee, rappresentati in blu nella figura \ref{figure:filtJWL}), e gli spettri sintetici descritti poc'anzi. Tale operazione consente di ricavare la distanza lungo l'indice $Cn_{JWL}$ tra i due spettri rappresentanti delle distinte popolazioni stellari. Possiamo interpretare i due spettri sintetici come il centro di due distinte distribuzioni di popolazione stellare lungo l'indice $Cn_{JWL}$. Cioè come rappresentanti di una distribuzione di stelle come quelle visibili nel secondo pannello di figura \ref{figure:confjwl}.\\
Eseguendo questa operazione otteniamo i valori degli indici, non calibrati (\textit{strumentali}), per lo spettro CN-strong  $Cn^{S}_{JWL}=-0.774$ e per lo spettro CN-weak $Cn^W_{JWL}=-0.861$. La differenza nell'indice di colore $Cn_{JWL}$ tra una stella CN-strong e una CN-weak, le due rappresentanti delle popolazioni, è pari a $0.087 mag$.

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/JWL39.pdf}
	\includegraphics[width=0.9\textwidth]{Figure/NewCa.pdf}
	\caption{I filtri riprodotti per il caso studio}\label{figure:filtJWL}
\end{figure}


\subsection{Deformazioni dei filtri teorici e distinguibilità delle popolazioni}

Come si può vedere dalle ultime due colonne di tabella \ref{table:EmpiFilter}, in presenza di un rapporto focale simile a quello LBC assistiamo ad un'arretramento della lunghezza d'onda di pivot pari a circa 3nm per entrambi i filtri, mentre la fwhm varia poco come ci aspettavamo da \ref{sec:quadrati}. Iratio non peggiora in maniera significativa per il filtro JWL39 (da 89\% a 88\%), ben più importante, sebbene non drammatico, quello del filtro $Ca_{NEW}$ che passa da 90\% a 82\%.Si può vedere indicato nei pannelli di figura \ref{figure:filtJWL}. \\ 
Eseguiremo una prima simulazione con le caratteristiche elencate e una seconda utilizzando una coppia di filtri avanzati di 3nm rispetto a quelli modellati. In questo modo la lunghezza d'onda di pivot è realmente pari a quella prevista da \textcite{Lee_2017} per distinguere senza ambiguità il doppietto del CaII e la banda di assorbimento del CN. Procediamo in questo modo dato che, come già accennato, l'arretramento è gestibile in fase di progettazione del filtro.


\begin{table}
	\centering
	\begin{tabular}{l|rrrrrr|r}
		nta & 0\degree & 2\degree & 4\degree & 6\degree & 8\degree & 10\degree & Spread \\ \hline
		CN-s & -0.783 & -0.783 & -0.784 & -0.785 & -0.786 & -0.787 & -0.004 \\ 
		CN-w & -0.873 & -0.874 & -0.874 & -0.875 & -0.877 & -0.878 & -0.005 \\  
		$\Delta$ & 0.090 & 0.091 & 0.090 & 0.090 & 0.091 & 0.091 & / \\ \hline
	\end{tabular}
	\caption{Variazioni in magnitudine dell'indice $Cn_{JWL}$ con i modelli di filtri in presenza di F/1.4 (come in tabella \ref{table:EmpiFilter}) per una stella con spettro sintetico ad alto CN (CN-s) e una a basso CN (CN-w), per differenti angoli non-telecentrici} \label{table:CNmagVar}
\end{table}

\begin{table}
	\centering
	\begin{tabular}{l|rrrrrr|r}
		nta & 0\degree & 2\degree & 4\degree & 6\degree & 8\degree & 10\degree & Spread \\ \hline
		CN-s & -0.6682 & -0.6687 & -0.6703 & -0.6728 & -0.6763 & -0.6806 & -0.0124 \\
		CN-w & -0.7282 & -0.7289 & -0.7307 & -0.7337 & -0.7378 & -0.7429 & -0.0147 \\ 
		$\Delta$ & 0.0600 & 0.0601 & 0.0604 & 0.0609 & 0.0615 & 0.0624 & / \\ \hline
	\end{tabular}
	\caption{Variazioni in magnitudine dell'indice $Cn_{JWL}$ con filtri corretti (+30\AA rispetto al modello iniziale) per una stella con spettro sintetico ad alto CN (CN-s) e una a basso CN (CN-w), per differenti angoli non-telecentrici } \label{table:CNmagVar+30}
\end{table}

Confrontando le due tabelle \ref{table:CNmagVar} e \ref{table:CNmagVar+30} si può notare un andamento comune: all'aumentare dell'angolo non-telecentrico (quindi allontanandosi dal centro del campo di vista) l'indice $Cn_{JWL}$ presenta un lento aumento verso magnitudini più negative. Questo aumento di luminosità si può interpretare osservando le figure \ref{figure:FiltriConSpettro1} e \ref{figure:FiltriConSpettro2}. Infatti vi si può notare come la deformazione del filtro JWL39 riduca il peso relativo della banda del Ca e consenta un piccolo incremento di flusso proveniente da una zona spettrale a $\lambda$ minori. Allo stesso tempo il filtro $Ca_{new}$ perde efficienza sulla banda del Ca \textit{spalmandosi} maggiormente senza però includere intervalli spettrali di maggiore intensità\footnote{$Ca_{new}$ presenta, per l'\textit{nta} usato per le figure, un drastico calo dell'efficienza massima per i motivi analizzati al capitolo \ref{Chap:Numerical}}. La combinazione, di non facile interpretazione, di questi effetti aumenta il rapporto tra il flusso nel filtro JWL39 e quello in CaNew che si traduce per $Cn_{JWL}=-2.5\log_{10}(F_{JWL39}/F_{CaNew)}$ in valori più negativi. \\
Questo effetto risulta pressoché identico per lo spettro CN-weak e per quello CN-strong, determinando uno spostamento sia per le stelle 1G che 2G verso indici $Cn_{JWL}$ più negativi, mentre la distanza in indice tra le due popolazioni rimane all'incirca costante ai vari angoli come riportato nella terza riga delle tabelle \ref{table:CNmagVar}, \ref{table:CNmagVar+30} e visibile in figura \ref{figure:Cnvsnta}.\\

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/ConfrontoFiltriSsnta0.pdf}
	\includegraphics[width=0.9\textwidth]{Figure/ConfrontoFiltriSsnta025.pdf}
	\caption{Filtri ad angolo 0 e 0.25, con sovraimpresso uno spettro}\label{figure:FiltriConSpettro1}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/ConfrontoFiltriNta0+30.pdf}
	\includegraphics[width=0.9\textwidth]{Figure/ConfrontoFiltriNta025+30.pdf}
	\caption{Filtri ad angolo 0 e 0.25, con sovrimpressi i due spettri Cn-w e Cn-s}\label{figure:FiltriConSpettro2}
\end{figure}
 
 
Osservando le due tabelle la separazione tra le popolazioni aumenta sia nel caso dei filtri non corretti, $\Delta_{nta}\sim0.090mag$, che nel caso dei filtri corretti, $\Delta_{nta}\sim0.060mag$. Inoltre i filtri non corretti presentano anche con uno spread, ovvero l'allontanamento in indice $Cn_{JWL}$ della stella ai bordi rispetto a quella al centro del campo di vista, più contenuto $Sp\sim0.005mag$ vs $Sp\sim0.014mag$. \\
Scegliere i filtri non corretti, necessiterebbe di una nuova verifica della correlazione tra il nuovo indice\footnote{Essendo la banda dei filtri differente da quella di Jae-Woo Lee si tratta sostanzialmente di un indice differente dal $Cn_{JWL}$}, e gli indici spettrali. Ci limitiamo quindi qui a considerare i valori di tabella \ref{table:CNmagVar+30}, che presentano una distanza tra le popolazioni, al centro del campo di vista, inferiore a quella del set teorico ($0.060 mag$ vs $0.087 mag$). Tale ridotta distanza è da ricondurre alla degradazione del filtro $Ca_{NEW}$ dovuta al rapporto focale come evidenziato in precedenza.\\

Essendo l'effetto di alterazione dell'indice simile per i due tipi di spettro, per ogni angolo non-telecentrico le due popolazioni rimangono distinguibili.\\
%Ci interessa però valutare, non se due stelle di spettri diversi posizionate nello stesso punto del campo di vista sono distinguibili, bensì se un mix di stelle 1G e 2G distribuite su tutto il campo in maniera casuale\footnote{Se è presente una distribuzione radiale non uniforme l'effetto va più attentamente osservato} presentino un allargamento della distribuzione dovuto al sistema di filtri interferenziali che le renda più difficilmente distinguibili. \\
Ci interessa quindi lo spread che gli angoli non-telecentrici introducono nelle due popolazioni. Possiamo qui stimare il fenomeno supponendo di avere una stella 2G (CN-strong) al centro del campo e una 1G (CN-weak) ai bordi o viceversa una stella povera in CN al centro e una ricca di CN ai bordi. Nel primo caso la distanza tra gli indici delle due stelle risulta maggiorata $\Delta_{max}=0.075$ nel secondo con una CN-weak al centro e una CN-strong ai bordi la distanza si ridurrebbe a $\Delta_{min}=0.048$. Le popolazioni quindi rimangono ancora ben distinguibili in via teorica e il rapporto $D_{pop}=\frac{Sp_{max}}{\bar{Delta_{nta}}}$, nel nostro caso $D_{pop}=0.23$, può essere utile per capire l'entità dell'aberrazione differenziale introdotta all'interno del campo di vista dalla specifica configurazione ottica in relazione alle distinte popolazioni che si ritengono presenti nell'ammasso.\\

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth]{Figure/Lee17fitgauss.png}
	\caption{immagine tratta da \textcite{Lee_2017} dove viene eseguito un fit gaussiano sugli istogrammi N vs $Cn_{JWL}$ per la stima del rapporto fra popolazioni 1G e 2G}\label{figure:histgauss}
\end{figure}


La presenza di questo allargamento strumentale può complicare il population tagging e il fit con le distribuzioni gaussiane degli istogrammi delle distribuzioni come quelli in figura 7 e 9 del \textcite{Lee_2017} di cui riportiamo un estratto in figura \ref{figure:histgauss}. Infatti la distribuzione gaussiana intrinseca risulterebbe deformata asimmetricamente (verso $Cn_{JWL}$ minori) peggiorando la qualità del fit e (dipende dallo spread e dalla separazione intrinseci) potenzialmente comportando una sovrapposizione maggiore delle due popolazioni rendendo l'assegnazione di una stella ad una popolazione o ad un'altra più arbitraria\footnote{chiaramente una analisi eseguita tramite ChM può attenuare questo problema}. 
L'effetto però è simile per i due tipi di spettro e prevedibile. Previa una adeguata verifica sperimentale delle simulazioni fin qui eseguite ed ulteriori simulazioni con variati parametri stellari, l'effetto potrebbe essere corretto. In fase di riduzione dati, in funzione della distanza dal centro del campo di vista, l'indice $Cn_{JWL}$ di ogni stella andrebbe incrementato del relativo ammontare introdotto dalla risposta dei filtri.  

In figura \ref{figure:Cnvsnta} si vede l'andamento dell'indice $Cn_{JWL}$ per le due distinte popolazioni all'aumentare della distanza dal centro del campo di vista. È indicata anche la distanza fra le due popolazioni a vari angoli nel FoV che cresce molto lentamente, come visibile nel pannello inferiore. 

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/GraficoNtaCn99.pdf}
	\includegraphics[width=0.9\textwidth]{Figure/GraficoNta982189.pdf}
	\caption{L'indice $Cn_{JWL}$ con l'angolo non-telecentrico e il corrispondente angolo nel FoV per i due tipi di spettro ($\mu_*=2$).Nel pannello inferiore distanza fra le due popolazioni. }\label{figure:Cnvsnta}
\end{figure}

Nell'ultima figura \ref{figure:CMDPopolazini} vediamo una rappresentazione di dove si troverebbero in un diagramma Luminosità vs. $Cn_{JWL}$ le due popolazioni a vari angoli nel campo di vista. Si nota l'allargamento strumentale e allo stesso tempo come esso rimanga contenuto. 

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/VvsCn.pdf}
	\caption{Rappresentazione di come si comporterebbero le due popolazioni in un CMD. L'indice $Cn_{JWL}$ si sposta verso sinistra all'aumentare dell'angolo nel FoV determinando un allargamento strumentale delle popolazioni, che rimangono però ben distinguibili.}\label{figure:CMDPopolazini}
\end{figure}

==> TeX_files/Conclusions.tex <==
\chapter{Conclusions}

==> TeX_files/Experimental.tex <==
\chapter{Validazioni sperimentali}\label{chap:exp}

Utilizzando un filtro interferenziale disponibile in laboratorio andiamo a fare misure del tipo riportato nelle tabelle \ref{table:squarefilter} e \ref{table:squarefilternta} e confrontarli con la riproduzione numerica del filtro presente in laboratorio. Il tutto per validare la bontà delle simulazioni numeriche e del codice di cui al capitolo \ref{Chap:Numerical}.

==> TeX_files/Immaginefiltro2.tex <==
\begin{tikzpicture}[x={(-0.866cm,-0.5cm)}, y={(-0.866cm,0.5cm)}, z={(0cm,1cm)}, scale=0.8,
%Option for nice arrows
>=stealth, %
inner sep=0pt, outer sep=2pt,%
axis/.style={thick,->},
wave/.style={thick,color=#1,smooth}]
% Colors
\colorlet{darkgreen}{green!50!black}
\colorlet{lightgreen}{green!80!black}
\colorlet{darkred}{red!50!black}
\colorlet{lightred}{red!80!black}
\colorlet{lightblue}{blue!80!black}

% Frame
\coordinate (O) at (0, 0, 0);
\draw[axis] (O) -- +(12.5, 0,   0);% node [bottom] {Direction of Propagation};
\draw[axis] (O) -- +(0,  2.5, 0);% node [right] {y};
\draw[axis] (O) -- +(0,  0,   2);% node [above] {z};

\newcommand\alfa{90}


%BEAM
\draw plot[variable=\y,domain=0:360,samples=180] (0,{cos(\y)},{sin(\y)});
\draw plot[variable=\y,domain=0:360,samples=180] (6,{cos(\y)},{sin(\y)});
\foreach \y in {45,50,...,225}		
\draw[red!50] (0,{cos(\y+1)},{sin(\y+1)}) -- ({6+cos(\alfa)},{cos(\y+1)},{sin(\y+1)}); 
\foreach \y in {45,50,...,225}	
\draw[blue!50] (0,{cos(\y+2)},{sin(\y+2)}) -- ({6+cos(\alfa)*cos(\y)},{cos(\y+2)},{sin(\y+2)});
\foreach \y in {45,50,...,225}	
\draw[green!50] (0,{cos(\y)},{sin(\y)}) -- ({6+cos(\alfa)*cos(\y)},{cos(\y)},{sin(\y)});
\foreach \y in {45,50,...,225}	
\draw[yellow!50] (0,{cos(\y+3)},{sin(\y+3)}) -- ({6+cos(\alfa)*cos(\y)},{cos(\y+3)},{sin(\y+3)});

\foreach \y in {5,10,...,360}			
\draw[blue!50]({6.25+cos(\alfa)*cos(\y+1)},{cos(\y+1)},{sin(\y+1)})--({6.25+cos(\alfa)*cos(\y+1)-6*cos((90-\alfa)*2)},{sin(\alfa)*cos(\y+1)+6*sin((90-\alfa)*2)},{sin(\y+1)}); 
\foreach \y in {5,10,...,360}			
\draw[red!50]({6.25+cos(\alfa)*cos(\y)},{cos(\y)},{sin(\y)})--({6.25+cos(\alfa)*cos(\y)-6*cos((90-\alfa)*2)},{sin(\alfa)*cos(\y)+6*sin((90-\alfa)*2)},{sin(\y)}); 



% Incident Blue
\draw[wave=blue, variable=\x,samples at={0,0.25,...,6.5}]
plot (\x,{sin(4*\x r)},0);
\foreach \x in{0,0.25,...,6.5}
\draw[color=blue,->] (\x,0,0) -- (\x,{sin(4*\x r)},0);


%Incident Red
\draw[wave=red, variable=\x,samples at={0,0.25,...,6.25}]
plot (\x,{sin(\x r)},0);
\foreach \x in{0, 0.25,...,6}
\draw[color=red,->] (\x,0,0) -- (\x,{sin(\x r)},0);

%Incident Green
\draw[wave=green, variable=\x,samples at={0,0.25,...,6.25}]
plot (\x,{sin(2*\x r)},0);	
\foreach \x in{0, 0.25,...,6}
\draw[color=green,->] (\x,0,0) -- (\x,{sin(2*\x r)},0);

\draw (3,1,1) node [text width=2.5cm, text centered]{Incident Policromatic Beam};
\draw (11,1,1) node [text width=2.5cm, text centered]{Transimitted Filtered Beam};
\draw (3.5,-3.5,-1) node [text width=2.5cm, text centered]{Reflected Beam};





%reflected beam		
\draw[wave=blue, variable=\y,samples at={0,-0.25,...,-6.25}]
plot ({6.25-sin(((4*\y)+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin(((4*\y)+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);
\foreach \y in{0,-0.25,...,-6}
\draw[color=green,->] ({6.25+\y*cos((90-\alfa)*2)},{-\y*(sin((90-\alfa)*2))},0) -- ({6.25-sin((4*\y+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin((4*\y+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);

\draw[wave=red, variable=\y,samples at={0,-0.25,...,-6.25}]
plot ({6.25-sin((\y+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin((\y+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);
\foreach \y in{0,-0.25,...,-6}
\draw[color=red,->] ({6.25+\y*cos((90-\alfa)*2)},{-\y*(sin((90-\alfa)*2))},0) -- ({6.25-sin((\y+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin((\y+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);


\draw[thick,dashed] (6.25,0,0) -- ({6.25-6*cos((90-\alfa)*2)},  {(6*sin((90-\alfa)*2)}, 0);    


%Filter
\draw (6,2.5,2.5) node [text width=2.5cm, text centered]{Thin-layer band-pass filter};
\begin{scope}[thick]
node [above, sloped, midway]{Intefrence filter section}
\foreach \shi in{0,0.1,0.2,0.3}
\filldraw[fill=blue!5] ({6+\shi-(2)*cos(\alfa)},{-2*sin(\alfa)-\shi*cos(\alfa)},-1.5) -- ({6-(2)*cos(\alfa)+\shi},{-2*sin(\alfa)-\shi*cos(\alfa)},1.5) -- ({6+(2)*cos(\alfa)+\shi}, {2*sin(\alfa)-\shi*cos(\alfa)}, 1.5) -- ({6+(2)*cos(\alfa)+\shi},{2*sin(\alfa)-\shi*cos(\alfa)}, -1.5) -- cycle;% Faces  

\foreach \shi in{0,0.1,0.2}
\draw 
({6+\shi-(2)*cos(\alfa)},{-2*sin(\alfa)-\shi*cos(\alfa)},-1.5) -- ({6-(2)*cos(\alfa)+\shi+0.1},{-2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},-1.5)
({6+\shi-(2)*cos(\alfa)},{-2*sin(\alfa)-\shi*cos(\alfa)},1.5) -- ({6-(2)*cos(\alfa)+\shi+0.1},{-2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},1.5)
({6+\shi+(2)*cos(\alfa)},{2*sin(\alfa)-\shi*cos(\alfa)},-1.5) -- ({6+(2)*cos(\alfa)+\shi+0.1},{2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},-1.5)
({6+\shi+(2)*cos(\alfa)},{2*sin(\alfa)-\shi*cos(\alfa)},1.5) -- ({6+(2)*cos(\alfa)+\shi+0.1},{2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},1.5);
\end{scope}	


% Electric field vectors
\draw[wave=green, variable=\x,samples at={6.50,6.75,...,12}]
plot (\x,{sin(2*\x r)},0);

%Polarized light between polaroid and thin section
\foreach \x in{6.50,6.75,...,12}
\draw[color=green,->] (\x,0,0) -- (\x,{sin(2*\x r)},0);

\draw (6.3,0,0) circle [x={({cos(\alfa)},1,0)},y={(0,0,1))},radius=1];
\draw (12,0,0) circle [x={(0,1,0)},y={(0,0,1))},radius=1];
%	\draw plot[variable=\y,domain=0:360,samples=180] (6,{cos(\y)},{sin(\y)});
%	\draw plot[variable=\y,domain=0:360,samples=180] (12,{cos(\y)},{sin(\y)});
\foreach \y in {45,50,...,225}		
\draw[green!50] ({6.3+cos(\alfa)*cos(\y)},{cos(\y+1)},{sin(\y+1)}) -- (12,{cos(\y+1)},{sin(\y+1)});

\end{tikzpicture}


\begin{tikzpicture}[x={(-0.866cm,-0.5cm)}, y={(-0.866cm,0.5cm)}, z={(0cm,1cm)}, scale=0.8,
%Option for nice arrows
>=stealth, %
inner sep=0pt, outer sep=2pt,%
axis/.style={thick,->},
wave/.style={thick,color=#1,smooth},
polaroid/.style={fill=black!60!white, opacity=0.3},
]
% Colors
\colorlet{darkgreen}{green!50!black}
\colorlet{lightgreen}{green!80!black}
\colorlet{darkred}{red!50!black}
\colorlet{lightred}{red!80!black}
\colorlet{lightblue}{blue!80!black}

% Frame
\coordinate (O) at (0, 0, 0);
\draw[axis] (O) -- +(12.5, 0,   0);% node [bottom] {Direction of Propagation};
\draw[axis] (O) -- +(0,  2.5, 0);% node [right] {y};
\draw[axis] (O) -- +(0,  0,   2);% node [above] {z};

\newcommand\alfa{100}


%BEAM
\draw plot[variable=\y,domain=0:360,samples=180] (0,{cos(\y)},{sin(\y)});
\draw plot[variable=\y,domain=0:360,samples=180] (6,{cos(\y)},{sin(\y)});
\foreach \y in {45,50,...,225}		
\draw[red!50] (0,{cos(\y+1)},{sin(\y+1)}) -- ({6+cos(\alfa)},{cos(\y+1)},{sin(\y+1)}); 
\foreach \y in {45,50,...,225}	
\draw[blue!50] (0,{cos(\y+2)},{sin(\y+2)}) -- ({6+cos(\alfa)*cos(\y)},{cos(\y+2)},{sin(\y+2)});
\foreach \y in {45,50,...,225}	
\draw[green!50] (0,{cos(\y)},{sin(\y)}) -- ({6+cos(\alfa)*cos(\y)},{cos(\y)},{sin(\y)});
\foreach \y in {45,50,...,225}	
\draw[yellow!50] (0,{cos(\y+3)},{sin(\y+3)}) -- ({6+cos(\alfa)*cos(\y)},{cos(\y+3)},{sin(\y+3)});

\foreach \y in {5,10,...,360}			
\draw[green!50]({6.25+cos(\alfa)*cos(\y+1)},{cos(\y+1)},{sin(\y+1)})--({6.25+cos(\alfa)*cos(\y+1)-6*cos((90-\alfa)*2)},{sin(\alfa)*cos(\y+1)+6*sin((90-\alfa)*2)},{sin(\y+1)}); 

\foreach \y in {5,10,...,360}			
\draw[red!50]({6.25+cos(\alfa)*cos(\y)},{cos(\y)},{sin(\y)})--({6.25+cos(\alfa)*cos(\y)-6*cos((90-\alfa)*2)},{sin(\alfa)*cos(\y)+6*sin((90-\alfa)*2)},{sin(\y)}); 


% Incident Blue
\draw[wave=blue, variable=\x,samples at={0,0.25,...,6.5}]
plot (\x,{sin(4*\x r)},0);
\foreach \x in{0,0.25,...,6.5}
\draw[color=blue,->] (\x,0,0) -- (\x,{sin(4*\x r)},0);


%Incident Red
\draw[wave=red, variable=\x,samples at={0,0.25,...,6.25}]
plot (\x,{sin(\x r)},0);
\foreach \x in{0, 0.25,...,6}
\draw[color=red,->] (\x,0,0) -- (\x,{sin(\x r)},0);

%Incident Green
\draw[wave=green, variable=\x,samples at={0,0.25,...,6.25}]
plot (\x,{sin(2*\x r)},0);	
\foreach \x in{0, 0.25,...,6}
\draw[color=green,->] (\x,0,0) -- (\x,{sin(2*\x r)},0);

\draw (3,1,1) node [text width=2.5cm, text centered]{Incident Policromatic Beam};
\draw (11,1,1) node [text width=2.5cm, text centered]{Transimitted Filtered Beam};
\draw (3.5,-3.5,-1) node [text width=2.5cm, text centered]{Reflected Beam};





%reflected beam		
\draw[wave=green, variable=\y,samples at={0,-0.25,...,-6.25}]
plot ({6.25-sin(((2*\y)+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin(((2*\y)+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);
\foreach \y in{0,-0.25,...,-6}
\draw[color=green,->] ({6.25+\y*cos((90-\alfa)*2)},{-\y*(sin((90-\alfa)*2))},0) -- ({6.25-sin((2*\y+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin((2*\y+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);

\draw[wave=red, variable=\y,samples at={0,-0.25,...,-6.25}]
plot ({6.25-sin((\y+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin((\y+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);
\foreach \y in{0,-0.25,...,-6}
\draw[color=red,->] ({6.25+\y*cos((90-\alfa)*2)},{-\y*(sin((90-\alfa)*2))},0) -- ({6.25-sin((\y+3.1415) r)*sin(2*\alfa)+\y*cos((90-\alfa)*2)},{sin((\y+3.1415) r)*cos(2*\alfa)-\y*(sin((90-\alfa)*2))},0);


\draw[thick,dashed] (6.25,0,0) -- ({6.25-6*cos((90-\alfa)*2)},  {(6*sin((90-\alfa)*2)}, 0);    


%Filter
\draw (6,2.5,2.5) node [text width=2.5cm, text centered]{Thin-layer band-pass filter};
\begin{scope}[thick]
node [above, sloped, midway]{Intefrence filter section}
\foreach \shi in{0,0.1,0.2,0.3}
\filldraw[fill=blue!5] ({6+\shi-(2)*cos(\alfa)},{-2*sin(\alfa)-\shi*cos(\alfa)},-1.5) -- ({6-(2)*cos(\alfa)+\shi},{-2*sin(\alfa)-\shi*cos(\alfa)},1.5) -- ({6+(2)*cos(\alfa)+\shi}, {2*sin(\alfa)-\shi*cos(\alfa)}, 1.5) -- ({6+(2)*cos(\alfa)+\shi},{2*sin(\alfa)-\shi*cos(\alfa)}, -1.5) -- cycle;% Faces  

\foreach \shi in{0,0.1,0.2}
\draw 
({6+\shi-(2)*cos(\alfa)},{-2*sin(\alfa)-\shi*cos(\alfa)},-1.5) -- ({6-(2)*cos(\alfa)+\shi+0.1},{-2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},-1.5)
({6+\shi-(2)*cos(\alfa)},{-2*sin(\alfa)-\shi*cos(\alfa)},1.5) -- ({6-(2)*cos(\alfa)+\shi+0.1},{-2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},1.5)
({6+\shi+(2)*cos(\alfa)},{2*sin(\alfa)-\shi*cos(\alfa)},-1.5) -- ({6+(2)*cos(\alfa)+\shi+0.1},{2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},-1.5)
({6+\shi+(2)*cos(\alfa)},{2*sin(\alfa)-\shi*cos(\alfa)},1.5) -- ({6+(2)*cos(\alfa)+\shi+0.1},{2*sin(\alfa)-(\shi+0.1)*cos(\alfa)},1.5);
\end{scope}	


% Electric field vectors
\draw[wave=blue, variable=\x,samples at={6.50,6.75,...,12}]
plot (\x,{sin(4*\x r)},0);

%Polarized light between polaroid and thin section
\foreach \x in{6.50,6.75,...,12}
\draw[color=blue,->] (\x,0,0) -- (\x,{sin(4*\x r)},0);

\draw (6.3,0,0) circle [x={({cos(\alfa)},1,0)},y={(0,0,1))},radius=1];
\draw (12,0,0) circle [x={(0,1,0)},y={(0,0,1))},radius=1];
%	\draw plot[variable=\y,domain=0:360,samples=180] (6,{cos(\y)},{sin(\y)});
%	\draw plot[variable=\y,domain=0:360,samples=180] (12,{cos(\y)},{sin(\y)});
\foreach \y in {45,50,...,225}		
\draw[blue!50] ({6.3+cos(\alfa)*cos(\y)},{cos(\y+1)},{sin(\y+1)}) -- (12,{cos(\y+1)},{sin(\y+1)});

\end{tikzpicture}


==> TeX_files/Introduction.tex <==
\chapter{Introduction}
A part of the galactic globular clusters were cataloged, for the first time, by Frederick William Herschel more than two centuries ago and the long struggle between astronomers and this rich galactic laboratories seemed to be overcome by the wonderful results obtained in the last decades of the twentieth century: particularly fine isochrones, combined with the stellar evolutionary models announced a perfect understanding of the globular clusters and the stellar populations within them. Strange things happens in the history of science, results that seemed settled reveal their weakness after they served to develop an entire field of study. Stellar evolution models hold their validity corroborated by experimental results, by coherence and thousands of observations, notwithstanting a branch of astronomy, on which they were built, has reveled to be, at the best, just a first approximation.
Various papers noticed some strange behavior in the red giant branch, but was the 1995 paper by THIS and THIS that the presence of multiple stars populations inside the same globular cluster become more then a suspect. Piotto Milone and Co. DADADADA, cromosome map, JWL studied using a very small telescope, the 90cm EOSCYE, getting very interesting results by a ground-based instruments, good preview in the show of the incoming end of the HST operations. He used narrow band interferometric filters building his own photometric system. The hope of using similar photometric system or at least to use narrow band filters to evaluate specific spettroscopic bands, guided our study. 
Interferometric filters are composed by a stack of thin (in teh most cases) layers of different refractive index and very sensible to the lenght of the optical path inside them in the selected pass band, having that filters are usually close to the the focal plane in astronomical instruments, a convergent-beam zone, it is clear that the chief ray and marginal ones hits the filter with different angles with all the intermediate options and the strong dependace on the the aperture of the light cone due to the focal ratio of the instrument. 

This thesis work starts by two defining and literature-review chapters: one dedicated to the definition of the issue of the multiple stars populations and the possible usage of narrow-band filters on ground-based telescope and one one the functioning of an interference filter \textit{a la} Fabry-Perrot, the main results from classical optical studies and the characteristics that are more relevant for astronomical cases. A second group of chapters is dedicated to my \textit{experimental} build-up and results, by development of a python code that simulate the distortion of the filter due to the optical design and in chap 5 the validation of these computational results with an optical bench set-up. Last chapter is dedicated to the results for the most general case and in particular for the MSPGCs studies. 

\begin{tikzpicture}[scale=2.5]
%ray 1
\draw[gray, thick] (0,4) -- (3,4);
\draw[gray, thick] (0,1) -- (3,1);
\draw[gray, thick] (3,4.5) -- (3,0.5);
\draw[gray, thick] (0,2.5)-- (6,2.5);

\draw[gray, thick] (3,4) -- (6,2.5);
\draw[gray, thick] (3,1) -- (6,2.5);
%ray 2
\draw[blue, thick] (0,4.2) -- (3,4) -- (6,2.3);
\draw[blue, thick] (0,1.2) -- (3,1) -- (6,2.3);
\draw[blue, thick] (0,2.7) -- (6,2.3);

%focalpoints
\draw[gray, thick] (6,1.2) -- (6,3.5);
%\filldraw[black] (6,2.5) circle (1pt) node[anchor=west]{};
%\filldraw[black] (6,2.3) circle (1pt) node[anchor=west]{};

%filter
\filldraw[color=green!60, fill=green!5, thick](5.2,3.5) rectangle (5.3,1.5);

%magnification
\end{tikzpicture}

\begin{tikzpicture}[scale=1.8]
%marginal ray
\draw[gray, thick] (0,4) -- (3,4);
\draw[gray, thick] (0,1) -- (3,1);
\draw[gray, thick] (3,4.5) -- (3,0.5);

\draw[gray, thick] (3,4) -- (7,2);
\draw[gray, thick] (3,1) -- (7,3);

\draw[gray, thick] (7,3.5) -- (7,1.5);
\draw[gray, thick] (7,2) -- (8.5,2);
\draw[gray, thick] (7,3) -- (8.5,3);
\draw[gray, thick] (0,2.5) -- (8.5,2.5);
%marginal ray 2
\draw[blue, thin] (0,4.2) -- (3,4) -- (6,2.31)-- (7,1.7)--(8.5,1.5);
\draw[blue, thin] (0,1.2) -- (3,1) -- (6,2.31)-- (7,2.7)--(8.5,2.5);
\draw[blue, thin] (0,2.7) -- (3,2.5) -- (7,2.25);

%focalpoint
%\filldraw[black] (6,2.5) circle (2pt) node [above]{};
\draw[gray, thick] (6,1.2) -- (6,3.5);
%filter
\filldraw[color=green!60, fill=green!5, thick](7.3,3.5) rectangle (7.4,1.5);

\end{tikzpicture}


==> TeX_files/MPsGCs.tex <==
\chapter[Cosa è un ammasso globulare?]{Cosa è un ammasso globulare? Le popolazioni multiple e come studiarle}\label{chap:MPsGCs}

Per molti decenni gli ammassi globulari sono stati considerati la più chiara esemplificazione di una Single Stellar Population (SSP) nonostante alcuni fenomeni rimanessero inspiegati in questo quadro. Oggi invece è largamente accettato che la maggior parte degli ammassi globulari sia formata da popolazioni stellari multiple e distinte. \\

La presenza di variazioni nella morfologia del ramo orizzontale di ammassi globulari con la medesima metallicità, la scoperta di disomogeneità chimiche all'interno di singoli ammassi globulari e la scoperta di sequenze multiple nello \textit{straordinario} $\omega Cen$ hanno suscitato l'interesse degli astronomi rispettivamente dagli anni '50, '70 e '90 del ventesimo secolo. Ad esempio, la presenza di una dicotomia nell'abbondanza del CN nel ramo gigante dell'ammasso NGC6752 era stata stabilita tramite uno studio degli spettri di 69 stelle giganti in \textcite{Norris1981AbundanceSI}. Così il secondo parametro della morfologia del ramo orizzontale (HB), suggeriva un legame con una differente composizione in Elio.  \\
Solo recentemente i tre fenomeni, apparentemente distinti, sono stati ricondotti ad aspetti dello stesso. In particolare con la scoperta che le sequenze multiple corrispondono a stelle con differenti abbondanze di C, N, O, Na ed altri elementi (\textcite*{Marino2008}, Yong et al. 2008) e che le diverse regioni dell'HB sono composte da popolazioni stellari distinte (Marino et al. 2011).\\
La scoperta dell'ubiquità delle anomalie chimiche e della presenza di sequenze multiple anche per stelle non evolute hanno suggerito che queste variazioni siano il frutto di una differente composizione iniziale invece che di un effetto evolutivo, possiamo quindi parlare di popolazioni stellari multiple negli ammassi globulari. \\

Lo sviluppo di una fotometria di precisione, tramite migliori tecniche di riduzione dati, ha spianato la strada alla possibilità di distinguere la presenza di differenti popolazioni nei diagrammi colore magnitudine (CMD). Ha dimostrato che l'allargamento in colore, dei vari rami del CMD, non era interamente dovuto ad errori fotometrici ma a popolazioni stellari con diversa composizione chimica. \\
È però la scelta di particolari ed ingegnose combinazioni di filtri, insieme al loro impiego per la costruzione di nuovi tipi di diagramma (pseudo)colore-colore (come le chromosome maps \textcite{Milone2015}) ad aver consentito i maggiori avanzamenti, permettendo l'individuazione dei tratti caratteristici degli ammassi globulari con la sufficiente robustezza statistica. Robustezza consentita dall'analisi contemporanea di miglia di stelle tramite fotometria in sostituzione della classica, ed ancora importantissima, spettrometria a media o alta risoluzione che soffre però forti limitazioni in luminosità ed affollamento del campo. \\

La diffusione delle disomogeneità chimiche degli elementi leggeri negli ammassi globulari è così ampia che è stata proposta una definizione che li ridurrebbe ai soli sistemi stellari che mostrano alcune tipiche anticorrelazioni tra gli elementi leggeri. Tale definizione appare assai insufficiente e non è accettata nella comunità scientifica ma ha sicuramente il pregio \parencite{Gratton2019} di portare l'attenzione sul complesso scenario di formazione degli ammassi globulari.\\
Benché sia ancora in corso il dibattito su come si formi un ammasso globulare, quali siano le sue prime fasi ed anche cosa determini la disparità di abbondanze degli elementi leggeri iniziali, lo studio sistematico degli ammassi globulari della nostra galassia e delle Nubi di Magellano, effettuati tramite ampie survey spettrometriche e fotometriche di alta qualità, come \textcite{Monelli2013} e \textcite{Piotto2015}; gli studi particolari, ed alcune innovazioni anche molto recenti, ci consentono di tratteggiare alcuni fatti fondamentali sulle popolazioni stellari multiple negli ammassi globulari. 

\section{Proprietà delle popolazioni multiple}

Elementi differenti sono creati o distrutti a differenti temperature e stelle di diversa massa sono capaci di raggiungere diverse temperature interne. Allo stesso tempo masse distinte significano fasi evolutive diverse a parità di età delle stelle. Queste constatazioni ci conducono a poter considerare le abbondanze relative degli elementi tra stella e stella come una fondamentale fonte di informazione per comprendere la natura e l'origine delle popolazioni stellari multiple negli ammassi globulari. Le abbondanze relative degli elementi, in particolare quelli leggeri, sono indizio dell'esistenza di popolazioni stellari differenti all'interno di un singolo ammasso (attraverso gli effetti che questi elementi hanno sullo spettro delle singole stelle) e allo stesso tempo gettano luce sui processi che portano a tali variazioni. \\

\textcite{Gratton2019}, sintetizza uno scenario che gode di solide basi e consenso nella comunità scientifica: la presenza di anticorrelazioni tra gli elementi leggeri come quelle N-C, Na-O, Al-Mg possono essere lette come il frutto di reazioni di cattura protonica nella fase di bruciamento del carbonio in sequenza principale (MS) ad alta temperatura\footnote{Se la trasformazione di C in N si attiva dalla temperatura di $10x10^6K$ bisogna superare i $70x10^6K$ per consentire la formazione di Al dal Mg}, quindi in stelle molto massicce, già arrivate alla fine del loro ciclo di vita, che hanno fornito, espellendolo attraverso venti stellari, il materiale processato per una nuova generazione di stelle. Le anticorrelazioni tra gli elementi leggeri sarebbero quindi una semplice manifestazione delle popolazioni multiple. \\

Questo scenario di formazione delle anticorrelazioni spiegherebbe alcuni consolidati risultati osservativi presenti in letteratura ricordati in \textcite{Gratton2019}:
\begin{itemize}
	\item C e N sono anticorrelati nei GCs ma allo stesso tempo C+N cresce al decrescere di C.
	\item Na-Al si comporta come l'anticorrelazione Na-O e la somma Al+Mg non varia in molti GCs.
	\item Nei casi in cui Mg+Al non è costante, lo è la somma Mg+Al+Si.
	\item Anche per elementi pesanti come K e Sc possono essere trovate variazioni delle abbondanze.
	%\item Non vi è corrispondenza tra le anticorrelazioni osservate e la temperatura di condensazione in grani o la sensibilità alla pressione di radiazione e alla sedimentazione che potrebbero avere effetto sulla composizione chimica delle stelle di MS. 
\end{itemize}

Altre anomalie chimiche che vanno ricordate sono:
\begin{itemize}
	\item In alcuni ammassi \textit{anomali} (detti Tipo II, \textcite{milone_2017}) sono riscontrabili significative variazioni in metallicità.
	\item Le popolazioni di seconda generazione sono arricchite in elio rispetto a quelle di prima che presentano l'abbondanza primordiale (Y$\sim$0.25). In alcuni casi il contenuto di elio di alcune stelle di seconda generazione raggiunge valori superiori a Y$\sim$0.40 (e.g. \textcite{ Zennaro2019}).
	
\end{itemize}

\cite{milone_2019} ha riassunto in 13 proprietà delle popolazioni multiple nei GCs i principali risultati ottenuti nell'ultimo decennio di intenso studio di questo così classico eppure così innovativo terreno. In particolare utilizzando mappe cromosomiche (ChMs) e fotometria HST\footnote{Delle tecniche diremo meglio nelle prossime sezioni}.
\begin{enumerate}
	\item Gli ammassi globulari studiati tramite fotometria HST e l'uso delle ChMs presentano solitamente due popolazioni discrete 1G e 2G \footnote{prima e seconda popolazione o prima e seconda generazione; 1G e 2G.} con, in alcuni casi, delle sub-popolazioni.
	\item Le popolazioni multiple sono una caratteristica comune degli ammassi globulari galattici e riscontrabili anche in ammassi delle Nubi di Magellano, di Fornax e nel GC G1 di M31. Solo pochi ammassi sembrano essere composti di un'unica popolazione stellare, sono normalmente quelli meno massicci. 
	\item Le stelle di seconda generazione sono presenti in tutti i GCs mentre sono rare nel campo galattico. 
	\item La frazione di stelle di 2G varia enormemente tra un GC e l'altro (dal 35\% di M71 al 90\% di $\omega Cen$), così come il numero di sub-popolazioni e la frazione in massa di elio che presenta fino a $\Delta Y_{max} \sim 0.18$.
	\item Esistono due classi di amassi globulari. La prima, Type I, mostra singole sequenze di stelle di prima e seconda generazione; la seconda, Type II, mostra nelle ChMs sequenze multiple di stelle di 1G e 2G, oltre ad uno split in SGBs nei diagrammi CMD costruiti con fotometria in bande ottiche. Gli ammassi di Type II coincidono con gli ammassi \textit{anomali}, di cui abbiamo accennato anche sopra, dotati di una variabilità interna degli elementi pesanti oltre a quelli leggeri.
	\item Le stelle 2G sono arricchite in He, N, Na e impoverite in C e O in confronto alle stelle 1G che presentano una composizione chimica come quella dell'alone galattico con la medesima metallicità. In alcuni casi le anticorrelazioni proseguono ad elementi successivi della catena di reazioni per cattura protonica. Le stelle 2G mostrano, quindi, la composizione chimica frutto del ciclo CNO e dei processi di cattura protonica ad alte temperature.
	\item La scoperta delle popolazioni multiple lungo i CMD ha fornito un nuovo punto di osservazione per stimare il contenuto in Elio delle popolazioni stellari. Infatti il contenuto in Elio è molto difficile da determinare tramite linee spettrali, mentre attraverso la fotometria multi-banda di HST è stato possibile stimare con buona precisione il contenuto in tale elemento di sessanta ammassi, che presentano variazioni che vanno da $\Delta Y_{max}< 0.01$ a $\Delta Y_{max} \sim 0.18$.
	\item Negli ammassi Type I le stelle di 1G e 2G presentano metallicità pressoché costante. Ciò esclude che l'origine dell'arricchimento delle stelle 2G sia dovuto a supernove. Gli ammassi Type II come $\omega Cen$ presentano invece variazioni in metallicità che possono essere spiegate ammettendo che anche soltanto il 2\% del ferro espulso da una supernova di tipo I venga trattenuto dalle stelle 2G. 
	\item In alcuni ammassi le stelle 2G sono maggiormente concentrate al centro rispetto alle 1G, mentre in altri casi le due popolazioni condividono la medesima distribuzione radiale. 
	\item Recenti lavori basati sui moti propri ad alta precisione ottenibili da immagini HST di epoche diverse e sulla \textit{Data Release 2} di Gaia hanno mostrato come le stelle 2G degli ammassi più massicci presentino una distribuzione radiale delle velocità più anisotropica che le stelle 1G. 
	\item La frazione di stelle 2G e il massimo della variazione interna in He e N, correlano tutte fortemente con la massa attuale ed iniziale dell'ammasso. 
	\item Ammassi con un grande raggio perigalattico presentano una frazione di stelle 1G maggiore, in media, degli ammassi più vicini al centro galattico. Ciò suggerisce che l'interazione con la galassia influenzi l'attuale rapporto 1G/2G.
	\item Alcuni studi hanno mostrato come il numero relativo di stelle nelle distinte popolazioni stellari sia costante in ampi range di massa. 
\end{enumerate}

\section{Tecniche di analisi e individuazione delle popolazioni}

Le proprietà delle popolazioni multiple derivanti dalle osservazioni riassunte nella sezione precedente, fanno comprendere come la corretta catalogazione di una stella tra le varie popolazioni (population tagging) che compongono l'ammasso sia di primaria importanza per la comprensione degli scenari di formazione ed evoluzione degli ammassi globulari.\\
Svolgere al meglio questo compito significa individuare adeguati \textit{spazi dei parametri} osservativi, in cui differenti popolazioni appaiano sufficientemente distinguibili le une dalle altre, ovvero spazi in cui la distanza fra le popolazioni sia massima.\\
A questo scopo sono state sviluppate negli anni numerose tecniche osservative e di riduzione dati. Sebbene la spettrometria mantenga una fondamentale importanza per lo studio dettagliato delle abbondanze chimiche, via via hanno preso più piede tecniche fotometriche multi-banda, che possono essere immaginate come una spettrometria a bassa risoluzione. Tale metodo ha il vantaggio di dare accesso contemporaneo ad un campione molto più vasto di stelle (quindi con una statistica ben più robusta) in tempi osservativi molto più brevi\footnote{ o per studiare stelle molto più deboli intrinsecamente o per la distanza (come per gli ammassi nelle MCs)} e potendo maneggiare anche le regioni più affollate ubicate nei pressi del centro degli ammassi. Le tecniche fotometriche necessitano però di una particolare cura nella scelta delle bande di osservazione e nell'interpretazione e riduzione delle immagini. Ulteriori miglioramenti sembrano possibili: ne parleremo in seguito presentando i lavori di Jae-Woo Lee. Va però ribadito come alcune di queste tecniche stiano rappresentando un radicale cambio di passo nella possibilità di studio delle popolazioni multiple negli ammassi globulari. \\

Tra queste tecniche un posto d'onore lo occupa sicuramente la fotometria in UV. \\
Seminale lo studio di M4 di \textcite{Marino2008}, nel quale è stato mostrato come stelle di prima e seconda generazione possono essere distinte in due diversi rami delle giganti rosse (RGBs) costruendo un diagramma colore magnitudine \textit{B} vs \textit{U-B}. Il filtro U include infatti le bande molecolari del CN e NH che come abbiamo ricordato precedentemente sono rafforzate nelle stelle 2G, determinando magnitudini più deboli per le stelle 2G rispetto alle 1G.\\
L'utilizzo delle bande nell'ultravioletto ha trovato poi estensione nell'utilizzo di bande di Hubble Space Telescope con analoghi colori come  ($m_{F366W}-m_{F438W}$) e ($m_{F3343N}-m_{F438W}$) o lo pseudo colore derivante dalla somma $((m_{F366W}-m_{F438W})+(m_{F3343N}-m_{F438W}))$ e nella combinazione dei colori \textit{U-B} \textit{B-I} e con gli analoghi HST per la costruzione di diagrammi a due colori sensibili sia alle variazioni di azoto che di elio come B vs (U-B+I) o B vs $C_{U,B,I}=(U-B)-(B-I)$ \parencite{Monelli2013,Milone2013}, quest'ultimo indice rivelatosi molto efficace per identificare sequenze multiple lungo RGB. \\
In questo quadro si inserisce l'utilizzo del terzetto di filtri HST detto \textit{the magic trio}, normalmente composto dei filtri F275W, F336W e F348W\footnote{spesso uno o più filtri del terzetto possono essere sostituiti rispettivamente da F225W, F343N e F410M} il quale presenta particolare efficacia nel distinguere differenti popolazioni in quanto la banda passante del filtro F225W include le bande molecolari di OH e NH, mentre F438W quelle di CN e CH e questi filtri possono essere utilizzati per costruire i diagrammi a due colori $((m_{F366W}-m_{F438W})vs(m_{F275W}-m_{F336W}))$. Inoltre è stato definito l'indice $C_{F275W,F336W,F438W}=(m_{F275W}-m_{F336W})-(m_{F336W}-m_{F438W})$ sulla falsariga di $C_{U,B,I}$, che consente di identificare le multiple popolazioni lungo l'intero CMD \parencite{milone_2019}.\\

Sempre sulla base della fotometria HST sono state introdotte le già citate mappe cromosomiche (ChMs) \parencite{Milone2015II}, ovvero digrammi a due pseudo-colori, dei rami di sequenza principale (MS), delle giganti rosse (RGB) o delle giganti asintotiche (AGB), costruiti con filtri sensibili alla specifica composizione chimica dei GCs \parencite{milone_2019}. Solitamente sono usati il magic trio più F814W.
Tali diagrammi sono ottenuti attraverso la rettificazione degli indici di colore del tipo prima elencato: ad esempio si parte da diagrammi come $m_{F814W}$ vs $m_{F275W}-m_{F814W}$ e $m_{F814W}$ vs $C_{F275W,F336W,F438W}$ sui quali si costruiscono delle fiducial line. Misurando le distanze in colore (ovvero lungo ascissa) da queste linee, gli indici di variazione così ottenuti, nel medesimo esempio $\Delta Y(F275W,F336W,F438W)$ e $\Delta X(F275W,F814W)$ sono quindi messi in relazione in un diagramma, le mappe cromosomiche, appunto. In figura \ref{Figure:ChMapMilone} è riassunta la procedura appena presentata che dà origine ad uno strumento che massimizza le informazioni sulle differenze in composizione chimica.\\

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{Figure/Milone2015II.png}
	\caption{\textcite{Milone2015II}, nel pannello (d) troviamo la Chromosome Map in cui si possoo distinguere 3 popolazioni A,B,C per il RGB di NGC 7089}\label{Figure:ChMapMilone}
\end{figure} 

La frequenza di stelle in diverse popolazioni può quindi ora essere stimata con una statistica molto migliore di quella possibile tramite spettrometria proprio grazie alla fotometria HST, che presenta però anche alcuni svantaggi di cui diremo all'\ref{sec:grandetelescopio}. 

%Non si tratta però di una determinazione diretta delle abbondanze, ma piuttosto di un'etichettatura qualitativa basata su indici che possono essere determinati con precisione per un grande campione di stelle. Questo introduce però un certo grado arbitrarietà che può condurre a risultati alquanto differenti (\cite{Gratton2019}): piccole differenze nei filtri o nelle procedure possono condurre ad ampie variazioni nelle stime della frazione di stelle 1G e 2G. Allo stesso modo \cite{Lee_2017} ha sottolineato una certa difficoltà di interpretazione del magic trio che misura contemporaneamente OH, NH, CN, CH  e Mg; accentuata dal fatto che è atteso un effetto di luminosità positivo per il CN e negativo per OH, NH e CH. Ciò può condurre a problemi interpretativi e difficoltà nel assegnare con precisione una stella all'una o all'altra popolazione, che è oggi il fondamentale obbiettivo per la comprensione degli scenari di formazione ed evoluzione dei GC.

\section{Una misura precisa del CN}\label{sec:CneLee}

Negli studi spettrometrici che hanno segnalato le anomalie delle abbondanze chimiche già nel passato come \textcite{Norris1981AbundanceSI} e più recentemente \textcite{Smith2009} è stato utilizzato l'indice $$S(3839)=-2.5\log_{10}(\frac{F_{CN}}{F_{comp}})=-2.5\log_{10}[\int_{3846}^{3883}I_{\lambda}d\lambda/\int_{3883}^{3916}I_{\lambda}d\lambda]$$
che compara il flusso nella regione della banda di assorbimento del CN tra $3846\AA$ e $3883\AA$ con il flusso in una regione di continuo adiacente. \\

A partire da tale indice, e per affrontare le problematiche presentate alla fine della sezione precedente, \textcite{Lee_2017} ha introdotto un set di filtri capace di selezionare la banda di assorbimento del CN a $\lambda 3883$ e definito un indice $Cn_{JWL}=JWL39-Ca_{new}$ per misurare la forza di assorbimento esclusivamente di questa banda, avvantaggiandosi anche del fatto che nella banda passante di JWL39 l'estinzione atmosferica non varia in maniera significativa. Nelle figure \ref{figure:filtJWL} e \ref{figure:confjwl} sono riprodotti alcuni diagrammi di \textcite{Lee_2017} che danno conto della correlazione esistente fra il nuovo indice fotometrico e l'indice spettrometrico S(3839) e della sua ottima capacità di separare distinte popolazioni stellari. \\
\begin{figure}\label{Figure:FiltriLee17}
	\centering
	\includegraphics[width=0.6\textwidth]{Figure/FiltriLee17.png}
	\caption{\textcite{Lee_2017}, curva di trasmissione dei filtri utilizzati da Lee per l'indice $Cn_{JWL}$}
\end{figure} 

\section{Strumenti a grande campo da terra}\label{sec:grandetelescopio}

Questa combinazione di filtri estende in maniera significativa la possibilità di studio delle popolazioni multiple con strumenti da terra. Come abbiamo visto la maggior parte degli studi recenti più significativi attraverso la fotometria sono stati possibili grazie alle bande fotometriche di HST. Il telescopio spaziale è capace di fornire immagini di incredibile pregio, anche se con alcune peculiarità:
\begin{itemize}
	\item la difficoltà di accesso allo strumento e di ottenere tempo telescopio, sia per l'altissimo costo ($\sim100k\$$ per una singola orbita) sia per la forte competizione;
	\item il ridotto campo di vista che arriva al massimo, per WFC3-UVIS, a $162"$x$162"$ (pari a $\sim4.4arcmin^2$), che rende impossibile studiare gli ammassi per intero o le regioni esterne, spesso molto rilevanti ai fini scientifici;
	\item l'impossibilità di introdurre nuove bande osservative;
	\item la probabile prossima, anche se indeterminata, conclusione della missione essendo diventata impossibile la manutenzione.
\end{itemize}

\textcite{Lee_2015} e \textcite{Lee_2017} hanno fornito sorprendenti risultati con un telescopio terrestre a grande campo, di ridottissime dimensioni (0.9m), attraverso un'attenta scelta dei filtri\footnote{Ed anche l'utilizzo di immagini di archivio HST per la costruzione di migliori cataloghi nelle zone più crowded dell'ammasso}. Tali risultati fanno intendere la possibilità di significativi sviluppi nelle osservazioni da terra, con telescopi di dimensioni più generose, a grande campo. \\
In attesa di sviluppi dell'ottica adattiva per ampi campi di vista, il vantaggio di uno strumento di maggiori dimensioni è sicuramente quello di ridurre i tempi di osservazione anche con filtri molto stretti e, potenzialmente, ottenere una maggiore precisione fotometrica, aumentando le possibilità di studio di ammassi lontani, o attenuati, o delle parti più deboli del CMD. \\
Lo studio tramite strumenti a grande campo è invece fondamentale per ampliare la statistica e soprattutto per poter misurare coerentemente l'eventuale presenza di un gradiente radiale nel rapporto fra popolazioni. \\

I filtri di Lee che abbiamo descritto nella sezione precedente, come tutti i narrow-bandpass, sono filtri costruiti tramite il fenomeno dell'interferenza. Si tratta di filtri interferenziali le cu proprietà spettrali dipendono dalla collocazione in un particolare sistema ottico. Il posizionamento in una zona di fascio parallelo o convergente e, in generale, gli angoli con cui la radiazione colpisce il filtro ne ridefiniscono la curva di trasmissione rispetto a quella nominale. In particolare questo è significativo quando abbiamo a che fare con rapporti focali molto veloci come quelli che caratterizzano normalmente gli strumenti a grande campo.\\

Studiare il comportamento dei filtri interferenziali all'interno di strumenti con una focale veloce e in presenza di angoli non-telecentrici significativi è il cuore di questo lavoro di tesi. Presenteremo questo tipo di filtri e delle configurazioni ottiche problematiche nel capitolo \ref{chap:optical} ed eseguiremo uno studio dettagliato delle risposte dei filtri in presenza di differenti rapporti focali e differenti angoli non-telecentrici nel capitolo \ref{Chap:Numerical}. Nel capitolo \ref{chap:casi} useremo quanto sviluppato in precedenza per applicare ad un concreto studio di fattibilità ciò che abbiamo presentato nel corrente capitolo: verificheremo come si potrebbe comportare l'indice $Cn_{JWL}$ costruendo dei filtri equivalenti al $JWL39$ e $Ca_{new}$ per lo strumento LBC-B installato al primo fuoco del Large Binocular Telescope, $8.4m$ di apertura, con $\sim30arcmin$ di diametro (pari a $\sim707arcmin^2$) del campo di vista, traendo conclusioni rassicuranti per questo caso specifico purché si tengano in considerazione i risultati medesimi in fase di progettazione e riduzione dati. 

==> TeX_files/OpticalIssue.tex <==
\chapter[Problematiche ottiche]{Le problematiche ottiche}\label{chap:optical}

%\input{FilterImage}

\begin{figure}\label{figure:filtro e angolo} \caption{Gli effetti di un filtro interferenziale, una certa banda (stretta) è trasmessa mentre il resto dello spettro è riflesso. All'aumentare della distanza dalla normale la $\lambda$ centrale filtrata si sposta verso lunghezze d'onda minori.}
	\centering
	\input{./TeX_files/Immaginefiltro2}
\end{figure}
%\input{./TeX_files/Immaginefiltro2}



%\begin{itemize}
%	\item Filtro F-P, ricavare formule su trasmissione e sensibilità angolo \ref{math:lambdatheta}
%	\item film strati sottili $\lambda/4$ $\rightarrow$ filtro all-dielectric tipo HLHLHLSHLHLHL, seguengo \cite{Lissberger:59I} o \cite{macleod2010thin}
%	\item Presentare un po' di risultati sui filtri da \cite{macleod2010thin}
%	\item Posizionamento dei filtri nel telescopio, fascio convergente o fascio parallelo (perché non è la soluzione)
%	\item L'angolo non-telecentrico
%	\item Esigenze sul campo di vista
%\end{itemize}

Nel presente lavoro di tesi ci occuperemo soprattutto di caratterizzare la risposta di un filtro interferenziale in uno strumento ottico dalla focale veloce. Per farlo studieremo nel dettaglio il comportamento di un filtro interferenziale quando è investito da un fascio di luce convergente. \\
In questo capitolo ci limiteremo a presentare i risultati fondamentali riguardo ai filtri interferenziali, le problematiche che derivano dalla fisica di tali filtri e le proprietà che vanno tenute in considerazione per i nostri scopi. \\
Come vedremo la curva di trasmissione di un filtro interferenziale non è sempre uguale a quella nominale, bensì essa cambia relativamente all'angolo con cui la radiazione colpisce la superficie del filtro: nel caso di un fascio convergente questo significa che sezioni differenti del fascio proveniente da una medesima sorgente (giungono con differenti angoli sul filtro) trovano davanti a sé un filtro le cui proprietà sono leggermente differenti\footnote{Vedremo questo aspetto più nel dettaglio nel prossimo capitolo \ref{Chap:Numerical} dove definiremo anche delle superfici isofiltranti pr scopi operativi, utili però anche per sviluppare intuizione sul fenomeno}. L'effetto di selezione delle lunghezze d'onda sarà diverso da quello stabilito nominalmente e misurato per un fascio parallelo con direzione di propagazione normale al piano del filtro.\\
Partiamo dalla definizione di un filtro interferenziale alla Fabry-Perot, spiegandone il funzionamento e ricavandone la risposta all'angolo di incidenza; vedremo poi a grandi linee come è costruito un moderno filtro interferenziale a strati sottili. Nell'ultima sezione di questo capitolo vedremo invece la rilevanza dell'angolo non-telecentrico nell'insorgere di una potenziale aberrazione differenziale all'interno del campo di vista che indagheremo nei capitoli seguenti. 

\section[Filtro Interferenziale F-P]{Filtri interferenziali a la Fabry-Perot}

La configurazione più semplice per ottenere un filtro interferenziale è quella usata Charles Fabry e Alfred Perot sul finire del diciannovesimo secolo per costruire il loro interferometro. Costituito da due superfici identiche parzialmente riflettenti parallele come in figura \ref{Figure:FP1}. \\

\begin{figure}
	\centering
	\begin{tikzpicture}[>=stealth]
	\draw(0,0)--(0,6);
	\draw (2,0)--(2,6);
	
	\draw[<->,dashed] (0,5)--(2,5) node[above,midway]{d};
	
	\draw[->] (-4,3) -- (-0.2,3)  node[above,midway]{$E_{in}$};
	\draw[->] (2.2,3) -- (6,3)  node[above,midway]{$E_{out}$};
	
	\node(a) at (1,-1) {superfici semi-riflettenti};
	\fill[red] (a.north) circle (1pt);
	
	\draw [->] (0,3) node[above right]{$E_{in}t$} to[bend left=30] (2,3) ;
	\draw [->] (2,3) node[below left]{$E_{in}tr$} to[bend left=30] (0,3) ;
	
	\draw [->,dashed] (a.north) to[bend left=15] (2,1);
	\draw [->,dashed] (a.north) to[bend right=15] (0,1);
	
	\end{tikzpicture}
	\caption{Superfici semi-riflettenti affacciate come nell'interferometro di Fabry-Perot. La radiazione incidente viene in parte trasmessa e in parte riflessa.} \label{Figure:FP1}
\end{figure}

Consideriamo una radiazione e.m., con un campo elettrico associato $E_{in}$ che si propaga con direzione perpendicolare alle due superfici. Dove queste presentano un coefficiente di trasmissione $T=t^2$, dove $t$ è il coefficiente di trasmissione dell'ampiezza d'onda. L'ampiezza del campo appena dopo il primo specchio sarà pari a $E_{in}t$ e, appena attraversata anche la seconda superficie riflettente, avremo un ampiezza pari a $$E_{out}^{(0)}=E_{in}t^2e^{i\frac{\phi}{2}} \label{eq:fp1}$$ dove $\phi=\frac{2d}{\lambda}2\pi$ rappresenta lo sfasamento intercorso nella propagazione. Esso è pari al doppio della separazione degli specchi, ovvero pari al tragitto di andata e ritorno tra i due. $\phi$ è detto talvolta \textit{roundtrip phase}. La radiazione che non viene trasmessa dalla seconda superficie viene riflessa verso la prima che a sua volta la riflette nuovamente sempre con il coefficiente $R=r^2=1-T$. Dopo queste due prime riflessioni $(E_{in}te^{i\frac{\phi}{2}})rre^{i\phi}$ avremo una ulteriore trasmissione per cui $$E_{out}^{(1)}=t^2E_{in}e^{i\frac{\phi}{2}}r^2e^{i\phi}=E_{out}^{(0)}r^2e^{i\phi}$$
si può proseguire iterativamente e considerare che le ampiezze si sommano 
\begin{equation}\label{eq:fp2}
\frac{E_{out}}{E_{in}}=t^2e^{i\frac{\phi}{2}}(1+r^2e^{i\phi}+(r^2e^{i\phi})^2+(r^2e^{i\phi})^3+...)
\end{equation}
dato che $r^2<1$ la serie converge e la \ref{eq:fp2} diviene 
\begin{equation}\label{eq:fp3}
	\frac{E_{out}}{E_{in}}=\frac{t^2e^{i\frac{\phi}{2}}}{1-r^2e^{i\phi}}=\frac{(1-R)e^{i\frac{\phi}{2}}}{1-Re^{i\phi}}
\end{equation}
per cui si ha il massimo della trasmissione 
\begin{equation}
	\left(\frac{E_{out}}{E_{in}}\right)_{max}=\frac{1-R}{1-R}=1
\end{equation}

quando due volte la distanza fra le due superfici riflettenti è pari ad un multiplo della lunghezza d'onda della radiazione elettromagnetica. In altre parole quando abbiamo a che fare con onde stazionarie tra le due superfici l'intensità della radiazione trasmessa è pari al 100\% di quella incidente.
\begin{equation}\label{eq:fbphi}
	\phi=n2\pi \Rightarrow \lambda=\frac{2d}{n}
\end{equation}
Viceversa per $\phi=n2\pi+\pi$ si ha il minimo della trasmissione pari a $(\frac{E_{out}}{E_{in}})_{min}=\frac{1-R}{1+R}$. Tale minimo dipende da $R$ così che quanto più la riflettività si avvicina a 1 tanto più il minimo della trasmissione è vicino a 0. Si tratta di un tipico effetto di interferenza che può essere utilizzato per ottenere una spettrometria ad alta risoluzione, se il sistema è costruito per consentire la variazione della distanza tra gli specchi, o, più semplicemente, per ottenere un filtro con una banda stretta (che dipende da R). \\ Quest'ultima è la configurazione che ci interessa e che costituisce il punto di partenza per la progettazione dei moderni filtri interferenziali a strati sottili. \\

Finora abbiamo mostrato solo il caso particolare in cui la radiazione incide perpendicolarmente agli specchi. Rimane da trovare la relazione tra la lunghezza d'onda, che massimizza la trasmissione, e l'angolo con cui la radiazione incide sull'interferometro così costituito. In figura \ref{Figure:FP2} la radiazione incide con angolo $\theta$ rispetto alla normale: si vede immediatamente che il cammino ottico all'interno della coppia di specchi (e quindi lo sfasamento ai bordi) cambia con l'angolo medesimo. Ci poniamo qui nell'approssimazione di considerare $d$ molto piccolo (dello stesso ordine di $\lambda$) così che la separazione fra i fasci successivi $t',t'',...$ sia tale da garantire l'interferenza. Differentemente bisognerebbe porre una lente convergente per riportare i fasci frutto delle riflessioni successive in condizione di interferenza\footnote{Che è proprio la configurazione di un interferometro F-P classico}.


\begin{figure}
	\centering
	\begin{tikzpicture}[>=stealth]
	
		%%NORMALE
	\draw[dash dot,very thin] (-4,3) to (6,3);
	\coordinate (a) at (-4,2); \coordinate (b) at (0,3); \coordinate (c) at (-4,3); 
	\pic[draw,"$\theta$", draw=orange,<->,angle eccentricity=1.3,angle radius=3.5cm]{angle=c--b--a};
	
	\draw(0,0)--(0,6);
	\draw (2,0)--(2,6);
	
	\draw[<->,dotted] (0,1)--(2,1) node[above,midway]{d};
	
	\draw[->,thick] (-4,2) -- (0,3) node[above,midway]{$I_{in}$};
	\draw[dashed] (0,3) to (2,3.5);
	\draw[dashed] (2,3.5) to (0,4);
	\draw[dashed] (0,4) to (2,4.5);
	\draw[dashed] (2,4.5) to (0,5);
	\draw[dashed] (0,5) to (2,5.5);
	\draw[dashed] (2,5.5) to (1,5.75);
	
	
	\draw[->] (2,4.5) -- (6,5.5) node[above,midway]{$t''$} node[above]{$I_{t}$};
	\draw[->,dashed] (2,3.5) -- (6,4.5)  node[above,midway]{$t'$};
	\draw[->,dashed] (2,5.5) -- (6,6.5) node[above,midway]{$t'''$};
	
	\draw[->,dashed] (0,3) -- (-4,4) node[above,midway]{$r'$};
	\draw[->] (0,4) -- (-4,5) node[above,midway]{$r''$} node[above]{$I_{r}$};
	\draw[->,dashed] (0,5) -- (-4,6) node[above,midway]{$r'''$};
	
	\draw[dashed] (2,4.5) --(2.5,2.5);
	\draw[red] (2,3.5) to (2.23,3.555);
	
	\node[below left, red] at (0,3) {A};
	\node[below left, red] at (2,3.5) {B};
	\node[below left, red] at (0,4) {C};
	\node[below left, red] at (2,4.5) {D};
	\node[below right, red] at (2.23,3.555) {E};
	\end{tikzpicture}
	\caption{fascio luminoso che incide non perpendicolarmente ad una coppia di specchi a la Fabry-Perot} \label{Figure:FP2}
\end{figure}

Come si vede in figura \ref{Figure:FP2} la differenza in cammino ottico fra $t'$ e $t''$ non è più pari semplicemente a $2d$ bensì

\begin{equation}
	\begin{array}{l}
		t': AB+BE \\
		t'':AB+BC+CD=3AB\\
		\Delta_{t''-t'}=2AB-BE
	\end{array}
\end{equation}

dato che $AB=\frac{d}{\cos\theta}$ e $$BE=BD\sin\theta=2AB\sin\theta=2d\frac{\sin^2\theta}{\cos\theta}$$ allora

\begin{equation}\label{eq:FPtheta}
\Delta=2d\cos\theta
\end{equation}

contrariamente a quello che potrebbe far crede l'intuizione all'aumentare dell'angolo la differenza in cammino ottico si riduce, come se le due superfici si avvicinassero l'una all'altra. Ricordando la \ref{eq:fbphi} la relazione fra angolo di incidenza e lunghezza d'onda corrispondente al massimo della trasmissione (all'ordine n-esimo) è
\begin{equation}
	\lambda=\frac{2d\cos\theta}{n}
\end{equation}

La presenza di una distanza angolare dalla normale sposta verso le lunghezze d'onda più blu la banda del filtro.\\

Con ragionamenti del tutto simili ma considerando una lamina sottile\footnote{o comunque un materiale di separazione con indice di rifrazione diverso da quello del mezzo esterno ai due specchi}, con indice di rifrazione $\mu_f$, e una interferenza dovuta a più fasci coerenti si ottiene
\begin{equation}\label{eq:FPDeltathl}
	\Delta=2\mu_f d\cos\theta
\end{equation}
e per l'intensità trasmessa $$I_t=I_i\textit{A}(\theta)$$ dove la $\textit{A}(\theta)$ è la funzione di Airy $\textit{A}(\theta)=\frac{1}{1+F\sin^2(\phi/2)}$ dove $F\equiv(\frac{2r}{1-r^2})^2$ è detto coefficiente di finesse e determina quanto è stretta la banda di trasmissione. Si può consultare \textcite{Hecht} per il dettaglio di questi ultimi risultati.

\section{Filtri All-dielectric}\label{sec:alldielectric}

Nella trattazione della sezione precedente abbiamo omesso sia la difficoltà costruttiva di due superfici perfettamente piane sia l'assorbimento delle superfici riflettenti, il quale può essere significativo. Va inoltre sottolineato che uno strumento costruito con due semplici superfici come l'interferometro di Fabry-Perot lascia un solo parametro libero per determinare la larghezza di banda del filtro e non consente di modificarne la forma. In particolare per ottenere filtri \textit{edge} e filtri passa-banda ben definiti è fondamentale espandere le superfici riflettenti in una pila di strati sottili dielettrici trasparenti e a basso assorbimento.\\
Questi filtri assumono numerosissime configurazioni differenti: presentiamo qui la più classica e flessibile. Un filtro \textit{all-dieletrics} si compone di una pila di dielettrici di spessore $\lambda/4$ di indice di rifrazione di valori alternati, una cavità risonante centrale, e un'altra pila simmetrica alla prima. In figura \ref{figure:HL}, è schematizzato un filtro interferenziale di questo tipo, che funziona anche da mattone costitutivo di filtri più complessi con due o tre cavità.

\begin{figure}
	\centering
	\begin{tikzpicture}
	\foreach \x in {0.,0.4,0.8,1.2,1.6}	{	
		\draw (0,0+\x) node[left]{\tiny H} rectangle (8,.2+\x);
		\draw[fill=black!25] (0.1,.2+\x)node[left]{\tiny L} rectangle (7.9,.4+\x);}
	\draw[fill=black!5](0,2) rectangle (8,2.4) ;
	\foreach \x in {0.,0.4,0.8,1.2,1.6}	{	
		\draw (0,2.6+\x) node[left]{\tiny H}  rectangle (8,2.8+\x);
		\draw[fill=black!25] (0.1,2.4+\x)node[left]{\tiny L} rectangle (7.9,2.6+\x);}
	
	\draw[->] (7,-1.25) node[left]{\footnotesize $\lambda/2$ spacer} to[bend right=40] (8,2.2);
	\draw (0,-1) rectangle (0.5,-1.5) node[above right]{\footnotesize $\lambda/4$ alto indice};
	\draw[fill=black!25] (0,-2.) rectangle (0.5,-2.5) node[above right]{\footnotesize $\lambda/4$ basso indice};
	\end{tikzpicture}
	\caption{Filtro all-dieletrics}\label{figure:HL}
\end{figure}

Il calcolo della banda passante per un filtro così costruito prende le mosse da una serie di passaggi simili a quelli che conducono alla \ref{eq:FPDeltathl}, considerando lo spessore $\lambda/4$ e che riflessioni su interfacce da indice di rifrazione minore a maggiore comportano un cambiamento di fase $\pi$ mentre su interfacce da indice maggiore a minore non si ha cambiamento di fase\footnote{avevamo trascurato questo aspetto nella trattazione precedente perché in trasmissione tra sole due superfici le riflessioni sono sempre in numero pari}. Una teoria degli strati sottili con una trattazione completa dell'argomento e il suo svolgimento analitico-computazionale, che va oltre gli scopi del presente lavoro, si trova esposta in gran dettaglio nel \textcite{macleod2010thin} che inoltre contiene molti dati sperimentali e tecnico-industriali per la costruzione, il calcolo e la comprensione della teoria degli strati sottili sia per quanto riguarda i più semplici coating antiriflesso a singolo strato, sia per i filtri più complessi. \\
La prima trattazione analitica adeguata a considerare questo tipo di filtro anche con luce non perfettamente perpendicolare si deve ad una serie di lavori di P. H. Lissberger a cavallo del 1960, in particolare \textcite{Lissberger:59I,Lissberger:59II}. In questi lavori Lissberger ha stabilito l'equivalenza di un filtro interferenziale all-dielectric con con un sistema a singolo strato (lo spacer) con riflettività calcolabile e con curva di trasmissione pari alla nota forma di Airy. Così si ottiene la lunghezza d'onda di massima trasmissione $\lambda$ da $$2\mu_* d\cos\theta_*=n\lambda$$ dove $\mu_*$ è indice di rifrazione efficace che prende valore intermedio fra quello degli strati H e quello degli strati L. Da qui si ricava la \ref{math:lambdatheta} considerando $\theta_f$ l'angolo di propagazione all'interno del filtro equivalente, quindi per la legge di Snell da cui, se l'indice di rifrazione all'esterno del filtro è pari a 1, $\sin\theta_*=\frac{\sin\theta}{\mu_*}$.

\section{Fascio convergente}

In uno strumento ottico per telescopi i filtri sono frequentemente collocati in una ruota porta filtri nei pressi del piano focale, quindi in una zona di fascio convergente. Un fascio parallelo di radiazione e.m. proveniente da un'unica sorgente, che quindi incide sul telescopio con un unico angolo, nella zona di fascio convergente viene trasformata in un cono che scansiona tutti gli angoli compresi fra quello del raggio principale ed uno estremo, dei raggi marginali, determinato dal rapporto focale. Raffigurandoci varie piccole sotto-aperture della pupilla di ingresso  possiamo notare come ognuna di esse lascia sul filtro una propria impronta che arriva con angolo differente a seconda della posizione nella pupilla. Per quanto detto nelle sezioni precedenti ognuna di queste sotto-aperture viene quindi filtrata in maniera leggermente differente. Mandando a zero la dimensione di queste sotto-aperture possiamo dire che ogni \textit{raggio} proveniente dalla stessa sorgente trova di fronte a sé un filtro con una curva di trasmissione differente. Sul piano focale troveremo quindi la radiazione risultante dalla somma, ovvero l'integrale, su ogni punto dell'intera pupilla: avremo quindi la somma di infinitesimi filtri leggermente differenti il cui risultato sarà in ogni caso, tanto o poco, differente dal filtro nominale la cui risposta in lunghezza d'onda è data per un fascio parallelo. \\
In \textcite{Lissberger:59II} si trova una prima trattazione analitica del problema di un fascio convergente con asse normale alla superficie del filtro, ovvero in configurazione telecentrica. 
Lissberger stabilisce a quanto equivale lo spostamento, verso lunghezze d'onda minori, della $\lambda$ centrale della banda passante, nell'approssimazione di angoli piccoli e di invarianza della curva di trasmissione. Per un fascio convergente di semiangolo $\alpha$, lo spostamento è pari alla metà di quello riscontrato per fascio parallelo che colpisca il filtro con angolo $\alpha$. Inoltre la larghezza a metà altezza della banda passante (FWHM) risulta, sotto le stesse ipotesi, proporzionale al quadrato dell'angolo di semi-apertura del fascio e inversamente al quadrato degli indici di rifrazione dei thin-layer.\\

Lissberger e Wilcock \parencite{Lissberger:59II} concludono che per F number non troppo veloci, maggiori di $F/3.3$ nella loro scelta di parametri\footnote{$\lambda_0=5000$, $n_*=2$ spaziatore di solfuro di zinco, $FWHM_0=50\AA$, e indice di rifrazione del solfuro di zinco a $5000\AA$ $\mu_z=2.39$}, il deterioramento delle performance del filtro è trascurabile. Anche per F number minori il deterioramento rimane di scarso rilievo qualora si tenga in considerazione lo spostamento della lunghezza d'onda centrale in fase di progettazione del filtro. Trovano, ad esempio, che per ottenere il massimo della trasmissione a $\lambda=5000\AA$ per un rapporto focale $F/2.0$ bisogna costruire un filtro con $\lambda_0=5020\AA$. Concludono inoltre che il deterioramento è maggiore per filtri più stretti. \\
Come vedremo nel capitolo \ref{Chap:Numerical}, ognuno di questi risultati è confermato dalle simulazioni numeriche e dalle valutazioni qualitative con le quali approfondiremo quanto espresso nella presente sezione. I limiti di un metodo analitico risiedono soprattutto nella difficoltà di trattare funzioni di trasmissione che non siano una funzione analitica facilmente integrabile, inoltre non hanno fin qui tenuto in considerazione un'altra fonte di deterioramento delle performance del filtro, molto rilevante in strumenti ottici per l'astronomia a grande campo: la presenza di un angolo non-telecentrico. \\ Per sorgenti non posizionate al centro del campo di vista (il cui fascio parallelo non arriva sulla pupilla di ingresso normalmente alla stessa) l'asse del cono convergente (il suo raggio principale) non è più normale al filtro. Non è sufficiente tenere in considerazione lo spostamento della banda passante in fase di progettazione per neutralizzare il deterioramento del filtro, poiché la presenza di angoli non-telecentrici determina una aberrazione differenziale all'interno del campo di vista: sorgenti a distanze differenti dal centro del campo vengono perciò filtrate in maniera differente. \\
\begin{figure}\label{figure:cone}
	\centering
	\input{./TeX_files/FilterCone}
	\caption{Fascio di luce parallelo viene trasformato in un fascio convergente dal telescopio. "Coni" di luce provenineti da stelle in posizioni differenti nel campo di vista presentano un raggio principale che incide il filtro con angoli differenti, tranne nel caso di un sistema telecentrico.}
\end{figure}

Si potrebbe supporre che per eliminare i problemi relativi al fascio convergente e all'angolo non-telecentrico sia quella di posizionare i filtri in una zona di fascio parallelo, magari in un reimaging della pupilla, cosa che peraltro avviene in alcuni strumenti, questo però non è affatto una soluzione. \\ 
L'invarianza di Lagrange ci dice infatti che il prodotto fra inclinazione e diametro del fascio è costante per cui $$\Theta D=\Theta' D'$$ ad un diametro più piccolo corrisponde un angolo più grande. Questo si traduce in un maggior spostamento della lunghezza d'onda centrale della curva di trasmissione del filtro, e differente per ogni sorgente, stante la necessità di costruire filtri molto più piccoli dell'apertura del telescopio\footnote{Non sarebbe così e fosse possibile costruire un filtro delle dimensioni dell'apertura del telescopio, per cui gli angoli di ingresso anche con un campo di vista grande rimangono tanto piccoli da non costituire un problema di deterioramento delle performance del filtro }.


\section{Angolo nel campo di vista e angolo non-telecentrico}

Per capire operativamente la possibilità di realizzare filtri interferenziali adatti alla caratterizzazione di popolazioni stellari multiple\footnote{lo faremo nel capitolo \ref{chap:casi}}, e in generale per comprendere l'impatto dell'aberrazione differenziale dovuta all'angolo non-telecentrico sulle nostre misure, dovremo conoscere la relazione tra la posizione nel campo di vista di una sorgente e l'angolo non-telecentrico. \\
Tale operazione è in via teorica molto semplice purché si conoscano alcune caratteristiche fondamentali degli strumenti ottici, risulta più complicato data la difficoltà di reperire alcune informazioni quale, ad esempio, la posizione della pupilla di uscita, non ricostruibile senza conoscere l'esatta configurazione ottica e allo stesso tempo quasi mai riportata negli articoli tecnico-scientifici relativi agli strumenti. Qui di seguito vediamo come calcolare la costante di proporzionalità tra distanza angolare dal centro del campo di vista e l'angolo non-telecentrico conoscendo i rapporti focali e la posizione della pupilla d'uscita. \\

\begin{figure}
	\centering
	\begin{tikzpicture}[scale=0.9]
	\draw[<->] (0,-3) to (0,3); %prima lente
	\draw[>-<] (7,-2.4) to (7,2.4); %seconda lente
	
	\draw[dash dot] (-2,0) to (10,0); %asse ottico
	
	\draw (-1,3) to (0,3) to (7,0.375);
	\draw[dotted] (7,0.375) to (8,0);
	
	\draw[red!50] (-1,2.75) to (0,3) to (7,2.125);
	\draw[dotted,red!50] (7,2.125) to (8,2);
	\draw[red!50] (7,2.125) to (9,4);
	
	\draw[red!50] (-2,-0.5) to (7,1.75);
	\draw[dotted,red!50] (7,1.75) to (8,2); %chief red
	\draw[red!50] (7,1.75) to (9,4);
	
	\draw[dash dot,red!50] (6,1.75) to (9,1.75);
	
	\draw[red!50] (-1,-3.25) to (0,-3) to (7,1.375);
	\draw[dotted,red!50] (7,1.375) to (8,2);
	\draw[red!50] (7,1.375) to (9,4);
	
	\draw[dotted,red!50] (7,0) to (9,4);
	
	\draw (-1,-3) to (0,-3) to (7,-0.375);
	\draw[dotted] (7,-0.375) to (8,0);
	
	\draw[dotted] (5.4444,0.66675) to (7,0.375);
	\draw[dotted] (5.4444,-0.66675) to (7,-0.375);
	\draw (7,0.375) to (9,0);
	\draw (7,-0.375) to (9,0);	
	
	
	\coordinate (a) at (-1,-0.25); \coordinate (b) at (0,0); \coordinate (c) at (-1,0); 
	\pic[draw,"$\theta_e$", draw=black,<->,angle eccentricity=1.3,angle radius=1.5cm]{angle=c--b--a};
	
	\coordinate (d) at (8,1.75); \coordinate (e) at (7,1.75); \coordinate (f) at (9,4); 
	\pic[draw,"$\theta_u$", draw=black,<->,angle eccentricity=1.3,angle radius=1.5cm]{angle=d--e--f};	

	\coordinate (g) at (7,0); \coordinate (h) at (5.4444,0); \coordinate (i) at (7,1.75); 
	\pic[draw,"$\theta_u$", draw=black,<->,angle eccentricity=1.3,angle radius=0.5cm]{angle=g--h--i};	
	
	\draw[dotted,red!50] (5.4444,0) to (7,1.75);
	
	\draw[red] (5.4444,0.66675) circle (1pt);
	\draw[dotted,red!50] (5.4444,0.66675) to (7,2.125);
	\draw[dotted,red!50] (5.4444,-0.66675) to (7,1.375);
	
	\draw[dotted] (5.4444,-3) to (5.4444,3);   
	\draw[-|] (5.4444,3) to (5.4444,0.66675);  %pupilla uscita
	\draw[-|] (5.4444,-3) to (5.4444,-0.66675);
	
	
	\draw[dashed, <->] (0,-3.5) -- (9,-3.5) node[above, midway]{$f_{eq}$};
	\draw[dashed, <->] (5.4444,-2.5) -- (9,-2.5) node[below, midway]{$d_p$};
	
	\end{tikzpicture}
	\caption{Schema di un telescopio con strumento ottico che accresce la focale equivalente e pupilla d'uscita più vicina al piano focale della pupilla di entrata per cui l'angolo non-telecentrico risulta maggiore dell'angolo di ingresso della radiazione}\label{figure:fovnta}
\end{figure}

Utilizzando la notazione di figura \ref{figure:fovnta} vediamo dallo schema che, in approssimazione di angoli piccoli, $$d_p \theta_u=f_{eq}\theta_e$$. Ricordando la definizione di F-number la lunghezza focale equivalente $f_{eq}$ è $f_{eq}=D_e F$ dove $D_e$ è la dimensione della pupilla di ingresso. Nel nostro schema, la dimensione delle pupilla di ingresso, equivale al diametro del primo elemento ottico, che frequentemente nei telescopi coincide con il diametro dello specchio primario. Quindi l'angolo non-telecentrico che qui abbiamo chiamato $\theta_u$ è direttamente proporzionale all'angolo di ingresso, ovvero la distanza da centro del campo di vista, al rapporto focale, è invece inversamente proporzionale alla distanza della pupilla d'uscita.
\begin{equation}
	\theta_u=\theta_e D_e \frac{F}{d_p}
\end{equation}
 

==> TeX_files/Results.tex <==
\chapter{Results}

==> TeX_files/Software.tex <==
\chapter[Simulazioni Numeriche]{Simulazioni numeriche} \label{Chap:Numerical}
In questo capitolo presenteremo alcune simulazioni numeriche di carattere generale che ci consentano di caratterizzare la risposta dei filtri interferenziali in differenti configurazioni ottiche. \\ 
I risultati numerici sono ottenuti attraverso la simulazione di vari filtri interferenziali passa-banda, caratterizzati da differenti forme della curva di trasmissione, della larghezza di banda e potenzialmente dell'indice di rifrazione equivalente. Lo studio è stato realizzato simulando filtri collocati in una zona convergente del fascio, in prossimità del piano focale, come molto frequente per gli strumenti in telescopi ground-based. A differenza dell'approccio analitico, utilizzato da autori \textit{classici} \parencite{Lissberger:59II,Pidgeon:64}, che presuppone una conoscenza esatta delle caratteristiche costruttive del filtro, abbiamo utilizzato i loro risultati più generali sulla risposta spettrale di un filtro per procedere numericamente.\\

Il codice Python realizzato per questo studio prende in input la forma della curva di trasmissione nello spazio delle lunghezze d'onda; il rapporto focale del telescopio; la dimensione relativa dell'ostruzione centrale; la scelta tra una pupilla di classica forma circolare o una pupilla di forma esagonale (come la pupilla dei telescopi Keck o come la forma dell'ostruzione del futuro ELT)\footnote{Pur avendo eseguito vari confronti utilizzando tale forma della pupilla non ne riporteremo qui i dati che non sono utili per trarre linee generali. L'effetto complessivo della presenza di una pupilla esagonale è quello di restringere a parità di rapporto focale la rilevanza della deformazione verso lunghezze minori, ma non cambiando sostanzialmente la situazione. In ogni caso per uno studio dettagliato di un preciso caso reale o per cercare la configurazione ottimale può risultare utile studiare anche il caso con la forma esagonale. }. 
In uscita possiamo ottenere tabelle numeriche e grafici che rappresentano la nuova forma della curva di trasmissione modificata dalla configurazione ottica (come in Figura \ref{deformed}) oppure grafici che relazionano tra loro differenti parametri: in particolare la larghezza di banda (FWHM) con F-number o con l'angolo non-telecentrico ovvero, proporzionalmente, la distanza dal centro del campo di vista. \\
Per i nostri particolari scopi lo spostamento della lunghezza d'onda centrale e la larghezza di banda in funzione dell'angolo non-telecentrico sono due relazioni di grande importanza, perché conducono ad una variazione differenziale all'interno del campo di vista. Un esempio di tali relazioni possiamo vederlo in Figura \ref{nta}. Come vedremo, la deformazione introdotta esclusivamente dal diverso rapporto focale come in una configurazione ottica completamente telecentrica, è, entro certi limiti, facilmente gestibile, potendo liberamente modificare la forma nominale del filtro per ottenere quella reale desiderata. Nel caso generico e più comune nella realtà, la deformazione, dovuta all'angolo con cui il raggio principale si discosta dalla normale al filtro, si sovrappone a quella dovuta al rapporto focale conducendo a risultati strettamente dipendenti dai dettagli della configurazione. Per questo motivo uno studio di casi specifici è necessario per trarre delle conclusioni sull'utilità scientifica di un particolare filtro. \\ 

\begin{figure}
	\subfloat[]{\includegraphics[width=0.55\textwidth]{Figure/deformed.pdf}}
	\subfloat[]{\includegraphics[width=0.55\textwidth]{Figure/Gauss_shape_fwhm50_@diff_f.pdf}}
	\caption{La curva di trasmissione del filtro è degradata a causa dell'angolo non costante con cui la radiazione investe il filtro}%Filter transmission's shape is deformed (shifted and smoothed) under the effect of a non-constant incidence angle. The extension of the angle aperture is related with the focal ratio.}
	\label{deformed}
\end{figure}

\begin{figure}
	\subfloat[]{\includegraphics[width=0.55\textwidth]{Figure/Shift_vs_nta.pdf}}
	\subfloat[]{\includegraphics[width=0.5\textwidth]{Figure/fwhm_vs_nta_obs_NewCa.pdf}}
	\caption{Con il variare dell'angolo non-telecentrico (nta), corrispondente a variazioni di posizione nel campo di vista, sia la lunghezza d'onda di pivot sia la fwhm variano}%With the variation of the non-telecentric angle (nta), corresponding to variation of position in the field of view, both pivotal wavelenght and fwhm vary, possibly dramatically. } 
	\label{nta}
\end{figure}


\section{Deformazione dovuta al rapporto focale}

Secondo la formula $\rho_{0}=\arctan(\frac{1}{2F})$ dove $\rho_{0}$ rappresenta la semiapertura del cono di luce, ovvero l'angolo massimo di scostamento dalla normale al filtro nel caso telecentrico, differenti rapporti focali corrispondono a differenti angoli di apertura del fascio convergente. Il caso telecentrico è rappresentato in figura \ref{lightcone}.
\\Ogni elemento d'area del filtro è raggiunto da una radiazione che incide sulla superficie con un differente angolo rispetto alla normale al filtro. Abbiamo rappresentato graficamente questa situazione in figura \ref{AnglesOnFilter}, dove i piccoli vettori disegnati all'interno dell'impronta della pupilla sul filtro indicano la direzione e il modulo dell'angolo di incidenza della radiazione in caso telecentrico. \\


\subsection{Lo spazio non-normale}
Nella figura \ref{nonNormality} abbiamo definito lo spazio non-normale nel quale rappresentare l'impronta della pupilla sul filtro \parencite{Cremillo} nei termini di misure angolari. \\
L'angolo $\theta_{0}$ definisce lo scostamento dalla normale del raggio principale del cono di luce convergente relativo ad una particolare sorgente, mentre $\rho_{0}$ e $\epsilon\rho_{0}$ rappresentano rispettivamente la semiapertura del fascio e dell'ostruzione. Per il calcolo del contributo che ogni elemento d'area del filtro fornisce al flusso totale che raggiunge il sensore abbiamo suddiviso l'impronta della pupilla con un griglia fine di quadrati (esagerati in figura \ref{nonNormality}) con una densità usuale di circa 15000 campionamenti sull'intera superficie \footnote{In realtà tutti i calcoli sono eseguiti su metà dell'impronta date le condizioni di simmetria. In figura \ref{nonNormality} ad essere realmente campionata è solo la metà con $\phi_{y}>0$}. 

\begin{figure}
\centering
\begin{tikzpicture}[scale=0.8]
	\draw 
	(0,0) coordinate (a) 
	-- (4,8) coordinate (b) node[above]{Focal point}
	-- (4,0) coordinate (c) node[midway,right]{$f$} node[below  left]{Exit Pupil}
	pic["$\rho_{0}$", draw=orange,<->,angle eccentricity=1.3,angle radius=3cm]{angle=a--b--c};
	\draw (8,0) -- (4,8);
	\draw (0,0) -- (8,0) ;
	\draw[<->] (4,-0.2) -- (8,-0.2) node[midway, below]{$\frac{D}{2}$};
	\draw (-1.5,7) node[right]{$\tan{\rho_{0}}=\frac{D/2}{f}$, $f=\frac{f}{D}$};
	\draw (-1.5,6) node[right]{$\Rightarrow \: \rho_{0}=\arctan{\frac{1}{2F}}$};
\end{tikzpicture}
	\caption{Fascio convergente} \label{lightcone}	
\end{figure}

\begin{figure}
	\centering
	\input{./TeX_files/AngleOnFilter.tex}
	\caption{La radiazione in zona di fascio convergente incide sul filtro con uno spettro di angoli da 0 al centro e aumentando verso l'esterno}%incident-light angles on the filter. The angle to the normal increases going outer} 
	\label{AnglesOnFilter}	
\end{figure}


\begin{figure}
	\centering
	\begin{tikzpicture}[>=stealth, inner sep=0pt, outer sep=2pt,]
	%GRID
	%\draw[step=1cm,gray!50,very thin,dashed] (-3,-5) grid (7,5);
	\foreach \x in {-3,-2,...,7}{
		\draw[dashed,black!40,very thin] (\x,-5)--(\x,5);
		\draw[dashed,black!40,very thin] (-3,\x-2)--(7,\x-2);
	}

	%AXIS
	\draw[thick, ->] (-3.5,0) -- (8,0) node[below,font=\large]{\textbf{$\phi_{x}$}};
	\draw[thick, ->] (0,-5.5) -- (0,6) node[left,font=\large]{\textbf{$\phi_{y}$}};
		
	%PUPIL
	\draw (2,0) circle (5);
	\draw (2,0) circle (1.5);
	
	%LITTLE SQUARE
	\draw[draw=black!50,pattern=dots,pattern color=orange!50] (3,3)--(3,4)--(4,4)--(4,3)--(3,3);
	\draw[<->] (2.9,3)--(2.9,4) node[midway,left,font=\large]{$d\phi_{y}$};
	\draw[<->] (3,2.9)--(4,2.9) node[midway,below,font=\large]{$d\phi_{x}$};
	%phi
	\draw[very thick,->,green!50] (0,0)--(3.5,3.5) node[right,black,font=\boldmath]{\textbf{$\theta$}};
	%nta
	\draw[very thick,->,orange] (0,0) -- (2,0) node[below left,black,font=\boldmath]{\textbf{$\theta_{0}$}};
	\draw[very thick,->,magenta] (2,0) -- (5,-4) node[below,black,font=\boldmath]{\textbf{$\rho_{0}$}};
	\draw[very thick,->,purple] (2,0) -- (2,-1.5) node[below,black,font=\boldmath]{\textbf{$\epsilon\rho_{0}$}};	
	\end{tikzpicture}
	\caption[Impronta della pupilla sul filtro]{La pupilla d'entrata come impressa sul filtro, rappresentato nello spazio non-normale, dove $\theta_{0}$ rappresenta l'angolo non-telecentrico di uno specifico punto del campo di vista e $\rho_{0}$ la semiapertura del cono come identificata in figura figure \ref{lightcone} }%the entrance pupil as footprinted on the filter, rapresented on a non-normality space where $\theta_{0}$ represents the non-telecentric angle of a specific pint in the field of view and $\rho_{0}$ rapresents the light-cone aperture as identified in figure \ref{lightcone} } 
	\label{nonNormality}
\end{figure}

Ogni elemento di area $d\phi_{x}d\phi_{y}$  (fig. \ref{nonNormality})riceve un flusso pari all'intensità complessiva del fascio (che consideriamo normalizzata a 1) divisa per il numero di campioni\footnote{Computazionalmente, non conoscendo a priori l'esatto numero di campioni, potendo variare apertura del fascio e forma della pupilla, si è considerato ogni elemento con flusso pari a 1, provvedendo poi a normalizzare l'integrale.}. Ogni campione rappresenta un filtro differente rispetto a quello nominale dato che riceve la radiazione con un angolo non-normale alla superficie, cosa che provoca un arretramento della banda passante come visto al capitolo \ref{chap:optical}. 

Infatti 
\begin{equation}\label{math:lambdatheta}
\lambda(\theta)=\lambda_0 \sqrt{1-\frac{\sin^2(\theta)}{\mu_*^2}}
\end{equation}
 rappresenta il comportamento della lunghezza d'onda di picco al variare dell'angolo di incidenza del raggio principale per un filtro interferenziale del tipo a strati sottili multipli. In maniera equivalente ad un semplice modello di filtro a la Fabry-Perot, dove $\mu_*$ rappresenta l'indice di rifrazione efficacie, definito in \textcite{Pidgeon:64} e visto alla sezione \ref{sec:alldielectric}. \\
 Questo significa che nello spazio non-normale esistono delle curve isofiltranti (circonferenze nel caso telecentrico, altrimenti archi di circonferenza) che possiamo approssimare con anelli isofiltranti come in figura \ref{isofiltranti}. È chiaro che nel caso telecentrico, anelli più esterni presentino una superficie maggiore di quelli più interni, andando a determinare una preminenza delle lunghezze d'onda più traslate.\\ 
 
 Se ne può vedere l'effetto in figura \ref{deltafunction} dove si nota il crollo dell'efficienza di trasmissione per un filtro molto stretto che viene \textit{trascinato} su lunghezze d'onda minori con una lenta crescita verso la lunghezza minima\footnote{Qui come in tutti i casi dove non diversamente specificati le simulazioni sono svolte considerando una ostruzione relativa $\epsilon=0.1$. Ostruzioni maggiori riducono lo spread di angoli.}. Se supponiamo che ogni elemento infinitesimo di filtro mantenga la medesima forma della curva di trasmissione nominale, semplicemente con una lunghezza d'onda centrale traslata secondo la \ref{math:lambdatheta}, il flusso integrato su tutta la superficie è conservato.\\ Questo risultato è consolidato in letteratura purché la progettazione degli strati sottili del filtro abbia tenuto in conto la possibilità che la superficie venga raggiunta da radiazione non-normale conservando la forma della curva di trasmissione \parencite[364-367]{macleod2010thin}. \\
 
 L'integrale su tutta la superficie del filtro è perciò il risultato dello spalmarsi su un'intervallo di lunghezze d'onda del contributo dei singoli elementi d'area. Più è ampio l'intervallo di lunghezze d'onda su cui si distribuisce il contributo dei singoli elementi d'area, ovvero più è ampia l'apertura del cono di luce (più piccolo è l'F-number), più l'efficienza di trasmissione per una certa lunghezza d'onda decresce. Ogni circonferenza concentrica rappresenta quindi un filtro differente: nel caso rappresentato in fig. \ref{deltafunction} anelli adiacenti presentano curve di trasmissione che quasi non si sovrappongono a causa della banda particolarmente stretta. \\
Nel caso non-telecentrico i rapporti fra le aree degli anelli isofiltranti si fanno più complessi\footnote{ad esempio in figura \ref{isofiltranti} le aree arancioni e quelle ciano sono comparabili.}, basti pensare che nei casi in cui $\phi_0$ è sufficientemente diversa da 0 il filtro è raggiunto da radiazione normale alla superficie, mentre nel caso telecentrico ne è esclusa perché ricade nell'ostruzione. Questo conduce a deformazioni del filtro integrato meno lineari, come illustrato in figura \ref{figure:asym-nta} e figura \ref{figure:squarefilternta} e approfondiremo nella prossima sezione. \\ 

\begin{figure}
	\input{./TeX_files/AnelloSuPupilla.tex}
	\caption[Anelli Isofiltranti]{Anelli più vicini alla normale presentano una lunghezza d'onda di picco del filtro più prossima a quella nominale, mano a mano che ci si sposta ad angoli maggiori assistiamo ad un più consistente spostamento.} \label{isofiltranti}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/DeltaFunction_@diff_f.pdf}
	\caption{Un filtro nominale molto stretto ($\sim\delta$) viene drammaticamente deformato a differenti rapporti focali perché ogni elemento del filtro riceve la radiazione con un differente angolo. Si può vedere come l'efficienza aumenti per le lunghezze d'onda minori, per i motivi illustrati nel testo riguardo gli anelli isofiltranti.} \label{deltafunction}
\end{figure}

I filtri interferenziali rispondono quindi a differenti F-numbers come rappresentato in figura \ref{deformed} (b). Il grafico è stato costruito partendo da un filtro gaussiano con una $fwhm=50\AA$: il filtro si allarga e l'efficienza di trasmissione per ogni lunghezza d'onda decresce al decrescere del rapporto focale. \\
Un primo sguardo qualitativo, tramite le figure \ref{deformed}(b) e \ref{deltafunction}, ci fornisce già alcune indicazioni. Per ogni F-number esiste un valore minimo della fwhm che si può raggiungere quantunque sia stretto il filtro, per $F/1$ parliamo di quasi $10nm$. Allo stesso modo però possiamo vedere come per F-number sufficientemente grandi l'effetto di deformazione sia contenuto e molto dipendente dalla forma iniziale del filtro. \\

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/SteepFilterSameFWHM60.pdf}
	\caption{Deformazione di un filtro quadrato di larghezza 60 \AA, ricentrato a 0\AA, da cui si nota la conservazione della fwhm e contemporaneamente la diminuzione del flusso che ricade all'interno della fwhm. Come apprezzabile in tabella \ref{table:squarefilter}}\label{figure:squarefilter}
\end{figure}

\subsection{Simulazioni su un set di filtri quadrati}\label{sec:quadrati}
Per uno studio più sistematico abbiamo costruito un set di filtri con curva di trasmissione quadrata\footnote{trasmissione zero ovunque e trasmissione uno nella banda passante, con una variazione molto rapida} e banda passante di 10, 20, 40, 60, 80 e 100$\AA$ dei quali studiare la deformazione dal punto di vista qualitativo e sopratutto il comportamento quantitativo di alcuni parametri: posizione della lunghezza d'onda di pivot\footnote{la lunghezza che divide a metà il flusso totale.}, la FWHM, il picco di trasmissione e quello che abbiamo chiamato $I_{ratio}$, il rapporto fra il flusso che ricade all'interno della FWHM e il flusso totale espresso in percentuale, ovvero un indicatore che in via complementare indica la rilevanza delle le code nella forma del filtro in analisi. \\
In figura \ref{figure:squarefilter} si può vedere l'effetto di deformazione sul filtro quadrato di larghezza $60\AA$ originariamente centrato a $4000\AA$  per differenti rapporti focali. Nell'immagine ogni forma della curva di trasmissione integrata è stata traslata su $\lambda_{Piv}=0$ per mettere in luce la conservazione della FWHM con differenti rapporti focali e la contemporanea diminuzione della quota di flusso che si può trovare all'interno della FWHM medesima, fenomeno che giustifica la necessità di introdurre il parametro $I_{ratio}$. \\
In tabella \ref{table:squarefilter} troviamo invece la trattazione quantitativa estesa a tutto il set di filtri definiti. Abbiamo riportato i dati relativi ad un set di filtri centrati su $4000\AA$ a sinistra e su $2000\AA$ a destra, la prima colonna rappresenta l'arretramento percentuale della lunghezza d'onda di pivot rispetto alla posizione iniziale di 4000 o 2000$\AA$, la seconda colonna riporta la variazione relativa della FWHM rispetto a quella nominale del filtro, la terza il rapporto $I_{ratio}$ definito in precedenza e l'ultima riporta il picco massimo di trasmissione. \\
Come si può notare, l'arretramento relativo per ogni F-number è caratteristico dell'F-number medesimo e uguale per ogni filtro: inferiore allo $0.05\%$ per F/8 e maggiori, fino allo $0.7\%$ per $F/1.4$ che nel caso centrato su $4000\AA$ si traduce in un arretramento assoluto di $28\AA$, che in talune applicazioni può risultare particolarmente significativo. La FWHM è sempre conservata ( $\frac{\Delta fwhm}{FWHM}=0$) per filtri nominali sufficientemente larghi, come nel caso dalla figura \ref{figure:squarefilter}. Possiamo notare, in particolare, che ovunque si abbia a che fare con intensità massima di picco pari ad uno, ovvero quando il filtro, a quel particolare rapporto focale, presenta almeno un ristrettissimo intervallo di frequenze in cui ogni \textit{filtro infinitesimo} si sovrappone a tutti gli altri (per F/1.4 inizia ad avvenire tra i 40\AA e $60\AA$), la FWHM è pari a quella originale. \\Alla conservazione della FWHM non corrisponde però l'equivalenza del filtro deformato con il filtro nominale. Assistiamo ad una forte degradazione delle caratteristiche ai bordi della curva di trasmissione che nel caso di figura \ref{figure:squarefilter} si trasforma da quadrata a triangolare. Le code esterne alla FWHM divengono quindi significative consentendo la trasmissione di radiazione ben oltre il limite del filtro nominale. \\

In ogni caso, fino a questo punto, abbiamo a che fare con trasformazioni della curva di trasmissione gestibili in fase progettuale: nel caso peggiore presente in tabella \ref{table:squarefilter},  $FWHM=60\AA$ e $F/1.4$, continuiamo comunque ad avere quasi l'$80\%$ del flusso all'interno della FWHM. Certo dobbiamo ricordare che, per ogni rapporto focale e proporzionalmente alla lunghezza d'onda di pivot, abbiamo una FWHM minima sotto la quale non possiamo scendere: sarà quindi velleitario cercare di costruire un filtro interferenziale al disotto dei $57\AA$ ($5.7*10\AA$ tab. \ref{table:squarefilter}) per strumenti con F/1.4 con $\lambda_0=4000\AA$ (o $28\AA$ con $\lambda_0=2000$, o ancora di $113\AA$ per $\lambda_0=8000\AA$) o sotto i $30\AA$ per F/2\footnote{stiamo operando sempre con una ostruzione pari a 0.1}. Per forme meno nette, come il caso di un filtro con curva di trasmissione gaussiana come quella di figura \ref{deformed}(b), dove le code contano, di per sé, maggiormente, l'esito può essere differente dal punto di vista pratico, ma questo studio ci fornisce comunque dei limiti orientativi. 

\begin{table}\centering
	\begin{tabular}{l|l}
		\begin{tabular}{lp{1.2cm}|lp{1.2cm}ll}
			\multicolumn{2}{c}{obs=0.1} & \multicolumn{4}{c}{4000\AA}\\ 
			&F/ & $\frac{\Delta\lambda_p}{\lambda_0}\%$ & $\frac{\Delta fwhm}{fwhm}$ & Iratio & $max_{tr}$ \\ \hline\hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{10 \AA}}
			&8.0 & 0.0 & 0.00 & 95.01 & 1.00 \\ 
			&5.6 & 0.1 & 0.00 & 90.02 & 1.00 \\ 
			&4.0 & 0.1 & 0.00 & 80.63 & 1.00 \\ 
			&2.8 & 0.2 & 0.55 & 83.63 & 0.65 \\ 
			&2.0 & 0.4 & 1.94 & 91.09 & 0.35 \\ 
			&1.4 & 0.7 & 4.67 & 95.19 & 0.18 \\ \hline %56.7\AA
			\multirow{6}{*}{\rotatebox[origin=c]{90}{20 \AA}}
			&8.0 & 0.0 & 0.00 & 97.50 & 1.00 \\ 
			&5.6 & 0.1 & 0.00 & 95.01 & 1.00 \\ 
			&4.0 & 0.1 & 0.00 & 90.31 & 1.00 \\ 
			&2.8 & 0.2 & 0.00 & 80.56 & 1.00 \\ 
			&2.0 & 0.4 & 0.47 & 82.72 & 0.68 \\ 
			&1.4 & 0.7 & 1.83 & 90.77 & 0.36 \\ \hline%56.6\AA
			\multirow{6}{*}{\rotatebox[origin=c]{90}{40 \AA}}
			&8.0 & 0.0 & 0.00 & 98.75 & 1.00 \\ 
			&5.6 & 0.1 & 0.00 & 97.50 & 1.00 \\ 
			&4.0 & 0.1 & 0.00 & 95.16 & 1.00 \\ 
			&2.8 & 0.2 & 0.00 & 90.28 & 1.00 \\ 
			&2.0 & 0.4 & 0.00 & 81.50 & 1.00 \\ 
			&1.4 & 0.7 & 0.42 & 82.05 & 0.71 \\ \hline %56.8
			\multirow{6}{*}{\rotatebox[origin=c]{90}{60 \AA}}
			&8.0 & 0.0 & 0.00 & 99.17 & 1.00 \\ 
			&5.6 & 0.1 & 0.00 & 98.34 & 1.00 \\ 
			&4.0 & 0.1 & 0.00 & 96.77 & 1.00 \\ 
			&2.8 & 0.2 & 0.00 & 93.52 & 1.00 \\ 
			&2.0 & 0.4 & 0.00 & 87.67 & 1.00 \\ 
			&1.4 & 0.7 & 0.00 & 76.20 & 1.00 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{80 \AA}}
			&8.0 & 0.0 & 0.00 & 99.38 & 1.00 \\ 
			&5.6 & 0.1 & 0.00 & 98.75 & 1.00 \\ 
			&4.0 & 0.1 & 0.00 & 97.58 & 1.00 \\ 
			&2.8 & 0.2 & 0.00 & 95.14 & 1.00 \\ 
			&2.0 & 0.4 & 0.00 & 90.75 & 1.00 \\ 
			&1.4 & 0.7 & 0.00 & 82.15 & 1.00 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{100 \AA}}
			&8.0 & 0.0 & 0.00 & 99.50 & 1.00 \\ 
			&5.6 & 0.1 & 0.00 & 99.00 & 1.00 \\ 
			&4.0 & 0.1 & 0.00 & 98.06 & 1.00 \\ 
			&2.8 & 0.2 & 0.00 & 96.11 & 1.00 \\ 
			&2.0 & 0.4 & 0.00 & 92.60 & 1.00 \\ 
			&1.4 & 0.7 & 0.00 & 85.72 & 1.00 \\
			\hline
		\end{tabular}
		&
		\begin{tabular}{llll}
     \multicolumn{4}{c}{2000\AA}\\
		 $\frac{\Delta\lambda_p}{\lambda_0}\%$ & $\frac{\Delta fwhm}{fwhm}$ & Iratio & $max_{tr}$ \\ \hline \hline
		 0.0 & 0.00 & 97.44 & 1.00 \\ 
		 0.1 & 0.00 & 94.96 & 1.00 \\ 
		 0.1 & 0.00 & 90.24 & 1.00 \\ 
		 0.2 & 0.00 & 80.60 & 1.00 \\ 
		 0.4 & 0.47 & 82.77 & 0.68 \\ 
		 0.7 & 1.83 & 90.79 & 0.36 \\ \hline %(28.3)
		 0.0 & 0.00 & 98.72 & 1.00 \\ 
		 0.1 & 0.00 & 97.48 & 1.00 \\ 
		 0.1 & 0.00 & 95.12 & 1.00 \\ 
		 0.2 & 0.00 & 90.30 & 1.00 \\ 
		 0.4 & 0.00 & 81.51 & 1.00 \\ 
		 0.7 & 0.42 & 82.07 & 0.71 \\ \hline %(28.4)
		 0.0 & 0.00 & 99.36 & 1.00 \\ 
		 0.1 & 0.00 & 98.74 & 1.00 \\
		 0.1 & 0.00 & 97.56 & 1.00 \\
		 0.2 & 0.00 & 95.15 & 1.00 \\ 
		 0.4 & 0.00 & 90.75 & 1.00 \\ 
		 0.7 & 0.00 & 82.14 & 1.00 \\ \hline
		 0.0 & 0.00 & 99.57 & 1.00 \\ 
		 0.1 & 0.00 & 99.16 & 1.00 \\ 
		 0.1 & 0.00 & 98.37 & 1.00 \\ 
		 0.2 & 0.00 & 96.76 & 1.00 \\ 
		 0.4 & 0.00 & 93.83 & 1.00 \\ 
		 0.7 & 0.00 & 88.09 & 1.00 \\ \hline
		 0.0 & 0.00 & 99.68 & 1.00 \\ 
		 0.1 & 0.00 & 99.37 & 1.00 \\ 
		 0.1 & 0.00 & 98.78 & 1.00 \\ 
		 0.2 & 0.00 & 97.57 & 1.00 \\ 
		 0.4 & 0.00 & 95.38 & 1.00 \\ 
		 0.7 & 0.00 & 91.07 & 1.00 \\ \hline
		 0.0 & 0.00 & 99.74 & 1.00 \\ 
		 0.1 & 0.00 & 99.50 & 1.00 \\ 
		 0.1 & 0.00 & 99.02 & 1.00 \\ 
		 0.2 & 0.00 & 98.06 & 1.00 \\ 
		 0.4 & 0.00 & 96.30 & 1.00 \\ 
		 0.7 & 0.00 & 92.85 & 1.00 \\ \hline
		\end{tabular}
	\end{tabular}
	\caption{Un serie di filtri centrati su 4000\AA  nella tabella di sinistra e 2000\AA in quella di destra sono deformati da differenti F-number} \label{table:squarefilter}
\end{table}




\section{Filtro sotto differenti angoli non-telecentrici}
Come già brevemente riassunto nella sezione precedente e illustrato in figura \ref{isofiltranti}, se il raggio principale del fascio convergente raggiunge la superficie del filtro discostandosi dalla normale il contributo dei singoli elementi di superficie conferisce alla curva di trasmissione integrata una deformazione, rispetto alla forma nominale, che dipende dalla distanza dalla normale. In figura \ref{nta}(a) si può seguire lo scostamento della lunghezza d'onda di picco da quella nominale del filtro in un caso gaussiano e in figura \ref{nta}(b), si può invece vedere come vari la $FWHM$ per un filtro che presenta una larghezza nominale di $85\AA$ non molto dissimile dal filtro $Ca_{new}$ utilizzato da JWL \parencite{Lee_2017}. 
La deformazione asimmetrica è apprezzabile qualitativamente in figura \ref{figure:asym-nta}. \\
Dato che l'angolo non-telecentrico è proporzionale alla distanza angolare dal centro del campo di vista, la deformazione introdotta genera una aberrazione differenziale: sorgenti in posizioni differenti all'interno del FoV vengono filtrate differentemente. Benché il picco di trasmissione rimanga abbastanza stabile, come visibile in figura \ref{figure:asym-nta}, il baricentro della curva di trasmissione si sposta a lunghezze d'onda minori e con una FWHM maggiore. Per tenere conto di questa deformazione abbiamo utilizzato le grandezze già precedentemente definite: la lunghezza d'onda di pivot e un indicatore che restituisce la frazione di flusso che ricade all'interno della FWHM $I_{ratio}$. In figura \ref{figure:Iratio} è possibile vedere l'effetto di deformazione su un filtro con indicate le grandezze appena ricordate.\\

\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{Figure/Gauss_shape_fwhm50_@diff_nta.pdf}	
	\caption{Deformazione di un filtro gaussiano con differenti angoli non-telecentrici}\label{figure:asym-nta}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.7\textwidth]{Figure/NewCa_f14_nta025_0bs01.pdf}
	\caption{Deformazione filtro. Indicate la lunghezza di Pivot e $I_{ratio}$}\label{figure:Iratio}
\end{figure}

In tabella \ref{table:squarefilternta} abbiamo gli stessi parametri riportati nella tabella \ref{table:squarefilter}, non più al variare dell'$F-number$ bensì dell'angolo non-telecentrico (da $0\deg$ a $10\deg$) su di uno strumento con ostruzione relativa di 0.1. Inoltre sono presentati due casi: a sinistra con F/1.4 e a destra con F/4. \\
La presenza di un angolo non-telecentrico (lo indicheremo come \textit{nta} da ora innanzi) conduce ad una aberrazione differenziale all'interno del campo di vista, per qualsiasi rapporto focale e qualsiasi FWHM, per due ordini di motivi: 
\begin{itemize}
	\item si verifica sempre un arretramento maggiore della lunghezza d'onda di pivot per \textit{nta} maggiori (quindi verso il bordo del FoV)
	\item può originare per l'$I_{ratio}$ una differenza maggiore del 10\%, anche per larghezze di banda ampie e F-number rilassato come nel caso del filtro di larghezza $80\AA$ con $F/4$ (ultime quattro colonne del quinto gruppo di righe di tabella \ref{table:squarefilternta}).
\end{itemize}
  Il caso da $60\AA$, visibile in figura \ref{figure:asym-nta} e segnalato in tabella, ci dà conto della asimmetria della deformazione introdotta dall'angolo non-telecentrico. Quindi ne possiamo dedurre la necessità di uno studio particolareggiato dell'accoppiamento strumento/caso scientifico per caratterizzare il filtro più adatto. \\

\begin{table}
	\begin{tabular}{l|l}
		\begin{tabular}{ll|llll}
			&nta & $\frac{\Delta\lambda_p}{\lambda_0}\%$ & $\frac{\Delta fwhm}{fwhm}$ & Iratio & $max_{tr}$ \\ \hline\hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{10 \AA}}
			&0.0 & 0.7 & 4.67 & 95.19 & 0.18 \\ 
			&2.0 & 0.7 & 4.67 & 90.63 & 0.18 \\ 
			&4.0 & 0.7 & 4.61 & 83.57 & 0.18 \\ 
			&6.0 & 0.8 & 4.44 & 75.50 & 0.17 \\ 
			&8.0 & 0.8 & 4.28 & 67.85 & 0.17 \\ 
			&10.0 & 0.9 & 3.69 & 56.81 & 0.17 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{20 \AA}}
			&0.0 & 0.7 & 1.83 & 90.77 & 0.36 \\ 
			&2.0 & 0.7 & 1.85 & 88.26 & 0.35 \\ 
			&4.0 & 0.7 & 1.82 & 81.53 & 0.35 \\ 
			&6.0 & 0.8 & 1.75 & 73.87 & 0.34 \\ 
			&8.0 & 0.8 & 1.72 & 66.92 & 0.33 \\ 
			&10.0 & 0.9 & 1.79 & 61.87 & 0.31 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{40 \AA}}
			&0.0 & 0.7 & 0.42 & 82.05 & 0.71 \\ 
			&2.0 & 0.7 & 0.43 & 81.11 & 0.70 \\ 
			&4.0 & 0.8 & 0.46 & 77.85 & 0.67 \\ 
			&6.0 & 0.8 & 0.54 & 74.28 & 0.63 \\ 
			&8.0 & 0.8 & 0.67 & 72.07 & 0.58 \\ 
			&10.0 & 0.9 & 0.87 & 70.98 & 0.53 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{60 \AA, fig.\ref{figure:squarefilternta}}}
			&0.0 & 0.7 & 0.00 & 76.20 & 1.00 \\ 
			&2.0 & 0.7 & 0.05 & 77.42 & 0.95 \\ 
			&4.0 & 0.8 & 0.11 & 77.34 & 0.89 \\ 
			&6.0 & 0.8 & 0.20 & 76.45 & 0.82 \\ 
			&8.0 & 0.9 & 0.33 & 75.94 & 0.76 \\ 
			&10.0 & 1.0 & 0.47 & 74.98 & 0.69 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{80 \AA}}
			&0.0 & 0.7 & 0.00 & 82.15 & 1.00 \\ 
			&2.0 & 0.8 & 0.00 & 81.40 & 1.00 \\ 
			&4.0 & 0.8 & 0.00 & 79.32 & 1.00 \\ 
			&6.0 & 0.8 & 0.04 & 77.54 & 0.95 \\ 
			&8.0 & 0.9 & 0.12 & 76.65 & 0.89 \\ 
			&10.0 & 1.0 & 0.23 & 76.20 & 0.83 \\ \hline
			\multirow{6}{*}{\rotatebox[origin=c]{90}{100 \AA}}
			&0.0 & 0.7 & 0.00 & 85.72 & 1.00 \\ 
			&2.0 & 0.8 & 0.00 & 85.12 & 1.00 \\ 
			&4.0 & 0.8 & 0.00 & 83.37 & 1.00 \\ 
			&6.0 & 0.9 & 0.00 & 80.47 & 1.00 \\ 
			&8.0 & 1.0 & 0.02 & 77.57 & 0.98 \\ 
			&10.0 & 1.1 & 0.07 & 76.29 & 0.93 \\ \hline \hline
		\end{tabular}&
		\begin{tabular}{llll}
 $\frac{\Delta\lambda_p}{\lambda_0}\%$ & $\frac{\Delta fwhm}{fwhm}$ & Iratio & $max_{tr}$ \\ \hline \hline
 0.1 & 0.00 & 80.63 & 1.00 \\ 
 0.1 & 0.07 & 77.61 & 0.92 \\
 0.1 & 0.37 & 75.64 & 0.74 \\ 
 0.2 & 0.85 & 76.80 & 0.57 \\ 
 0.3 & 1.59 & 82.75 & 0.42 \\ 
 0.4 & 2.37 & 86.57 & 0.32 \\ \hline
 0.1 & 0.00 & 90.31 & 1.00 \\ 
 0.1 & 0.00 & 87.21 & 1.00 \\ 
 0.2 & 0.00 & 79.63 & 1.00 \\ 
 0.2 & 0.10 & 76.01 & 0.91 \\ 
 0.3 & 0.38 & 78.64 & 0.74 \\ 
 0.5 & 0.71 & 81.88 & 0.60 \\ \hline
 0.1 & 0.00 & 95.16 & 1.00 \\ 
 0.1 & 0.00 & 93.60 & 1.00 \\ 
 0.2 & 0.00 & 89.81 & 1.00 \\ 
 0.2 & 0.00 & 85.52 & 1.00 \\ 
 0.3 & 0.00 & 81.16 & 1.00 \\ 
 0.5 & 0.01 & 77.50 & 0.98 \\ \hline
 0.1 & 0.00 & 96.77 & 1.00 \\ 
 0.1 & 0.00 & 95.74 & 1.00 \\ 
 0.2 & 0.00 & 93.21 & 1.00 \\ 
 0.2 & 0.00 & 90.35 & 1.00 \\ 
 0.3 & 0.00 & 87.44 & 1.00 \\ 
 0.5 & 0.00 & 84.53 & 1.00 \\ \hline
 0.1 & 0.00 & 97.58 & 1.00 \\ 
 0.1 & 0.00 & 96.80 & 1.00 \\ 
 0.2 & 0.00 & 94.90 & 1.00 \\ 
 0.2 & 0.00 & 92.76 & 1.00 \\ 
 0.3 & 0.00 & 90.58 & 1.00 \\ 
 0.5 & 0.00 & 88.40 & 1.00 \\ \hline
 0.1 & 0.00 & 98.06 & 1.00 \\ 
 0.1 & 0.00 & 97.44 & 1.00 \\ 
 0.2 & 0.00 & 95.92 & 1.00 \\
 0.2 & 0.00 & 94.21 & 1.00 \\ 
 0.3 & 0.00 & 92.46 & 1.00 \\ 
 0.5 & 0.00 & 90.72 & 1.00 \\	\hline \hline	\end{tabular}
	\end{tabular}
\caption{Filtri di diverse larghezze centrati su 4000\AA sono deformati dalla presenza di un angolo non telecentrico, a sinistra per un F/1.4 a destra per F/4}\label{table:squarefilternta}
\end{table}

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/SteepFilterNTAdifffiter60.pdf}
	\caption{Deformazione di un filtro quadrato di larghezza 60 \AA  a differenti angoli non-telecentrici con F/1.4. Come apprezzabile in tabella \ref{table:squarefilternta}}\label{figure:squarefilternta}
\end{figure}


\section{Convoluzione filtro spettro}

Per avere un'indicazione più quantitativa dell'effetto di aberrazione differenziale abbiamo simulato l'effetto che la deformazione ha sulla magnitudine di una medesima sorgente\footcite{Pollux_2010} (stesso spettro) posizionata a differenti angoli non telecentrici e filtrata con i filtri quadrati definiti sopra. In tabella \ref{table:convolution1} e tabella \ref{table:convolution2} sono riportati i risultati numerici per F/1.4  e F/4 per un filtro centrato sul doppietto del $CaII$: si può arrivare, anche in un caso \textit{rilassato}, come quello con $FWHM=60\AA$ e $F/4$ evidenziato in tabella \ref{table:convolution2}, a differenze di due decimi di magnitudine. Due sorgenti con lo stesso identico spettro, posizionate una al centro del campo di vista ed una con un angolo non-telecentrico di $10\degree$, possono presentare una magnitudine che differisce di due decimi. Considerando che la maggior parte degli studi sulle popolazioni multiple in ammassi globulari fanno uso di indici di colore (quindi differenze di magnitudini in differenti filtri) o pseudo-colori che si ricavano da tre bande, gli effetti cumulativi possono essere anche maggiori. È però necessario uno studio specifico delle bande di osservazione particolari in relazione allo strumento utilizzato e alle caratteristiche peculiari degli spettri delle sorgenti. Così abbiamo fatto nel capito \ref{chap:casi} ottenendo risultati in controtendenza con le valutazioni espresse in questa sezione, per l'indice $Cn_{JWL}$.\\
In figura \ref{figure:filteredspectra} si può vedere come la differenza in magnitudine sia effettivamente dovuta al deformarsi del filtro, che provoca l'ingresso di flusso a lunghezze d'onda minori, mentre esclude quello a lunghezze maggiori. 

\begin{table}
	\centering
	\begin{tabular}{r|rrrrr}
		& \multicolumn{5}{c}{mag} \\
		width [\AA] & 2\degree & 4\degree & 6\degree & 8\degree & 10\degree \\ \hline \hline
		10 & -0.043 & -0.104 & -0.181 & -0.263 & -0.313 \\ 
		20 & -0.020 & -0.081 & -0.149 & -0.219 & -0.265 \\ 
		40 & -0.019 & -0.059 & -0.105 & -0.145 & -0.181 \\ 
		60 & -0.007 & -0.026 & -0.053 & -0.081 & -0.107 \\ 
		80 & -0.000 & -0.006 & -0.024 & -0.048 & -0.064 \\ 
		100 & -0.003 & -0.008 & -0.017 & -0.025 & -0.030 \\ \hline \hline
	\end{tabular}
\caption{La deformazione di un filtro del tipo precedente con F/1.4 e centrato sul doppietto del CaII, $\lambda=3950\AA$, dovuta alla presenza di un angolo non-telecentrico, porta a variazioni in magnitudine. In particolare, spostandosi verso l'esterno del campo, una stella con il medesimo spettro appare più luminosa che al centro, fino a tre decimi di magnitudine a causa del flusso fuori dalle righe di assorbimento che entra a causa della deformazione. } \label{table:convolution1}
\end{table}

\begin{table}
	\centering
	\begin{tabular}{r|rrrrr}
	band [\AA] & 2\degree & 4\degree & 6\degree & 8\degree & 10\degree \\ \hline \hline
	10 & 0.041 & 0.157 & 0.291 & 0.340 & 0.208 \\ 
	20 & 0.040 & 0.139 & 0.244 & 0.264 & 0.174 \\ 
	40 & -0.003 & -0.010 & -0.031 & -0.070 & -0.144 \\ \hline
	60 & -0.018 & -0.063 & -0.120 & -0.173 & -0.225 \\ \hline
	80 & 0.001 & 0.009 & 0.009 & -0.002 & -0.024 \\ 
	100 & 0.004 & 0.023 & 0.046 & 0.065 & 0.071 \\ \hline \hline
	\end{tabular}
	\caption{Variazioni di magnitudine come in tabella \ref{table:convolution1} ma con F/4, in figura \ref{figure:filteredspectra} si può vedere per il caso del filtro quadrato largo $60\AA$ come varia il flusso a differenti angoli} \label{table:convolution2}
\end{table}

\begin{figure}
	\centering
	\includegraphics[width=0.9\textwidth]{Figure/TransimittedSpectra60-0-f4.pdf}
	\includegraphics[width=0.9\textwidth]{Figure/TransimittedSpectra60-10-f4.pdf}
	\caption{Spettro attraverso filtro quadrato di larghezza $60 \AA$ deformato a differenti angoli non-telecentrici con F/4, sopra nta=0\degree, sotto nta=10\degree. Come apprezzabile in tabella \ref{table:convolution2} alla quarta riga}\label{figure:filteredspectra}
\end{figure}





==> TeX_files/tikzlibraryoptics.code.tex <==
\iffalse
The tikzoptics library

Copyright (C) 2013-2016 by
  Michel Fruchart <michel.fruchart@ens-lyon.org>

This work may be distributed and/or modified under the conditions of
the LaTeX Project Public License (LPPL), version 1.3c, which can be
found at the address:
https://www.latex-project.org/lppl/lppl-1-3c/

Alternatively, it may be distributed and/or modified under the conditions of
the GNU General Public License (GNU GPL), version 2, which can be found
at the address:
https://www.gnu.org/licenses/gpl-2.0.en.html
or any later version published by the Free Software Foundation.
\fi
\makeatletter


\def\tikzopticsversion{0.2.3}
\def\tikzopticsversiondate{2017-03-11}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% errors from this library
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\opticserror#1{\pgfutil@packageerror{tikz/optics}{#1}{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% handler |collect unknowns|
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% from http://tex.stackexchange.com/questions/81821/filtering-options-with-pgfkeys/81985#81985
% used by /tikz/optics/->n-
%
\pgfkeys{
  /handlers/.collect unknowns/.style = {
    unknown options/.initial = {},
    .unknown/.code = {%
      \letcs\reserved{pgfk@\pgfkeyscurrentpath/unknown options}%
      \csedef{pgfk@\pgfkeyscurrentpath/unknown options}{%
        \ifx\reserved\empty\else\expandonce\reserved,\fi
        \expandonce\pgfkeyscurrentname
        \ifx\pgfkeysnovalue##1\else=\expandonce\pgfkeyscurrentvalue\fi
      }%
    }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% defining |optics| family
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfkeys{
  /tikz/.cd,
  optics/.is family,
  optics/.search also={/tikz},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% [use optics] 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfkeys{
  /tikz/use optics/.append code={
  \pgfkeys{
    /tikz/.cd,
      % shapes 
      % FIXME il ne devrait pas y avoir de logique (ni de valeurs par défaut) ici, seulement l'export dans l'espace de nom commun
      lens/.prefix style={shape=lens,optics,draw},
      slit/.prefix style={shape=slit,optics,draw},
      double slit/.prefix style={shape=double slit,optics,draw},
      thin optics element/.prefix style={shape=thin optics element,optics,draw},
      polarizer/.prefix style={shape=polarizer,optics,draw,object aspect ratio=0.1},
      generic optics io/.prefix style={shape=generic optics io,optics,draw},
      sensor/.prefix style={shape=sensor,optics,object aspect ratio=1,draw},
      sensor line/.prefix style={shape=sensor line,optics,draw},
      mirror/.prefix style={shape=mirror,optics,draw},
      spherical mirror/.prefix style={shape=spherical mirror,optics,draw},
      thick optics element/.prefix style={shape=thick optics element,optics,draw,object aspect ratio=0.1},
      heat filter/.prefix style={shape=thick optics element,optics,draw, object aspect ratio=0.05},
      double amici prism/.prefix style={shape=double amici prism,optics,draw, prism height=1cm, prism apex angle=60},
      % styles
      screen/.prefix style={optics,/tikz/optics/screen},
      diffraction grating/.style={optics,/tikz/optics/diffraction grating},
      grid/.style={optics, /tikz/optics/grid},
      semi-transparent mirror/.style={optics, /tikz/optics/semi-transparent mirror},
      diaphragm/.style={optics, /tikz/optics/diaphragm},
      beam splitter/.prefix style={optics,/tikz/optics/beam splitter},
      generic lamp/.prefix style={optics,/tikz/optics/generic lamp},
      generic sensor/.prefix style={optics,/tikz/optics/generic sensor},
      halogen lamp/.prefix style={optics,/tikz/optics/halogen lamp},
      spectral lamp/.prefix style={optics,/tikz/optics/spectral lamp},
      laser/.prefix style={optics,/tikz/optics/laser},
      laser'/.prefix style={optics,/tikz/optics/laser'},
      concave mirror/.prefix style={optics, /tikz/optics/concave mirror},
      convex mirror/.prefix style={optics, /tikz/optics/convex mirror},
      % arrows (styles)
      ->-/.prefix style={optics,/tikz/optics/->-={##1}},
      -<-/.prefix style={optics,/tikz/optics/-<-={##1}},
      ->>-/.prefix style={optics,/tikz/optics/->>-={##1}},
      -<<-/.prefix style={optics,/tikz/optics/-<<-={##1}},
      ->>>-/.prefix style={optics,/tikz/optics/->>>-={##1}},
      -<<<-/.prefix style={optics,/tikz/optics/-<<<-={##1}},
      ->>>>-/.prefix style={optics,/tikz/optics/->>>>-={##1}},
      -<<<<-/.prefix style={optics,/tikz/optics/-<<<<-={##1}},
      ->n-/.prefix style={optics,/tikz/optics/->n-={##1}},
      -<n-/.prefix style={optics,/tikz/optics/-<n-={##1}},
    }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We need some existing tikz libraries and tex packages.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{decorations,decorations.markings, decorations.pathreplacing}
\usepackage{etoolbox}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Key |object height|
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfkeys{/tikz/optics/.cd,
  object height/.initial=2cm,
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [thin optics element]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{thin optics element}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedanchor{\north}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north}{\north}

  \savedanchor{\south}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south}{\south}

  \anchor{east}{\center}
  \anchor{west}{\center}

  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \south%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \north%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }

  \backgroundpath
  {
    \north \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \south \pgf@xb=\pgf@x \pgf@yb=\pgf@y

    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [lens]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\iftikz@optics@lens@converging
\tikz@optics@lens@convergingtrue

% keys
% - focal lens is used to define anchors |east focus| and |west focus|
% - lens height is used to define anchors |lens north| and |lens south|
% - lens type (converging or diverging)
\pgfkeys{/tikz/optics/.cd,
  focal length/.initial=1cm,
  lens height/.initial=0.8,
  lens type/.is choice,
  lens type/converging/.code={\tikz@optics@lens@convergingtrue},
  lens type/diverging/.code={\tikz@optics@lens@convergingfalse}
}
\pgfdeclareshape{lens}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\focalLength{%
    \edef\focalLength{\pgfkeysvalueof{/tikz/optics/focal length}}%
  }

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedmacro\lensHeight{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/lens height}}%
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\lensHeight}{\pgfkeysvalueof{/tikz/optics/lens height}}%
    \else%
      \pgfmathsetlengthmacro{\lensHeight}{\pgfkeysvalueof{/tikz/optics/lens height}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
  }

  \savedanchor{\lensnorth}{
    \pgfpointorigin
    \pgf@y=\lensHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{lens north}{\lensnorth}

  \savedanchor{\lenssouth}{
    \pgfpointorigin
    \pgf@y=\lensHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{lens south}{\lenssouth}

  \savedanchor{\north}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north}{\north}

  \savedanchor{\south}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south}{\south}

  \savedanchor{\eastfocal}{
    \pgf@x=\focalLength%
    \pgf@y=0cm%
  }
  \anchor{east focal point}{\eastfocal}
  \anchor{east focus}{\eastfocal}
  

  \savedanchor{\westfocal}{
    \pgf@x=-\focalLength%
    \pgf@y=0cm%
  }
  \anchor{west focal point}{\westfocal}
  \anchor{west focus}{\westfocal}

  \anchor{east}{\center}
  \anchor{west}{\center}

  \inheritanchorborder[from=thin optics element]

  \backgroundpath
  {
    \north \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \south \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}

    \iftikz@optics@lens@converging
      \pgfsetarrowsstart{lens arrow}
      \pgfsetarrowsend{lens arrow}
    \else
      \pgfsetarrowsstart{lens arrow reversed}
      \pgfsetarrowsend{lens arrow reversed}
    \fi
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [slit]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys : slit height
\pgfkeys{/tikz/optics/.cd,
  slit height/.initial=0.1
}

\pgfdeclareshape{slit}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}
  \anchor{slit center}{\center} 
  % TODO par cohérence ?

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedmacro\slitHeight{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/slit height}}%
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\slitHeight}{\pgfkeysvalueof{/tikz/optics/slit height}}%
    \else%
      \pgfmathsetlengthmacro{\slitHeight}{\pgfkeysvalueof{/tikz/optics/slit height}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
  }

  \savedanchor{\north}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north}{\north}

  \savedanchor{\south}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south}{\south}

  \savedanchor{\slitnorth}{
    \pgf@x=0cm%
    \pgf@y=\slitHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{slit north}{\slitnorth}

  \savedanchor{\slitsouth}{
    \pgf@x=0cm%
    \pgf@y=\slitHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{slit south}{\slitsouth}

  \anchor{east}{\center}
  \anchor{west}{\center}

  \inheritanchorborder[from=thin optics element]

  \backgroundpath
  {
    % erreurs possibles dans la spécification du dessin
    \pgfmathparse{notless(\slitHeight, \objectHeight)}
    \ifnum\pgfmathresult=1
      \opticserror{<slit height> should be strictly lower than <object height> (in slit)}
    \fi
    \north \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \slitnorth \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}

    \south \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \slitsouth \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [double slit]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys :
% - slit height : (relative) height of the holes (each)
% - slit separation : (relative) distance between the centers of the holes
\pgfkeys{/tikz/optics/.cd,
  object height/.initial=2cm,
  slit height/.initial=0.075,
  slit separation/.initial=0.2
}

\pgfdeclareshape{double slit}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}
  
  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedmacro\slitHeight{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/slit height}}%
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\slitHeight}{\pgfkeysvalueof{/tikz/optics/slit height}}%
    \else%
      \pgfmathsetlengthmacro{\slitHeight}{\pgfkeysvalueof{/tikz/optics/slit height}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
  }

  \savedmacro\slitSeparation{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/slit separation}}%
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\slitSeparation}{\pgfkeysvalueof{/tikz/optics/slit separation}}%
    \else%
      \pgfmathsetlengthmacro{\slitSeparation}{\pgfkeysvalueof{/tikz/optics/slit separation}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
  }

  \savedmacro\macro@slitOneCenter{
    \def\macro@slitOneCenter{
      \pgfpointorigin
      \pgf@ya=\slitSeparation
      \pgf@ya=0.5\pgf@ya
      \advance \pgf@y by \pgf@ya
    }
  }

  \savedmacro\macro@slitTwoCenter{
    \def\macro@slitTwoCenter{
      \pgfpointorigin
      \pgf@ya=\slitSeparation
      \pgf@ya=-0.5\pgf@ya
      \advance \pgf@y by \pgf@ya
    }
  }

  \savedanchor{\north}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north}{\north}

  \savedanchor{\south}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south}{\south}

  % slit 1
  \savedanchor{\slitOneCenter}{
    \macro@slitOneCenter
  }
  \anchor{slit 1 center}{\slitOneCenter}

  \savedanchor{\slitOneNorth}{
    \macro@slitOneCenter
    \pgf@ya = \slitHeight
    \pgf@ya = 0.5\pgf@ya
    \advance \pgf@y by \pgf@ya
  }
  \anchor{slit 1 north}{\slitOneNorth}

  \savedanchor{\slitOneSouth}{
    \macro@slitOneCenter
    \pgf@ya = \slitHeight
    \pgf@ya = -0.5\pgf@ya
    \advance \pgf@y by \pgf@ya
  }
  \anchor{slit 1 south}{\slitOneSouth}

  % slit 2
  \savedanchor{\slitTwoCenter}{
    \macro@slitTwoCenter
  }
  \anchor{slit 2 center}{\slitTwoCenter}

  \savedanchor{\slitTwoNorth}{
    \macro@slitTwoCenter
    \pgf@ya = \slitHeight
    \pgf@ya = 0.5\pgf@ya
    \advance \pgf@y by \pgf@ya
  }
  \anchor{slit 2 north}{\slitTwoNorth}

  \savedanchor{\slitTwoSouth}{
    \macro@slitTwoCenter
    \pgf@ya = \slitHeight
    \pgf@ya = -0.5\pgf@ya
    \advance \pgf@y by \pgf@ya
  }
  \anchor{slit 2 south}{\slitTwoSouth}

  \anchor{east}{\center}
  \anchor{west}{\center}

  \inheritanchorborder[from=thin optics element]

  \backgroundpath
  {
    % erreurs possibles dans les spécifications du dessin
    \pgfmathparse{notgreater(\slitSeparation, \slitHeight)}
    \ifnum\pgfmathresult=1
      \opticserror{<slit separation> should be strictly lower than <slit height> (in double slit)}
    \fi
    \pgfmathparse{notless(\slitSeparation+\slitHeight, \objectHeight)}
    \ifnum\pgfmathresult=1
      \opticserror{<slit height> plus <slit separation> should be strictly lower than <object height> (in double slit)}
    \fi
    \north \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \slitOneNorth \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}

    \slitOneSouth \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \slitTwoNorth \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}

    \slitTwoSouth \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \south \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [mirror]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys
% - mirror decoration separation
% - mirror decoration amplitude
\pgfkeys{/tikz/optics/.cd,
  object height/.initial=2cm,
  mirror decoration separation/.initial=0.15cm,
  mirror decoration amplitude/.initial=0.125cm,
}

\pgfdeclareshape{mirror}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedanchor{\north}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north}{\north}

  \savedanchor{\south}{
    \pgf@x=0cm%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south}{\south}

  \anchor{east}{\center}
  \anchor{west}{\center}

  % bof
  \inheritanchorborder[from=thin optics element]

  \backgroundpath
  {
    \north \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \south \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    % We use a border decoration to make a mirror (hachures).
    % First set the decoration parameters :
    % - decoration angle
    % l'angle est 45-180 et on multiplie l'amplitude par -1 pour que la décoration commence et finisse par un trait (c'est un peu louche mais bon)
    \def\pgfdecorationsegmentangle{45-180}%
    % - decoration step length
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/mirror decoration separation}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentlength}{\pgfkeysvalueof{/tikz/optics/mirror decoration separation}}%
    \else%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentlength}{\pgfkeysvalueof{/tikz/optics/mirror decoration separation}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
    % magouillons pour que \pgfdecorationsegmentlength soit un multiple de la longueur ...
    \pgfmathsetmacro\initialstep{\pgfdecorationsegmentlength} 
    \pgfmathsetmacro\totallength{\pgfkeysvalueof{/tikz/optics/object height}} 
    \pgfmathsetmacro\newstep{\totallength/floor(\totallength/\initialstep)} 
    \pgfmathsetlengthmacro{\pgfdecorationsegmentlength}{\newstep}
    % fin magouille
    % - decoration amplitude
    % on multiplie par -1 pour que ça aille dans le bon sens (pour éviter des problèmes louches)
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/mirror decoration amplitude}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentamplitude}{-1*\pgfkeysvalueof{/tikz/optics/mirror decoration amplitude}}%
    \else%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentamplitude}{-1*\pgfkeysvalueof{/tikz/optics/mirror decoration amplitude}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
    % Use decoration.
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfdecoratecurrentpath{border} %
    % dessin du miroir (trait)
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [spherical mirror]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys :
% - spherical mirror angle : the aperture angle of the mirror
% - spherical mirror type (concave or convex)
% - spherical mirror orientation (ltr or rtl)
% The properties of the decoration are controled by the same parameters as in [mirror].
% Height is controled by |object height|, as usual.
\pgfkeys{/tikz/optics/spherical mirror angle/.initial=150}

\newif\iftikz@optics@sphericalmirror@concave
\tikz@optics@sphericalmirror@concavetrue
\pgfkeys{/tikz/optics/.cd,
  spherical mirror type/.is choice,
  spherical mirror type/concave/.code={\tikz@optics@sphericalmirror@concavetrue},
  spherical mirror type/convex/.code={\tikz@optics@sphericalmirror@concavefalse}
}

\newif\iftikz@optics@sphericalmirror@ltr
\tikz@optics@sphericalmirror@ltrtrue
\pgfkeys{/tikz/optics/.cd,
  spherical mirror orientation/.is choice,
  spherical mirror orientation/ltr/.code={\tikz@optics@sphericalmirror@ltrtrue},
  spherical mirror orientation/rtl/.code={\tikz@optics@sphericalmirror@ltrfalse}
}

% shortcuts (styles) : [concave mirror] and [convex mirror]
\pgfkeys{/tikz/optics/.cd,
      concave mirror/.style={optics, spherical mirror, /tikz/optics/spherical mirror type=concave},
      convex mirror/.style={optics, spherical mirror, /tikz/optics/spherical mirror type=convex},
}

\pgfdeclareshape{spherical mirror}{%
  \savedmacro\installsphericalmirrorparameters{%
    %
    % Define a \centerpoint
    %
    \pgfextract@process\centerpoint{%
      \pgfpointorigin
    }%
    %
    % Define height
    %
    \pgfmathsetlengthmacro\height{\pgfkeysvalueof{/tikz/optics/object height}}%
    %
    % Function to define angle from radius
    % use e.g. [spherical mirror angle=from_radius(2cm)] instead of e.g. [spherical mirror angle=90]
    % This can seem somewhat ridiculous as we will undo this when calculating \radius, however it helps providing a simpler API.
    % This function has to be defined before parsing \pgfkeysvalueof{/tikz/optics/spherical mirror angle}.
    %
    \pgfmathdeclarefunction{from_radius}{1}{
      \begingroup
      \pgfmathparse{notless(2*#1,\height)}
      \ifnum\pgfmathresult=0
        \opticserror{(in /tikz/optics/spherical mirror angle=from_radius(R)) : for a spherical mirror, the radius R cannot be smaller than half the height </tikz/optics/object height>. Set a bigger radius of a smaller height.}
      \fi
      \newdimen\angle
      \pgfmathsetlength\angle{2*asin(\height/(2*#1))}
      \pgf@x=\angle
      \pgfmathreturn\pgf@x
      \endgroup
    }
    %
    % Define angle
    %
    \pgfmathsetmacro\angle{\pgfkeysvalueof{/tikz/optics/spherical mirror angle}}
    %
    % Compute radius from height and angle
    %
    \pgfmathsetlengthmacro\radius{\height/(2*sin(\angle/2))}
    %
    % Half of the sector angle is more useful.
    %
    \pgfmathmod{\angle}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi%
    \let\angle\pgfmathresult%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\halfangle\pgfmathresult%
    %
    % Get the start and end angles of the arc.
    %
    \iftikz@optics@sphericalmirror@concave
      \iftikz@optics@sphericalmirror@ltr
        \pgfmathsetmacro\startangle{-\halfangle}
        \pgfmathsetmacro\endangle{+\halfangle}
      \else
        \pgfmathsetmacro\startangle{180-\halfangle}
        \pgfmathsetmacro\endangle{180+\halfangle}
      \fi
      \else
      \iftikz@optics@sphericalmirror@ltr
        \pgfmathsetmacro\startangle{180-\halfangle}
        \pgfmathsetmacro\endangle{180+\halfangle}
      \else
        \pgfmathsetmacro\startangle{-\halfangle}
        \pgfmathsetmacro\endangle{+\halfangle}
      \fi
    \fi
    % 
    % Calculate R cos(angle/2) and R sin(angle/2)
    % 
    \pgfmathabs@{\halfangle}%
    \pgfmathcos@{\pgfmathresult}%
    \let\coshalfangle\pgfmathresult%
    \pgfmathabs@{\halfangle}%
    \pgfmathsin@{\pgfmathresult}%
    \let\sinhalfangle\pgfmathresult%
    \pgfmathsetlength\pgf@xa{\radius*\coshalfangle}
    \edef\rcoshalfangle{\the\pgf@xa}%
    \pgfmathsetlength\pgf@xa{\radius*\sinhalfangle}
    \edef\rsinhalfangle{\the\pgf@xa}%
    %
    % Calculate the arc coordinates
    %
    \pgfextract@process\arcstart{%
      \pgfqpointpolar{\startangle}{\radius}%
      \pgf@xa\pgf@x%
      \pgf@ya\pgf@y%
      \centerpoint%
      \advance\pgf@x\pgf@xa%
      \advance\pgf@y\pgf@ya%
    }%
    \pgfextract@process\arcend{%
      \pgfqpointpolar{\endangle}{\radius}%
      \pgf@xa\pgf@x%
      \pgf@ya\pgf@y%
      \centerpoint%
      \advance\pgf@x\pgf@xa%
      \advance\pgf@y\pgf@ya%
    }%
    \def\convexrtlsetx#1#2{
      \iftikz@optics@sphericalmirror@concave%
        \iftikz@optics@sphericalmirror@ltr%
          \advance\pgf@x by #1
        \else% % => rtl
          \advance\pgf@x by #2
        \fi%
      \else% % => convex
        \iftikz@optics@sphericalmirror@ltr%
          \advance\pgf@x by #2
        \else% % => rtl
          \advance\pgf@x by #1
        \fi%
      \fi%
    }
    \def\convexrtlinvert{%
      \iftikz@optics@sphericalmirror@concave%
        \iftikz@optics@sphericalmirror@ltr%
          %nothing
        \else% % => rtl
          \pgf@x=-\pgf@x%
        \fi%
      \else% % => convex
        \iftikz@optics@sphericalmirror@ltr%
          \pgf@x=-\pgf@x%
        \else% % => rtl
          %nothing
        \fi%
      \fi%
    }%
    %
    % Save everything. 
    % "NB \addtosavedmacro is currently experimental. May get changed." d'après le code où je l'ai piqué
    %
    \addtosavedmacro{\radius}%
    %
    \addtosavedmacro{\rcoshalfangle}%
    \addtosavedmacro{\rsinhalfangle}%
    %
    \addtosavedmacro{\endangle}%
    \addtosavedmacro{\startangle}%
    %
    \addtosavedmacro{\centerpoint}%
    \addtosavedmacro{\arcstart}%
    \addtosavedmacro{\arcend}%
     \addtosavedmacro{\convexrtlinvert}%
    %
  }%
  %
  % Define anchors
  %
  \savedanchor\mirrorcenterpoint{%
    \pgfpointorigin
  }%
  \savedanchor\centerpoint{%
    \pgfpointorigin%
    \advance\pgf@x by \radius%
    \advance\pgf@x by \rcoshalfangle%
    \iftikz@optics@sphericalmirror@concave%
      \iftikz@optics@sphericalmirror@ltr%
        %nothing
      \else% % => rtl
        \pgf@x=-\pgf@x%
      \fi%
    \else% % => convex
      \iftikz@optics@sphericalmirror@ltr%
        \pgf@x=-\pgf@x%
      \else% % => rtl
        %nothing
      \fi%
    \fi%
    \divide\pgf@x by 2%
  }%
  \savedanchor\focalpoint{%
    \pgfpointorigin%
    \pgf@xa=\radius%
    \advance\pgf@x by .5\pgf@xa%
    \iftikz@optics@sphericalmirror@concave%
      \iftikz@optics@sphericalmirror@ltr%
        %nothing
      \else% % => rtl
        \pgf@x=-\pgf@x%
      \fi%
    \else% % => convex
      \iftikz@optics@sphericalmirror@ltr%
        \pgf@x=-\pgf@x%
      \else% % => rtl
        %nothing
      \fi%
    \fi%
  }%
  \savedanchor\north{%
    \pgfpointorigin
    \pgf@xa=0pt
    \advance\pgf@xa by \rcoshalfangle
    \advance\pgf@xa by \radius
    \divide\pgf@xa by 2
    \advance\pgf@x by \pgf@xa
    \advance\pgf@y by \rsinhalfangle
    \convexrtlinvert
  }%
  \savedanchor\arccenter{%
    \centerpoint
    \advance\pgf@x by \radius
    \convexrtlinvert
  }
  \savedanchor\south{%
    \pgfpointorigin
    \pgf@xa=0pt
    \advance\pgf@xa by \rcoshalfangle
    \advance\pgf@xa by \radius
    \divide\pgf@xa by 2
    \advance\pgf@x by \pgf@xa
    \advance\pgf@y by -\rsinhalfangle
    \convexrtlinvert
  }
  \savedanchor\east{%
    \pgfpointorigin
    \convexrtlsetx{\radius}{\rcoshalfangle}
    \convexrtlinvert
  }
  \savedanchor\west{%
    \pgfpointorigin
    \convexrtlsetx{\rcoshalfangle}{\radius}
    \convexrtlinvert
  }
  \savedanchor\northwest{%
    \pgfpointorigin
    \convexrtlsetx{\rcoshalfangle}{\radius}
    \advance\pgf@y by \rsinhalfangle
    \convexrtlinvert
  }
  \savedanchor\southwest{%
    \pgfpointorigin
    \convexrtlsetx{\rcoshalfangle}{\radius}
    \advance\pgf@y by -\rsinhalfangle
    \convexrtlinvert
  }
  \savedanchor\northeast{%
    \pgfpointorigin
    \convexrtlsetx{\radius}{\rcoshalfangle}
    \advance\pgf@y by \rsinhalfangle
    \convexrtlinvert
  }
  \savedanchor\southeast{%
    \pgfpointorigin
    \convexrtlsetx{\radius}{\rcoshalfangle}
    \advance\pgf@y by -\rsinhalfangle
    \convexrtlinvert
  }
  \anchor{arc start}{%
    \installsphericalmirrorparameters%
    \arcstart%
  }
  \anchor{arc end}{%
    \installsphericalmirrorparameters%
    \arcend%
  }
  \anchor{focal point}{%
    \installsphericalmirrorparameters%
    \focalpoint
  }
  \anchor{focus}{%
    \installsphericalmirrorparameters%
    \focalpoint
  }
  \anchor{mirror center}{\mirrorcenterpoint}  
  \anchor{center}{\centerpoint} 
  \anchor{arc center}{\arccenter}
  \anchor{north}{\north}%
  \anchor{south}{\south}%
  \anchor{east}{\east}%
  \anchor{west}{\west}%
  \anchor{north west}{\northwest}%
  \anchor{south west}{\southwest}%
  \anchor{north east}{\northeast}%
  \anchor{south east}{\southeast}%
  %
  % Draw backgroundpath
  %
  \backgroundpath{%
    \installsphericalmirrorparameters%
    % We use a border decoration to make a mirror.
    % First set the decoration parameters :
    % - decoration angle
    \iftikz@optics@sphericalmirror@concave
      \def\pgfdecorationsegmentangle{45}%
    \else
      \def\pgfdecorationsegmentangle{-90-45}%
    \fi
    % - decoration step length
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/mirror decoration separation}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentlength}{\pgfkeysvalueof{/tikz/optics/mirror decoration separation}}%
    \else%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentlength}{\pgfkeysvalueof{/tikz/optics/mirror decoration separation}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
    % magouillons pour que \pgfdecorationsegmentlength soit un multiple de la longueur ...
    \pgfmathsetmacro\initialstep{\pgfdecorationsegmentlength} 
    \pgfmathsetmacro\totallength{(2*pi/360)*\angle*\radius} 
    \pgfmathsetmacro\newstep{\totallength/floor(\totallength/\initialstep)} 
    \pgfmathsetlengthmacro{\pgfdecorationsegmentlength}{\newstep}
    % fin magouille
    % - decoration amplitude
    % on multiplie par -1 pour que ça aille dans le bon sens sans devoir modifier l'angle (pour éviter des problèmes louches)
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/mirror decoration amplitude}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentamplitude}{-1*\pgfkeysvalueof{/tikz/optics/mirror decoration amplitude}}%
    \else%
      \pgfmathsetlengthmacro{\pgfdecorationsegmentamplitude}{-1*\pgfkeysvalueof{/tikz/optics/mirror decoration amplitude}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
    % Now use decoration.
    % Draw decoration of path : an arc of radius \radius from \arcstart to \arcend
    \pgfpathmoveto{\arcstart}%
    \pgfpatharc{\startangle}{\endangle}{\radius}%
    \pgfdecoratecurrentpath{border} %
    % Now draw the path.
    \pgfpathmoveto{\arcstart}%
    \pgfpatharc{\startangle}{\endangle}{\radius}%
  }
  %
  % Anchor border
  % This is needed for anchors .<angle> (like mirror.0, mirror.90, etc.) to work.
  %
  \anchorborder{%
    % Save x and y
    \edef\externalx{\the\pgf@x}%
    \edef\externaly{\the\pgf@y}%
    \installsphericalmirrorparameters%
    % Use circular border
    \pgfpointborderellipse{ \pgfpoint{\externalx}{\externaly} }{ \pgfpoint{\radius}{\radius} }%
  }%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [thick optics element]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys :
% - object aspect ratio (alias : object width)
% ar = largeur/hauteur => largeur = ar * hauteur
\pgfkeys{/tikz/optics/.cd,
  object aspect ratio/.initial=0.2,
  object width/.style={/tikz/optics/object aspect ratio=#1}
}

\pgfdeclareshape{thick optics element}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedmacro\objectWidth{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/object aspect ratio}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/object aspect ratio}}%
    \else%
      \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/object aspect ratio}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
  }

  \savedanchor{\northeast}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
    \pgf@x=0.5\pgf@x%
  }
  \anchor{north east}{\northeast}

  \savedanchor{\southwest}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
    \pgf@x=-0.5\pgf@x%
  }
  \anchor{south west}{\southwest}

  \anchor{north}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{south}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{east}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{west}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{north west}{
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{south east}{
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \inheritanchorborder[from=rectangle]

  \backgroundpath
  {
    % rectangle
    \pgfpathrectanglecorners{\northeast}{\southwest}
  }
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [polarizer]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{polarizer}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/object height}}%
  }

  \savedmacro\objectWidth{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/object aspect ratio}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/object aspect ratio}}%
    \else%
      \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/object aspect ratio}*\pgfkeysvalueof{/tikz/optics/object height}}%
    \fi%
  }

  \savedanchor{\northeast}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
    \pgf@x=0.5\pgf@x%
  }
  \anchor{north east}{\northeast}

  \savedanchor{\southwest}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
    \pgf@x=-0.5\pgf@x%
  }
  \anchor{south west}{\southwest}

  \anchor{north}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{south}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{east}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{west}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{north west}{
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{south east}{
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \inheritanchorborder[from=rectangle]

  \backgroundpath
  {
    % rectangle
    \pgfpathrectanglecorners{\northeast}{\southwest}

    % diagonale du polariseur
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [double amici prism]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys :
% - prism height
% - prism apex angle
\pgfkeys{/tikz/optics/.cd,
  prism height/.initial=1.5cm,
  prism apex angle/.initial=60,
}
% Idea : we get 
% apexAngle
% prismHeight
% demiPrismWidth = tan(apexAngle/2)*prismHeight
%
% so we compute
%
% C = (0,0)
% NE = (demiPrismWidth,0.5*prismHeight)
% SW = (-2*demiPrismWidth,-0.5*prismHeight)
% NW = (-demiPrismWidth,0.5*prismHeight)
% SE = (2*demiPrismWidth,-0.5*prismHeight)
%
% N = (0,0.5*prismHeight)
% S = (0,-0.5*prismHeight)
% E = (3*0.5*demiPrismWidth,0)
% W = (-3.0.5*demiPrismWidth,0)
\pgfdeclareshape{double amici prism}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\prismHeight{%
    \edef\prismHeight{\pgfkeysvalueof{/tikz/optics/prism height}}%
  }

  \savedmacro\apexAngle{%
      \pgfmathsetlengthmacro{\apexAngle}{\pgfkeysvalueof{/tikz/optics/prism apex angle}}
  }

  \savedmacro\demiPrismWidth{%
      \pgfmathsetlengthmacro{\demiPrismWidth}{tan(0.5*\pgfkeysvalueof{/tikz/optics/prism apex angle})*\pgfkeysvalueof{/tikz/optics/prism height}}
  }

  \savedanchor{\northeast}{
    \pgf@x=\demiPrismWidth%
    \pgf@y=\prismHeight%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north east}{\northeast}

  \savedanchor{\southwest}{
    \pgf@x=\demiPrismWidth%
    \pgf@y=\prismHeight%
    \pgf@x=-2\pgf@x%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south west}{\southwest}

  \savedanchor{\northwest}{
    \pgf@x=\demiPrismWidth%
    \pgf@y=\prismHeight%
    \pgf@x=-\pgf@x%
    \pgf@y=0.5\pgf@y%
  }
  \anchor{north west}{\northwest}

  \savedanchor{\southeast}{
    \pgf@x=\demiPrismWidth%
    \pgf@y=\prismHeight%
    \pgf@x=2\pgf@x%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south east}{\southeast}

  \anchor{north}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \savedanchor{\south}{
    \pgfpointorigin
    \pgf@y=\prismHeight%
    \pgf@y=-0.5\pgf@y%
  }
  \anchor{south}{\south}

  \anchor{east}{
    \southeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \advance\pgf@x by\pgf@xb
    \pgf@x=0.5\pgf@x
    \pgf@y=\pgf@ya
    \advance\pgf@y by\pgf@yb
    \pgf@y=0.5\pgf@y
  }

  \anchor{west}{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \advance\pgf@x by\pgf@xb
    \pgf@x=0.5\pgf@x
    \pgf@y=\pgf@ya
    \advance\pgf@y by\pgf@yb
    \pgf@y=0.5\pgf@y
  }

   \inheritanchorborder[from=rectangle]

  \backgroundpath
  {
    \northwest
    \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
    \southwest
    \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
    \southeast
    \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
    \northeast
    \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
    \pgfpathclose
    %
    % FIXME : ceci devrait s'appliquer seulement au triangle intérieur -> un fgpath ou assimilé
    \pgfsetbeveljoin
    \northwest
    \pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
    \south
    \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
    \northeast
    \pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
  }
}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [generic optics io]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% keys :
% - io body height : height of the body of the io body
% - io body aspect ratio (alias io body width) : width/height of the body of the io body
% - io aperture width : width of the output device (condenser, etc.) [in units of io body height]
% - io aperture height : height of the output device (condenser, etc.) [in units of io body height]
% - io aperture shift : vertical shift of the output device [in units of io body height]
% - io orientation (ltr or rtl)
\pgfkeys{/tikz/optics/.cd,
  io body height/.initial=0.75cm,
  io body aspect ratio/.initial=2,
  io aperture width/.initial=0.33,
  io aperture height/.initial=0.66,
  io aperture shift/.initial=0,
}
\pgfkeys{/tikz/optics/io body width/.style={/tikz/optics/io body aspect ratio=#1}}
%
\newif\if@tikz@optics@io@ltr
\@tikz@optics@io@ltrtrue
%
\pgfkeys{/tikz/optics/io orientation/.is choice}
\pgfkeys{/tikz/optics/io orientation/ltr/.code={\@tikz@optics@io@ltrtrue}}
\pgfkeys{/tikz/optics/io orientation/rtl/.code={\@tikz@optics@io@ltrfalse}}
%
\pgfdeclareshape{generic optics io}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/io body height}}%
  }

  \savedmacro\objectWidth{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/io body aspect ratio}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/io body aspect ratio}}%
    \else%
      \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/io body aspect ratio}*\pgfkeysvalueof{/tikz/optics/io body height}}%
    \fi%
  }

  \savedmacro\outHeight{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/io aperture height}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\outHeight}{\pgfkeysvalueof{/tikz/optics/io aperture height}}%
    \else%
      \pgfmathsetlengthmacro{\outHeight}{\pgfkeysvalueof{/tikz/optics/io aperture height}*\pgfkeysvalueof{/tikz/optics/io body height}}%
    \fi%
  }

  \savedmacro\outWidth{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/io aperture width}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\outWidth}{\pgfkeysvalueof{/tikz/optics/io aperture width}}%
    \else%
      \pgfmathsetlengthmacro{\outWidth}{\pgfkeysvalueof{/tikz/optics/io aperture width}*\pgfkeysvalueof{/tikz/optics/io body height}}%
    \fi%
  }

  \savedmacro\outShift{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/io aperture shift}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\outShift}{\pgfkeysvalueof{/tikz/optics/io aperture shift}}%
    \else%
      \pgfmathsetlengthmacro{\outShift}{\pgfkeysvalueof{/tikz/optics/io aperture shift}*\pgfkeysvalueof{/tikz/optics/io body height}}%
    \fi%
  }

  \savedanchor{\bodynortheast}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
    \pgf@x=0.5\pgf@x%
  }
  \anchor{body north east}{\bodynortheast}

  \savedanchor{\bodysouthwest}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
    \pgf@x=-0.5\pgf@x%
  }
  \anchor{body south west}{\bodysouthwest}

  \savedanchor{\outnortheast}{   
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \advance\pgf@x by\outWidth
    \else
      % Right To Left (RTL)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \pgf@x=-\pgf@x%
    \fi
    \pgf@y=0pt%
    \advance\pgf@y by\outHeight
    \pgf@y=0.5\pgf@y%
    \advance\pgf@y by\outShift
  }
  \anchor{aperture north east}{\outnortheast}

  \savedanchor{\outsouthwest}{
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
    \else
      % Right To Left (RTL)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \advance\pgf@x by\outWidth
      \pgf@x=-\pgf@x%
    \fi
    \pgf@y=0pt%
    \advance\pgf@y by\outHeight
    \pgf@y=-0.5\pgf@y%
    \advance\pgf@y by\outShift
  }
  \anchor{aperture south west}{\outsouthwest}

  \savedanchor{\outcenter}{
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      \pgf@x=\objectWidth%
      \advance\pgf@x by\outWidth
    \else
      % Right To Left (RTL)
      \pgf@x=\objectWidth%
      \advance\pgf@x by\outWidth
      \pgf@x=-\pgf@x%
    \fi
    \pgf@x=0.5\pgf@x%
    \pgf@y=0pt%
    \advance\pgf@y by\outShift
  }
  \anchor{aperture center}{\outcenter}
  

  \anchor{body center}{\center}

  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{body north}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodynortheast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }
  % north = body north
  \anchor{north}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodynortheast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{body south}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodysouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }
  % south = body south
  \anchor{south}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodysouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{body east}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodynortheast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{body west}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodysouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{body north west}{
    \bodynortheast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodysouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{body south east}{
    \bodynortheast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \bodysouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }


  \anchor{aperture north}{
    \outcenter \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \outnortheast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{aperture south}{
    \outcenter \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \outsouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{aperture east}{
    \outcenter \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \outnortheast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{aperture west}{
    \outcenter \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \outsouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{aperture north west}{
    \outnortheast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \outsouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{aperture south east}{
    \outnortheast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \outsouthwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{center}{\center}

  \savedanchor{\realeast}{
    \pgfpointorigin
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      %ltr : aperture east (<- out north east)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \advance\pgf@x by\outWidth
      %\pgf@y=0pt%
    \else
      % Right To Left (rtl)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
    \fi
  }
  \anchor{east}{\realeast}

  \savedanchor{\realwest}{
    \pgfpointorigin
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      \pgf@x=\objectWidth%
      \pgf@x=-0.5\pgf@x%
    \else
      % Right To Left (rtl)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \advance\pgf@x by\outWidth
      \pgf@x=-\pgf@x%
    \fi
  }
  \anchor{west}{\realwest}

  % this is used only for the anchorborder
  \savedanchor{\anchorbordersouthwest}{
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      \pgf@x=\objectWidth%
      \pgf@x=-0.5\pgf@x%
    \else
      % Right To Left (rtl)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \advance\pgf@x by\outWidth
      \pgf@x=-\pgf@x%
    \fi
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
  }

  % this is used only for the anchorborder
  \savedanchor{\anchorbordernortheast}{
    \if@tikz@optics@io@ltr
      % Left To Right (LTR)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      \advance\pgf@x by\outWidth
    \else
      % Right To Left (RTL)
      \pgf@x=\objectWidth%
      \pgf@x=0.5\pgf@x%
      %\pgf@x=-\pgf@x%
    \fi
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
  }

  % anchorborder
  % c'est celui de rectangle, mais un peu ajusté
  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \anchorbordersouthwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \anchorbordernortheast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    % \advance\pgf@x by\pgf@xa%
    % \advance\pgf@y by\pgf@ya%
  }

  \backgroundpath
  {
    % corps
    \pgfpathrectanglecorners{\bodynortheast}{\bodysouthwest}
    % out
    \pgfpathrectanglecorners{\outnortheast}{\outsouthwest}

    %\pgfusepath{draw}
    % il ne faut PAS mettre ça pour pouvoir utiliser des styles correctement après (genre double)
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sensors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shape [sensor line]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sensor line.
%
% This defines anchors center, north, south, east, west, north east
% north west, south east, south west, as well as
% pixel <i> <subanchor> with <subanchor> is any of the former.
% ça va être horrible à faire
%
% keys :
% - sensor line height
% - sensor line aspect ratio (largeur en unités de la hauteur du capteur)
% - sensor line pixel number
% - sensor line pixel width (en unités de la largeur du capteur)
% - sensor line inner ysep (en unités de la hauteur du capteur)
\pgfkeys{/tikz/optics/.cd,
  sensor line height/.initial=2cm,
  sensor line aspect ratio/.initial=0.2,
  sensor line pixel number/.initial=5,
  sensor line pixel width/.initial=0.4,
  sensor line inner ysep/.initial=0.05, % entre le bord et les capteurs
}

\pgfdeclareshape{sensor line}
{
  \savedanchor{\center}{
    \pgfpointorigin
  }
  \anchor{center}{\center}

  \savedmacro\objectHeight{%
    \edef\objectHeight{\pgfkeysvalueof{/tikz/optics/sensor line height}}%
  }

  \savedmacro\objectWidth{%
    \pgfmathsetlengthmacro{\objectWidth}{\pgfkeysvalueof{/tikz/optics/sensor line aspect ratio}*\pgfkeysvalueof{/tikz/optics/sensor line height}}
  }

  \savedmacro\pixelNumber{%
    \pgfmathtruncatemacro\pixelNumber{\pgfkeysvalueof{/tikz/optics/sensor line pixel number}}%
  }

  \savedmacro\innerysep{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/sensor line inner ysep}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\innerysep}{\pgfkeysvalueof{/tikz/optics/sensor line inner ysep}}%
    \else%
      \pgfmathsetlengthmacro{\innerysep}{\pgfkeysvalueof{/tikz/optics/sensor line inner ysep}*\pgfkeysvalueof{/tikz/optics/sensor line height}}%
    \fi%
  }
  
  \savedmacro\pixelWidth{%
    \pgfmathparse{\pgfkeysvalueof{/tikz/optics/sensor line pixel width}}
    \ifpgfmathunitsdeclared%
      \pgfmathsetlengthmacro{\pixelWidth}{\pgfkeysvalueof{/tikz/optics/sensor line pixel width}}%
    \else%
      \pgfmathsetlengthmacro{\pixelWidth}{\pgfkeysvalueof{/tikz/optics/sensor line pixel width}*\objectWidth}%
    \fi%
  }

  \savedmacro\pixelHeight{%
    \pgfmathparse{(\objectHeight-2*\innerysep)/\pixelNumber}
    \edef\pixelHeight{\pgfmathresult pt}%
  }

  \savedanchor{\northeast}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=0.5\pgf@y%
    \pgf@x=0.5\pgf@x%
  }
  \anchor{north east}{\northeast}

  \savedanchor{\southwest}{
    \pgf@x=\objectWidth%
    \pgf@y=\objectHeight%
    \pgf@y=-0.5\pgf@y%
    \pgf@x=-0.5\pgf@x%
  }
  \anchor{south west}{\southwest}

  \anchor{north}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{south}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  \anchor{east}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{west}{
    \center \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{north west}{
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xb
    \pgf@y=\pgf@ya
  }

  \anchor{south east}{
    \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@x=\pgf@xa
    \pgf@y=\pgf@yb
  }

  % ok, idée :
  % HAUT (north) du pixel n (allant de 1 à N)
  % \objectHeight/2 - \innerysep - (n-1) * \pixelHeight
  % BAS (south) du pixel n
  % \objectHeight/2 - \innerysep - n * \pixelHeight
  % west = le même que la boite, donc utiliser \southwest
  % east = west + \pixelWidth   

  % Le but de ce code est de définir des ancres
  % pixel <i> <pos>
  % pour <i> = 4, 2, ..., \pixelNumber
  % et <pos> = north, south, east, west, north west, south west, north east south east, center
  % Comme \pixelNumber est défini dynamiquement, il faut passer par cette horreur.
  % Le code est inspiré de pfglibraryshapes.geometric.code.tex (shape regular polygon).
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@sensor line\endcsname{%
    \c@pgf@counta\pixelNumber\relax%
    \pgfmathloop%
      \ifnum\c@pgf@counta>0\relax%
        \pgfutil@ifundefined{pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space north west}{%
        %
        % ...(manually \xdef as \gdef is normally used by \anchor)...
        %
        %
        % pixel surface north
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space north\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pixelWidth
          \noexpand\pgf@x=.5\noexpand\pgf@x
          \noexpand\advance\noexpand\pgf@x by\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface north east
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space north east\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pixelWidth
          \noexpand\advance\noexpand\pgf@x by\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface north west
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space north west\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface south
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space south\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pixelWidth
          \noexpand\pgf@x=.5\noexpand\pgf@x
          \noexpand\advance\noexpand\pgf@x by\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber-1)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface south east
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space south east\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pixelWidth
          \noexpand\advance\noexpand\pgf@x by\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber-1)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface south west
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space south west\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber-1)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface east
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space east\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pixelWidth
          \noexpand\advance\noexpand\pgf@x by\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber-0.5)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface center
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space center\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pixelWidth
          \noexpand\pgf@x=.5\noexpand\pgf@x
          \noexpand\advance\noexpand\pgf@x by\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber-0.5)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
        %
        %
        % pixel surface west
        \expandafter\xdef\csname pgf@anchor@sensor line@pixel\space\the\c@pgf@counta\space west\endcsname{%
          \noexpand\northeast \noexpand\pgf@xa=\noexpand\pgf@x \noexpand\pgf@ya=\noexpand\pgf@y
          \noexpand\southwest \noexpand\pgf@xb=\noexpand\pgf@x \noexpand\pgf@yb=\noexpand\pgf@y
          \noexpand\pgf@x=\noexpand\pgf@xb
          \noexpand\pgf@y=\noexpand\pgf@ya
          \noexpand\newdimen\noexpand\temp@y
          \noexpand\pgfmathsetlength\noexpand\temp@y{(\the\c@pgf@counta-\noexpand\pixelNumber-0.5)*\noexpand\pixelHeight-\noexpand\innerysep}
          \noexpand\advance\noexpand\pgf@y by\noexpand\temp@y
        }%
      }{\c@pgf@counta0\relax}% 
      \advance\c@pgf@counta-1\relax%
    \repeatpgfmathloop% 
  }%

  \inheritanchorborder[from=rectangle]

  \backgroundpath
  {
    % rectangle contour
    \pgfpathrectanglecorners{\northeast}{\southwest}

    % dessin des pixels
    \c@pgf@counta\pixelNumber\relax%
    \pgfmathloop%
      \ifnum\c@pgf@counta>0\relax%
        \newdimen\pixel@northeast@x
        \newdimen\pixel@northeast@y
        \newdimen\pixel@southwest@x
        \newdimen\pixel@southwest@y
        \northeast \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        \southwest \pgf@xb=\pgf@x \pgf@yb=\pgf@y
        % calcul pixel@northeast
        %% calcul x
        \pixel@northeast@x=\pgf@xb
        \advance\pixel@northeast@x by\pixelWidth
        %% calcul y
        \pixel@northeast@y=\pgf@ya
        \newdimen\temp@y
        \pgfmathsetlength\temp@y{(\the\c@pgf@counta-\pixelNumber)*\pixelHeight-\innerysep}
        \advance\pixel@northeast@y by\noexpand\temp@y
        % calcul pixel@southwest
        \pixel@southwest@x=\pgf@xb
        \pixel@southwest@y=\pgf@ya
        \newdimen\temp@y
        \pgfmathsetlength\temp@y{(\the\c@pgf@counta-\pixelNumber-1)*\pixelHeight-\innerysep}
        \advance\pixel@southwest@y by\temp@y
        % dessin
        \pgfpathrectanglecorners{\pgfpoint{\pixel@northeast@x}{\pixel@northeast@y}}{\pgfpoint{\pixel@southwest@x}{\pixel@southwest@y}}
      \advance\c@pgf@counta-1\relax%
    \repeatpgfmathloop% 
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Styles defining optics elements in terms of the existing shapes.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Style [screen]
\pgfkeys{/tikz/optics/screen/.style={thin optics element, very thick}}
% Style [diffraction grating]
\pgfkeys{/tikz/optics/diffraction grating/.style={thin optics element, /tikz/optics/cheating dash={on 4pt off 2pt}}}
% Style [grid]
\pgfkeys{/tikz/optics/grid/.style={thin optics element, /tikz/optics/cheating dash={on 4pt off 2pt}, ultra thick}}
% Style [semi-transparent mirror]
\pgfkeys{/tikz/optics/semi-transparent mirror/.style={thin optics element, densely dotted, thick}}
% Style [diaphragm]
\pgfkeys{/tikz/optics/diaphragm/.style={slit,/tikz/optics/slit height=0.4}}


% Style [generic lamp]
\pgfkeys{/tikz/optics/generic lamp/.style={shape=generic optics io,optics,draw}}
% Style [generic sensor]
\pgfkeys{/tikz/optics/generic sensor/.style={shape=generic optics io,optics,io orientation=rtl,draw, io body height=1cm, io body aspect ratio=0.5, io aperture width=0.15}}
% Style [halogen lamp]
\pgfkeys{/tikz/optics/halogen lamp/.style={/tikz/optics/generic lamp, io body height=0.75cm, io body aspect ratio=2,io aperture width=0.33,io aperture height=0.66,io aperture shift=0}}
% Style [spectral lamp]
\pgfkeys{/tikz/optics/spectral lamp/.style={/tikz/optics/generic lamp, io body height=2.25cm, io body aspect ratio=2/3,io aperture width=0.11,io aperture height=0.22,io aperture shift=0.25,/tikz/optics/io multiline}}
% Style [laser]
\pgfkeys{/tikz/optics/laser/.style={/tikz/optics/generic lamp, io body height=0.5cm, io body aspect ratio=3,io aperture width=0.22,io aperture height=0.5,io aperture shift=0}}
% Style [laser']
\pgfkeys{/tikz/optics/laser'/.style={/tikz/optics/generic lamp, io body height=0.5cm, io body aspect ratio=3,io aperture width=0,io aperture height=0.5,io aperture shift=0}}
% Style [beam splitter]
\pgfkeys{/tikz/optics/beam splitter/.style={shape=polarizer, optics, draw, object height=1cm, object aspect ratio=1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Helper style to draw correctly dashed paths.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% source : http://tex.stackexchange.com/questions/133271/can-tikz-dashed-lines-emulate-pstricks-dashed-lines
% le but est d'avoir des dash symétriques par rapport au milieu et surtout avec un trait entier de chaque côté
\tikzset{
    /tikz/optics/cheating dash/.code args={on #1 off #2}{
        % Use csname so catcode of @ doesn't have do be changed.
        \csname tikz@addoption\endcsname{%
            \pgfgetpath\currentpath%
            \pgfprocessround{\currentpath}{\currentpath}%
            \csname pgf@decorate@parsesoftpath\endcsname{\currentpath}{\currentpath}%
            \pgfmathparse{\csname pgf@decorate@totalpathlength\endcsname-#1}\let\rest=\pgfmathresult%
            \pgfmathparse{#1+#2}\let\onoff=\pgfmathresult%
            \pgfmathparse{max(floor(\rest/\onoff), 1)}\let\nfullonoff=\pgfmathresult%
            \pgfmathparse{max((\rest-\onoff*\nfullonoff)/\nfullonoff+#2, #2)}\let\offexpand=\pgfmathresult%
            \pgfsetdash{{#1}{\offexpand}}{0pt}}%
    }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Helper style for multiline io elements.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfkeys{/tikz/optics/io multiline/.code={\newdimen\tmplen\pgfmathsetlength{\tmplen}{\pgfkeysvalueof{/tikz/optics/io body aspect ratio}*\pgfkeysvalueof{/tikz/optics/io body height}}\tikzset{text width=\the\tmplen,align=center}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Helper styles to mark interesing points
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Style [mark point]
% Describes how interesting points should be drawn (e.g. by [draw focal points], [draw mirror focus], [draw mirror center])
\pgfkeys{/tikz/optics/mark point/.style={optics/mark a cross}}

% Style [draw focal points]
% Should be applied to a [shape=lens] node to draw its focal points according to the style [mark point].
\pgfkeys{/tikz/optics/draw focal points/.style={append after command={
    \pgfextra{
      \begin{pgfinterruptpath}
          \node[/tikz/optics/mark point,#1] at (\tikzlastnode.west focal point) {};
          \node[/tikz/optics/mark point,#1] at (\tikzlastnode.east focal point) {};
      \end{pgfinterruptpath}
    }
  }
}}

% Style [draw mirror focus]
% Should be applied to a [shape=spherical mirror] node to draw its focal point according to the style [mark point].
\pgfkeys{/tikz/optics/draw mirror focus/.style={append after command={
    \pgfextra{
      \begin{pgfinterruptpath}
          \node[/tikz/optics/mark point,#1] at (\tikzlastnode.focus) {};
      \end{pgfinterruptpath}
    }
  }
}}

% Style [draw mirror center]
% Should be applied to a [shape=spherical mirror] node to draw its center according to the style [mark point].
\pgfkeys{/tikz/optics/draw mirror center/.style={append after command={
    \pgfextra{
      \begin{pgfinterruptpath}
          \node[/tikz/optics/mark point,#1] at (\tikzlastnode.mirror center) {};
      \end{pgfinterruptpath}
    }
  }
}}

% Style [mark a cross]
% Draws a cross at the node
\pgfkeys{/tikz/optics/mark a cross/.style={cross out,draw,inner sep=0pt,minimum width=2pt,minimum height=2pt}}

% idée : utiliser pgfextra pour les flèches, si on peut avoir les deux dernières nodes ?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Helper styles to easily put things on paths.
% It is often needed in optics to have e.g. arrows in the middle of a path.
% It is often needed everywhere to be able to put a coordinate somewhere on 
% a path. 
% This is the aim of these helpers.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style [put coordinate]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Le style [put coordinate=<coord> at <pos>] crée une node[coordinate]
% à l'abscisse curviligne <pos> sur le chemin auquel est appliqué le style.
%
% Exemple : 
% \draw[put coordinate=P at 0.3] (0,0) to[bend left] (2cm,0);
% \draw[red] (P) -- (0,0);
%
\tikzset{
  put coordinate/.style args={#1 at #2}{decoration={markings, mark=at position #2 with {\node[coordinate] (#1) {};}},postaction={decorate}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style [put arrow]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% The aim of this horrible mess is that I want expansion to take place at the right time, so I can ask for something like
% \draw[/tikz/optics/->-={at=0.25}, /tikz/optics/->-={at=0.75}] (0,0) -- (2cm,2cm) -- (4cm,0);
% and have it work. Obviously, I want more complicated things (several arrows with different directions, colors, number of >, etc. on the same path).
% With a naive implementation, this does not work and the last setting always wins. 
% A possible solution would be positional arguments, however keywords arguments are Better (tm).
% Hence the need to take care of expansion order, so the specifications apply only to the currently drawn arrow tip.
% The main idea behing this code is to use Magic (tm) so that Things Work (tm) and never touch it again. 
% However, it is obvious from a trivial application of Murphy Law that this will backfire sometime.
% Indeed, a key with positional arguments are used internally (|ordered draw key|), which is called from the parsed arguments.
\tikzset{/tikz/put arrow/.cd,
  pos/.initial=0.5,
  at/.style={pos=#1},
  pos var/.initial={},
  style/.initial={},
  style var/.initial={},
  postaction style/.initial={}, % more expansion magic needed for ->n- and friends (\arrow[thing=stuff] does not seem to work, probably because of the =)
  arrow macro/.initial={arrow},
  arrow macro var/.initial={},
  arrow type/.initial={>},
  arrow type var/.initial={},
  reversed/.style={arrow macro=arrowreversed},
  arrow/.style={arrow type=#1},
  arrow'/.style={arrow type=#1, reversed},
  every arrow/.style={},
}

\tikzset{put arrow/.code={
  % parse arguments correctly
  \tikzset{/tikz/put arrow/.cd, #1}
  \tikzset{/tikz/put arrow/pos var/.expand once={\pgfkeysvalueof{/tikz/put arrow/pos}}}
  \tikzset{/tikz/put arrow/style var/.expanded={\pgfkeysvalueof{/tikz/put arrow/style}}}
  \tikzset{/tikz/put arrow/arrow macro var/.expand once={\pgfkeysvalueof{/tikz/put arrow/arrow macro}}}
  \tikzset{/tikz/put arrow/arrow type var/.expand once={\pgfkeysvalueof{/tikz/put arrow/arrow type}}}
  % call |ordered draw key| which does the real job
  \tikzset{/tikz/put arrow/ordered draw key/.expanded=%
      {\pgfkeysvalueof{/tikz/put arrow/pos var}}%
      {\pgfkeysvalueof{/tikz/put arrow/style var}}%
      {\pgfkeysvalueof{/tikz/put arrow/arrow macro var}}%
      {\pgfkeysvalueof{/tikz/put arrow/arrow type var}}%
      {\pgfkeysvalueof{/tikz/put arrow/postaction style}}%
  }
  % restore initial values
  \tikzset{/tikz/put arrow/pos=0.5} 
  \tikzset{/tikz/put arrow/style={}}
  \tikzset{/tikz/put arrow/arrow macro={arrow}}
  \tikzset{/tikz/put arrow/arrow type={>}}
}}

\tikzset{/tikz/put arrow/ordered draw key/.code n args={5}{
  \tikzset{postaction={#5,decorate, decoration={markings, mark=at position #1 with {\csname #3\endcsname[/tikz/put arrow/every arrow,#2]{#4}};}}}
}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Styles to mark light rays
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{/tikz/optics/multiple ray arrow/.cd,
  n/.initial=1,
  n var/.initial=1,
  set n/.code={\pgfsetarrowoptions{multiple ray arrow}{#1}},
}


\pgfkeys{
  /tikz/optics/.cd, 
  use ray arrow >/.code 2 args={
    \pgfsetarrowoptions{ray arrow@length}{4pt}
    \pgfsetarrowoptions{ray arrow@angle}{50}
    \tikzset{/tikz/put arrow/postaction style/.expanded={/tikz/optics/multiple ray arrow/set n=#1}}
    \tikzset{/tikz/put arrow/.expanded={arrow={multiple ray arrow}, #2}}
  },
  use ray arrow </.code 2 args={
    \pgfsetarrowoptions{ray arrow@length}{4pt}
    \pgfsetarrowoptions{ray arrow@angle}{50}
    \tikzset{/tikz/put arrow/postaction style/.expanded={/tikz/optics/multiple ray arrow/set n=#1}}
    \tikzset{/tikz/put arrow/.expanded={arrow'={multiple ray arrow}, #2}}
  },
  ->n-/.code={
    \tikzset{/tikz/optics/multiple ray arrow/.cd, .collect unknowns,%
      #1,
      unknown options/.get = \arrowkeys}
    \tikzset{/tikz/optics/multiple ray arrow/n var/.expand once={\pgfkeysvalueof{/tikz/optics/multiple ray arrow/n}}}
    \tikzset{/tikz/optics/use ray arrow >={\pgfkeysvalueof{/tikz/optics/multiple ray arrow/n var}}{\arrowkeys}}
  },
  -<n-/.code={
    \tikzset{/tikz/optics/multiple ray arrow/.cd, .collect unknowns,%
      #1,
      unknown options/.get = \arrowkeys}
    \tikzset{/tikz/optics/multiple ray arrow/n var/.expand once={\pgfkeysvalueof{/tikz/optics/multiple ray arrow/n}}}
    \tikzset{/tikz/optics/use ray arrow <={\pgfkeysvalueof{/tikz/optics/multiple ray arrow/n var}}{\arrowkeys}}
  },
  %
  ->-/.style={/tikz/optics/->n-={n=1, #1}},
  -<-/.style={/tikz/optics/-<n-={n=1, #1}},
  ->>-/.style={/tikz/optics/->n-={n=2, #1}},
  -<<-/.style={/tikz/optics/-<n-={n=2, #1}},
  ->>>-/.style={/tikz/optics/->n-={n=3, #1}},
  -<<<-/.style={/tikz/optics/-<n-={n=3, #1}},
  ->>>>-/.style={/tikz/optics/->n-={n=4, #1}},
  -<<<<-/.style={/tikz/optics/-<n-={n=4, #1}},
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Styles [dim arrow] and [short dim arrow]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dimarrow@short@position{0}
\newif\ifdimarrow@nearstart
\dimarrow@nearstarttrue
\tikzset{%
  /tikz/dim arrow/.code={\tikzset{draw,/tikz/dim arrow/draw dim arrow}\pgfkeys{/tikz/dim arrow/.cd,#1}},
  /tikz/dim arrow'/.code={\pgfkeysgetvalue{/tikz/dim arrow/raise}{\tmp@tdar}\tikzset{draw,/tikz/dim arrow/draw dim arrow,/tikz/dim arrow/raise=-\tmp@tdar}\pgfkeys{/tikz/dim arrow/.cd,#1}},
  /tikz/short dim arrow/.code={\tikzset{draw,/tikz/dim arrow/draw short dim arrow}\pgfkeys{/tikz/dim arrow/.cd,#1}},
  /tikz/short dim arrow'/.code={\pgfkeysgetvalue{/tikz/dim arrow/raise}{\tmp@tdar}\tikzset{draw,/tikz/dim arrow/draw short dim arrow,/tikz/dim arrow/raise=-\tmp@tdar}\pgfkeys{/tikz/dim arrow/.cd,#1}},
  /tikz/dim arrow/.cd,
  raise/.initial={0.5cm},
  no raise/.style={raise=0},
  label/.code={\pgfkeys{/tikz/dim arrow/label text=#1}},
  label'/.code={\pgfkeys{/tikz/dim arrow/label text=#1,/tikz/dim arrow/label style/.append style={swap},}},
  label text/.initial={},
  label style/.style={},
  label near start/.code={\def\dimarrow@short@position{0}}, % only short
  label near middle/.code={\def\dimarrow@short@position{2}}, % only short
  label near end/.code={\def\dimarrow@short@position{1}}, % only short
  arrow length/.initial={5mm}, % only for short
  draw short dim arrow/.style={to path={\pgfextra{%
    \let\tikz@mode@save=\tikz@mode%
        \let\tikz@options@save=\tikz@options%
    \newdimen\labelTotalRaise
    \pgfmathsetlength\labelTotalRaise{\pgfkeysvalueof{/tikz/dim arrow/raise}}
        \pgfinterruptpath
        \draw[>=technical,->|] \pgfextra{\let\tikz@mode=\tikz@mode@save\let\tikz@options=\tikz@options@save}
    let
        \p1=($(\tikztostart)!\pgfkeysvalueof{/tikz/dim arrow/raise}!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\pgfkeysvalueof{/tikz/dim arrow/raise}!-90:(\tikztostart)$)
        in ($(\p1)!-\pgfkeysvalueof{/tikz/dim arrow/arrow length}!(\p2)$) -- ($(\p1)!0!(\p2)$);
    \draw[>=technical,->|] \pgfextra{\let\tikz@mode=\tikz@mode@save\let\tikz@options=\tikz@options@save}
    let
        \p1=($(\tikztostart)!\pgfkeysvalueof{/tikz/dim arrow/raise}!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\pgfkeysvalueof{/tikz/dim arrow/raise}!-90:(\tikztostart)$)
        in ($(\p2)!-\pgfkeysvalueof{/tikz/dim arrow/arrow length}!(\p1)$) -- ($(\p2)!0!(\p1)$);
    \ifnum\dimarrow@short@position=0
    \path let 
        \p1=($(\tikztostart)!\labelTotalRaise!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\labelTotalRaise!-90:(\tikztostart)$)
        in let
    \p3=($(\p1)!-1*\pgfkeysvalueof{/tikz/dim arrow/arrow length}!(\p2)$),
    \p4=($(\p1)!-0*\pgfkeysvalueof{/tikz/dim arrow/arrow length}!(\p2)$)
    in
    (\p3) -- (\p4) node[pos=0.5,auto=left,/tikz/dim arrow/label style] {\pgfkeysvalueof{/tikz/dim arrow/label text}};
  \fi
    \ifnum\dimarrow@short@position=1
      \path let 
        \p1=($(\tikztostart)!\labelTotalRaise!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\labelTotalRaise!-90:(\tikztostart)$)
        in let
    \p3=($(\p2)!-1*\pgfkeysvalueof{/tikz/dim arrow/arrow length}!(\p1)$),
    \p4=($(\p2)!-0*\pgfkeysvalueof{/tikz/dim arrow/arrow length}!(\p1)$)
    in
    (\p4) -- (\p3) node[pos=0.5,auto=left,/tikz/dim arrow/label style] {\pgfkeysvalueof{/tikz/dim arrow/label text}};
    \fi
  \ifnum\dimarrow@short@position=2
    \path let 
        \p1=($(\tikztostart)!\labelTotalRaise!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\labelTotalRaise!-90:(\tikztostart)$)
    in
    (\p1) -- (\p2) node[pos=0.5,/tikz/dim arrow/label style] {\pgfkeysvalueof{/tikz/dim arrow/label text}};
  \fi
        \endpgfinterruptpath
      }(\tikztostart) (\tikztotarget) \tikztonodes
    }
  },
  draw dim arrow/.style={to path={\pgfextra{%
    \let\tikz@mode@save=\tikz@mode%
        \let\tikz@options@save=\tikz@options%
    \newdimen\labelTotalRaise
    \pgfmathsetlength\labelTotalRaise{\pgfkeysvalueof{/tikz/dim arrow/raise}}
        \pgfinterruptpath
        \draw[>=technical,|<->|] \pgfextra{\let\tikz@mode=\tikz@mode@save\let\tikz@options=\tikz@options@save}
    let 
        \p1=($(\tikztostart)!\pgfkeysvalueof{/tikz/dim arrow/raise}!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\pgfkeysvalueof{/tikz/dim arrow/raise}!-90:(\tikztostart)$)
        in (\p1) -- (\p2);
    \path let 
        \p1=($(\tikztostart)!\labelTotalRaise!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!\labelTotalRaise!-90:(\tikztostart)$)
        in (\p1) -- (\p2) node[pos=0.5,auto=left,/tikz/dim arrow/label style] {\pgfkeysvalueof{/tikz/dim arrow/label text}};
    % rq : inner sep controle la distance chemin-node
        \endpgfinterruptpath
      }(\tikztostart) (\tikztotarget) \tikztonodes
    }
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arrows
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arrow lens arrow
% used to draw lenses (perhaps not the best idea).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfsetarrowoptions{lens arrow@length}{6pt}
\pgfsetarrowoptions{lens arrow@angle}{50}
\pgfarrowsdeclare{lens arrow}{lens arrow}
{
   \pgfarrowsleftextend{0pt}
   \pgfarrowsrightextend{0pt}
}
{
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfmathsetlength{\pgfutil@tempdimb}{\pgfgetarrowoptions{lens arrow@length}*sin(\pgfgetarrowoptions{lens arrow@angle}/2)}    
  \def\arrow@origin{\pgfpoint{0pt}{0pt}}
  \pgfutil@tempdima=\pgfgetarrowoptions{lens arrow@length}%
  \pgfmathsetmacro{\tmp@lens@angle}{90+\pgfgetarrowoptions{lens arrow@angle}}
  \pgfmathsetmacro{\tmp@lens@anglediv}{\pgfgetarrowoptions{lens arrow@angle}/2}
  \advance\pgfutil@tempdima by -1.5\pgflinewidth%
  \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(\pgfgetarrowoptions{lens arrow@angle}/2)}    
  \pgfpathmoveto{\pgfpointadd{\arrow@origin}{\pgfqpointpolar{\tmp@lens@angle}{\pgfutil@tempdima}}}
  \pgfpathlineto{\arrow@origin}
  \pgfpathlineto{\pgfpointadd{\arrow@origin}{\pgfqpointpolar{-\tmp@lens@angle}{\pgfutil@tempdima}}}
  \pgfusepathqstroke
}
\pgfarrowsdeclarereversed{lens arrow reversed}{lens arrow reversed}{lens arrow}{lens arrow}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ray arrow
% It is useful to have an arrow which goes on the exact middle of a path.
% This is used on ->-, etc.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% flèche utilisée pour marquer les rayons lumineux (avec les styles ->-, etc.)
\pgfsetarrowoptions{ray arrow@length}{4pt}
\pgfsetarrowoptions{ray arrow@angle}{45}

\makeatletter

\pgfsetarrowoptions{multiple ray arrow}{0}
\pgfarrowsdeclare{multiple ray arrow}{multiple ray arrow}
{
    \pgfarrowsleftextend{0pt}
    \pgfarrowsrightextend{0pt}
}
{
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfutil@tempdima=\pgfgetarrowoptions{ray arrow@length}%
  \pgfmathsetmacro{\tmp@ray@angle}{90+\pgfgetarrowoptions{ray arrow@angle}}
  \pgfmathsetmacro{\tmp@ray@anglediv}{\pgfgetarrowoptions{ray arrow@angle}/2}
  \advance\pgfutil@tempdima by -1.5\pgflinewidth%
  \pgfmathsetlength{\pgfutil@tempdima}{\pgfutil@tempdima/cos(\pgfgetarrowoptions{ray arrow@angle}/2)}
  %
  \foreach \i in {1,...,\pgfgetarrowoptions{multiple ray arrow}}
  {
    \pgfmathsetlength{\pgfutil@tempdimb}{(2*\i-\pgfgetarrowoptions{multiple ray arrow})*\pgfgetarrowoptions{ray arrow@length}*sin(\pgfgetarrowoptions{ray arrow@angle}/2)}
    %
    \def\arrow@origin{\pgfpoint{\pgfutil@tempdimb}{0pt}}
    %
    \pgfpathmoveto{\pgfpointadd{\arrow@origin}{\pgfqpointpolar{\tmp@ray@angle}{\pgfutil@tempdima}}}
    \pgfpathlineto{\arrow@origin}
    \pgfpathlineto{\pgfpointadd{\arrow@origin}{\pgfqpointpolar{-\tmp@ray@angle}{\pgfutil@tempdima}}}
    \pgfusepathqstroke
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arrow technical
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\pgfarrowsdeclare{technical}{technical}
{%
  \pgfutil@tempdima=0.48pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfarrowsleftextend{+-3\pgfutil@tempdima}%
  \pgfarrowsrightextend{+8\pgfutil@tempdima}%
}
{%
  \pgfutil@tempdima=0.48pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfpathmoveto{\pgfqpoint{8\pgfutil@tempdima}{0pt}}%
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{3\pgfutil@tempdima}}%
  \pgfpathlineto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{-3\pgfutil@tempdima}}%
  \pgfusepathqfill%
}

\pgfarrowsdeclare{technical reversed}{technical reversed}
{%
  \pgfutil@tempdima=0.48pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfarrowsleftextend{-8\pgfutil@tempdima}
  \pgfarrowsrightextend{-8\pgfutil@tempdima}
}
{%
  \pgfutil@tempdima=0.48pt%
  \pgfutil@tempdimb=\pgflinewidth%
  \ifdim\pgfinnerlinewidth>0pt%
    \pgfmathsetlength\pgfutil@tempdimb{.6\pgflinewidth-.4*\pgfinnerlinewidth}%
  \fi%
  \advance\pgfutil@tempdima by.3\pgfutil@tempdimb%
  \pgfpathmoveto{\pgfqpoint{-8\pgfutil@tempdima}{0pt}}%
  \pgfpathlineto{\pgfqpoint{3\pgfutil@tempdima}{3\pgfutil@tempdima}}%
  \pgfpathlineto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{3\pgfutil@tempdima}{-3\pgfutil@tempdima}}%
  \pgfusepathqfill%
}


% Changelog:
% 2013-10-21 : ajout du style |distance arrow| et de la décoration |line| correspondante.
% 2013-11-19 : suppression de |distance arrow| et ajout à la place de |dim arrow| et assimilés
% 2013-11-22 : choix entre distances relatives et absolues (http://www.texample.net/tikz/examples/supersonic-nozzle/)
% 2013-11-24 : styles de flèches |->-|, |-<-|, |->>-|, |-<<-| (et flèches pgf |ray arrow|, etc. correspondantes)
% 2013-11-24 : flèches pgf |lens arrow| et |lens arrow reversed|
% 2013-11-24 : |generic optics element| -> |thin optics element| et |thick optics element| ; conséquences. |beam splitter|
% 2014-01-01 : ajout de |double amici prism|,  |optics| -> |use optics| et |one arrow| -> |put arrow| ; |mark a *| supprimés
% 2014-03-19 : anchorborder pour |generic optics io| (les labels devraient donc être placés correctement)
%              |io body aspect ratio| accepte désormais aussi des longueurs absolues, ajout d'un alias |io body width| pour |io body aspect ratio|
% 2014-06-26 : modification du code des flèches |->-|, |->>-|, etc. et ajout de |->>>-|, |->>>>-|,|->n-=<nombre>| (idem dans l'autre sens)
% 2014-07-08 : ajout de |arrow style| à |put arrow|
% 2014-09-20 : ajout de |spherical mirror| et quelques modifications à |mirror| (ajustement de la décoration et de ses réglages par défaut)
% 2014-09-22 : ajustements de |spherical mirror| (concave et convexe), et ajout des styles correspondants |convex mirror| et |concave mirror|
% 2014-09-24 : ajustements de |spherical mirror| (ltr/rtl) ; correction des ancres de generic optics io (aperture north, aperture center, aperture south étaient incorrectes)
% 2014-09-25 : corrections à |spherical mirror| (ltr/rtl vs concave/convex) ; 
% 2014-10-02 : ajout d'une fonction |from_radius| pour définir l'angle d'ouverture de |spherical mirror|, encore des corrections à |spherical mirror| (ltr/rtl vs concave/convex) ; 
%               macro pour les messages d'erreur
% 2014-10-03 : vérifications de cohérence des grandeurs pour |slit| et |double slit| ; messages d'erreur au besoin
% 2014-12-07 : modifications substantielles à |put arrow| et |optics/->n-|, etc. pour pouvoir avoir plusieurs flèches sur le même chemin ; la compatibilité arrière est brisée.
% 2014-12-11 : nettoyage
% 2015-03-10 : ajout d'un alias |object width| pour |object aspect ratio|, qui accepte désormais aussi des longueurs absolues
% 2015-06-13 : mise en cohérence des noms des points focaux pour le miroir et la lentille (désormais, "focus" et "focal point")
% 2016-11-21 : appel aux biblothèques tikz |decorations| et |decorations.pathreplacing| qui sont nécessaires
\makeatother
